Degrees of Separation: A Flexible Type System for Data Race Prevention

Data races are a notorious problem in parallel programming. There has been great research interest in type systems that statically prevent data races. Despite the progress in the safety and usability of these systems, lots of existing approaches enforce strict anti-aliasing principles to prevent data races. The adoption of them is often intrusive, in the sense that it invalidates common programming patterns and requires paradigm shifts. We propose Capture Separation Calculus (System CSC), a calculus based on Capture Calculus (System CC<:box), that achieves static data race freedom while being non-intrusive. It allows aliasing in general to permit common programming patterns, but tracks aliasing and controls them when that is necessary to prevent data races. We study the formal properties of System CSC by establishing its type safety and data race freedom. Notably, we establish the data race freedom property by proving the confluence of its reduction semantics. To validate the usability of the calculus, we implement it as an extension to the Scala 3 compiler, and use it to type-check the examples in the paper.

==> figures/mv-sub.tex <==
\begin{wide-rules}

\textbf{Top-level subtyping \quad $\subMDft{T}{U}{E}$}


  \infrule[capt]
  {\subDft{S_1}{S_2}\\
    \subMDft{C_1}{C_2}{E}}
  {\subMDft{\tCap{C_1}{S_1}}{\tCap{C_2}{S_2}}{E}}

\textbf{Subcapturing \quad $\subMDft{C_1}{C_2}{E}$}

\begin{multicols}{2}

  \infrule[capt-var]
  {\G(x) = \tCap{C}{S}\andalso \new{{\fresh} \notin C}\\
  \subMDft{C^\theta}{C^\prime}{E}}
  {\subMDft{\set{x^\theta}}{C^\prime}{E}}

  \newruletrue
  \infrule[capt-fresh]
  {\G(x) = \tCap{\set{\fresh}}{S}\\
    \subMDft{\set{\fresh}}{C}{E} \\
    \theta \in \set{\pEx, \pArb}}
  {\subMDft{\set{x^\theta}}{C}{E \cup \set{x}}}
  \newrulefalse

  \infrule[capt-elem]
  {c \in C}
  {\subMDft{\set{c}}{C}{\varemptyset}}

  \infrule[capt-set]
  {\subMDft{\set{c_1}}{C}{E_1} \\
    \cdots \\
    \subMDft{\set{c_n}}{C}{E_n}}
  {\subMDft{\set{c_1, \cdots, c_n}}{C}{\bigcup_{i=1}^n E_i}}

  \newruletrue
  \infrule[capt-ex]
  {\subMDft{\set{{x}^\pEx}}{C}{E}}
  {\subMDft{\set{x^\pArb}}{C}{E}}

  \infrule[capt-*]
  {\subMDft{\set{*^\theta}}{C}{E}}
  {\subMDft{\set{x^\theta}}{C}{E}}
  \newrulefalse

\end{multicols}

\caption{Subtyping and subcapturing rules.}
  \label{fig:mv-sub}

\end{wide-rules}


==> figures/mv-typ.tex <==
\begin{wide-rules}

\textbf{Typing \quad $\typMDft{t}{\sigma}{E}$}

\begin{multicols}{2}

  \infrule[var]
  {x : \tCap CS \in \G}
  {\typMDft{x}{\tCapSet{x}{S}}{\varemptyset}}

  % \infrule[sub]
  % {\typMDft{t}{T}{E_1} \\
  % \subMDft{T}{U}{E_2}}
  % {\typMDft{t}{U}{E_1 \cup E_2}}

  \infrule[ex]
  {\typMDft{x}{\tCap{C}{S}}{\varemptyset}}
  {\typMDft{\ex{x}}{\tCap{\set{x^\pEx}}{S}}{\varemptyset}}

  \infrule[abs]
  {\typ{[\G], x : U}{t}{\tau} \\ \wfTyp{\G}{U} \andalso \excEnv{[\G], x : U}}
  {\typDft{\tLambda{x}{U}{t}}{\tCap{\cv{t}/x}{\tForall{x}{U}{\tau}}}}

  \infrule[tabs]
  {\typ{\extendGT{X}{S}}{t}{\tau} \\ \wfTyp{\G}{S}}
  {\typDft{\tTLambda{X}{S}{t}}{\tCap{\cv{t}}{\tTForall{X}{S}{\tau}}}}

  \infrule[app]
  {\typM{[\G]}{x}{\tCap{C}{\tForall{z}{T}{U}}}{\varemptyset} \\
    \typMDft{y}{T^\prime}{\varemptyset} \\
    \subMDft{T^\prime}{T}{E}\\
    \dropped{[\G]}{E}}
  {\typMDft{x\ y}{[y/z]{U}}{E}}

  \infrule[tapp]
  {\typMDft{x}{\tCap{C}{\tTForall{X}{S}{T}}}{\varemptyset} \\
    \subMDft{S^\prime}{S}{\varemptyset}}
  {\typMDft{x[S^\prime]}{[S/X]{U}}{\varemptyset}}

  \infrule[box]
  {\typMDft{x}{\tCap C S}{\varemptyset} \\ C \subseteq \dom{\G}}
  {\typMDft{\tBox{x}}{\tBox{\tCap C S}}{\varemptyset}}

  \infrule[unbox]
  {\typMDft{x}{\tBox{\tCap C S}}{\varemptyset} \\ C \subseteq \dom{\G}}
  {\typMDft{\tUnbox{C}{x}}{\tCap{C}{S}}{\varemptyset}}

\end{multicols}

% \begin{multicols}{2}

%   \infrule[read]
%   {\typDft{x}{\tCap{\set{x}}{\tRef{S}}}}
%   {\typDft{\tRead{x}}{S}}

%   \infrule[write]
%   {\typDft{x}{\tCap{\set{x}}{\tRef{S}}}\\
%    \typDft{t}{S}}
%   {\typDft{\tWrite{x}{t}}{\tUnit}}

% \end{multicols}

% \infrule[kill]
% {\typDft{x}{\tCap{\set{x}}{\tRef{S}}}\\
%  \typDft{k}{\tCap{\set{\kx{x}}}{\top}}}
% {\typDft{\tKill{k}{x}}{\tUnit}}

\begin{multicols}{2}

\infrule[let-fresh]
{\typMDft{s}{\tCap{\set{\fresh}}{S}}{E_1} \\
  \typM{[\G], x: \tCap{\set{\fresh}}{S}}{t}{\tau}{E_2}\\ %k_x: \tCap{\set{\kx{x}}}{\top}
  \tau^\prime = \generalise{x}{\tau}\\
  \dropped{[\G]}{E_1}}
{\typMDft{\tLet{x}{s}{t}}{\tau^\prime}{E_1 \cup E_2}}

\infrule[let]
{\typMDft{s}{\exists \overline{x_i}. \tCap{C}{S}}{E_1}\\
  \typM{\G^\prime}{t}{\tau}{E_2}\andalso
  x \notin \fv{\tau} \\
  \G^\prime = [\G], \overline{y_i : \tCap{\set{\fresh}}{\top}}, x : [\overline{y_i}/\overline{x_i}](\tCap{C}{S})\\
  \tau^\prime = \generalise{\overline{y_i}}{U}\\
  \excEnv{\G^\prime} \andalso \dropped{\G^\prime}{E_1}}
 % U^\prime = \generalise{\overline{y_i}}{\overline{\tCap{\set{\exex}}{S_i}}}{U}}
{\typMDft{\tLetEx{\overline{y_i}}{x}{s}{t}}{\tau^\prime}{E_1 \cup E_2}}

\end{multicols}

\caption{Typing rules.}
  \label{fig:mv-typ}

\end{wide-rules}


==> figures/reachable.tex <==
\begin{wide-rules}

% \textbf{Reachable Roots \quad $\reachDft{C_1}{C_2}$}

% \begin{multicols}{2}

%   \infrule[\pEx{}-share]
%   {\G(x) = \tCap{\excs{C}}{S}}
%   {\reachDft{\set{x}}{\set{x}}}

%   \infax[\pEx{}-exc]
%   {\reachDft{\set{x^\pEx}}{\set{x^\pEx}}}

%   \infax[$*$]
%   {\reachDft{\set{*}}{\dom{\G}^\pEx}}

%   \infrule[\ures{}-var]
%   {x : \tCap{\urcs{C}}{S} \in \G}
%   {\reachDft{\set{x}}{\varemptyset}}

%   \infrule[var]
%   {\G(x) = \tCap{C_s}{S} \\
%   \reachDft{C}{C^\prime}}
%   {\reachDft{\set{x}}{C^\prime}}

%   \infrule[set]
%   {\reachDft{\set{c_1}}{C_1}\\
%     \cdots\\
%     \reachDft{\set{c_n}}{C_n}}
%   {\reachDft{\set{c_1, \cdots, c_n}}{\bigcup_{i=1}^n C_i}}

%   % \infrule[{!}]
%   % {\G(x) = \tCap{\{{!}\}}{S}}
%   % {\reachDft{\set{x}}{\set{x^\pEx}}}

%   % \infrule[\pEx{}]
%   % {\G(x) = \tCap{\{\pEx{}\}}{S}}
%   % {\reachDft{\set{x}}{\{ x^\pEx \ | \ \forall x. x : \tCap{\set{\fresh}}{S} \in \G \}}}

%   % \infrule[{*}]
%   % {\G(x) = \tCap{\set{*}}{S}}
%   % {\reachDft{\set{x}}{\{ x^\pEx \ | \ \forall x. x : \tCap{\set{\fresh}}{S} \in \G \}}}

%   % \infrule[*-$\pArb$]
%   % {\G(x) = \tCap{\set{*}}{S}}
%   % {\reachDft{\set{x^\pArb}}{\set{x^\pArb}}}

%   % \infrule[*-$\pEx$]
%   % {\G(x) = \tCap{\set{*}}{S}}
%   % {\reachDft{\set{{x}^\pEx}}{\set{ x^\pEx \ | \ \forall x. \G(x) = \tCap{\set{\fresh}}{S} }}}

% \end{multicols}

\textbf{Non-Interfering \quad $\ninter{\G}{x}{y}$}

\infrule[ninter]
{\fConflict{\G}{\fClosure{\G}{x}} \cap \fClosure{\G}{y} = \varemptyset\\
  \fConflict{\G}{\fClosure{\G}{y}} \cap \fClosure{\G}{x} = \varemptyset}
{\ninter{\G}{x}{y}}

% \textbf{Exclusive Environment \quad $\excEnv{\G}$}

% \infrule[exc-env]
% {\domR{\G} = \{x_1, \cdots, x_n\}\\
%   \reachDft{x_1}{C_1}\\
%   \cdots\\
%   \reachDft{x_n}{C_n}\\
%   \neg(\exists x \exists i \exists j. x^\pEx \in C_i \wedge (x^\theta \in C_j \vee * \in C_j))\\
%   \neg(\exists x \exists i \exists j. x : \{*\} \in \G \wedge x^\pArb \in C_i \wedge x^\pArb \in C_j)}
% {\ninter{\G}}

% \textbf{Disjoint Capture Set \quad $\disjcs{\G}{C}$}

% \infrule[disj]
% {\reachDft{C}{\set{x_1^\pEx, x_2^\pEx, \cdots, x_n^\pEx}}}
% {\disjcs{\G}{C}}

\caption{Non-Interference}
\label{fig:exclusive-environment}

\end{wide-rules}

==> figures/reduction.tex <==
\begin{wide-rules}

\textbf{Store Context}

\begin{equation*}
	\sta  \quad ::=  \quad \cdot \OR \sta, \tVal{x} \mapsto v
  \OR \sta, \tVar{x} = v
  \OR \sta, \tSet{x} = v
  % []  \OR  \tLet{x}{v}{\sigma}  \OR  \tLetVar{x}{v}{\sigma}
  % \OR  \tSetVar{x}{v}{\sigma}
\end{equation*}

\textbf{Evaluation Context}
\begin{equation*}
	e  \quad ::=  \quad  []  %\OR  \tLet{x}{e}{t}  %\OR  \tLetVar{x}{e}{t}
  \OR  \tLetMode{m}{x}{e}{t}
  \OR \tLetMode{\parmode}{x}{t}{e}
\end{equation*}

\textbf{Reduction \quad $\reduction{\stDft{t}}{\st{\sta^\prime}{{t^\prime}}}$}

\begin{multicols}{2}

  \infrule[\ruledef{apply}]
  {\sta(\tVal{x}) = \lambda(z :_{D} T) t}
  {\reduction{\stDft{\evctx{x\,y}}}{\stDft{\evctx{[y/z]t}}}}

  % \infrule[apply-$\epsilon$]
  % {\sta(\tVal{x}) = \lambda(z :_{\epsilon} T) t \andalso \sta(\tVal{y}) = v}
  % {\reduction{\stDft{\evctx{x\,y}}}{\st{\sta, \tValM{\epsilon}{z} \mapsto {v}}{\evctx{t}}}}

  \infrule[\ruledef{tapply}]
  {\sta(\tVal{x}) = \lambda[X <: S^\prime] t}
  {\reduction{\stDft{\evctx{x[S]}}}{\stDft{\evctx{[S/X]t}}}}

  \infrule[\ruledef{open}]
  {\sta(\tVal{x}) = \Box{} \, y}
  {\reduction{\stDft{\evctx{\tUnbox{C}{x}}}}{\stDft{\evctx{y}}}}

  \infrule[\ruledef{get}]
  {\sta(\tVal{x}) = \reader y\andalso \sta(\tVar{y}) = v}
  {\reduction{\stDft{\evctx{\tRead{x}}}}{\stDft{\evctx{v}}}}

\end{multicols}

\begin{multicols}{2}

	% \infax[rename-$\epsilon$]
  % {\reduction{\stDft{\evctx{\tLetMode{\epsilon}{x}{y}{t}}}}{\stDft{\evctx{[y/x]t}}}}

  \infrule[\ruledef{lift-let}]
  {\fv{v} \subseteq \dom{\sta}}
  {\reduction{\stDft{\evctx{\tLetMode{m}{x}{v}{t}}}}{\st{\gamma, \tVal{x} \mapsto v}{\evctx{t}}}}

  \infax[\ruledef{rename}]
  % {y \in \bvalM{!}{\sta} \cup \bvar{\sta}}
  {\reduction{\stDft{\evctx{\tLetMode{m}{x}{y}{t}}}}{\stDft{\evctx{[y/x]t}}}}

  % \infrule[lookup-$\epsilon$]
  % {y \in \bvalM{\epsilon}{\sta} \andalso \sta(\tVal{y}) = v}
  % {\reduction{\stDft{\evctx{\tLetMode{m}{x}{y}{t}}}}{\st{\sta, \tValM{m}{x} \mapsto v}{\evctx{t}}}}

\end{multicols}

% \begin{multicols}{2}

%   % \infrule[let$_{!}$-value]
%   % {e \neq []}
%   % {\reduction{\stevctx{\tLetPar{x}{v}{t}}}{\stctx{\tLetPar{x}{v}{\evctx{t}}}}}

% 	\infax[let$_{!}$-value]
%   % {e \neq []}
%   {\reduction{\stDft{\tLetPar{x}{v}{t}}}{\st{\gamma, \tVal{x} \mapsto v}{t}}}

% 	\infax[rename$_!$]
%   {\reduction{\stDft{\tLetPar{x}{y}{t}}}{\stDft{[y/x]t}}}

% \end{multicols}

% \begin{multicols}{2}

	% \infrule[var-value]
  % {\dom{e} \cap \fv{v} = \varemptyset}
  % {\reduction{\stDft{\evctx{\tLetVar{x}{v}{t}}}}{\st{\sta, \tVar{x} \mapsto v}{\evctx{t}}}}


% \end{multicols}

\begin{multicols}{2}

  \infrule[\ruledef{lift-var}]
  {\sta(\tVal{y}) = v}
  {\reduction{\stDft{\evctx{\tLetVarM{D}{x}{y}{t}}}}{\st{\sta, \tVar{x} = v}{\evctx{t}}}}

  \infrule[\ruledef{lift-set}]
  {\sta(\tVal{y}) = v}
  {\reduction{\stDft{\evctx{\tWrite{x}{y}}}}{\st{\sta,\tSet{x} = v}{\evctx{v}}}}

\end{multicols}

% \infrule[let-ctx]
% {\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}}
% {\reduction{\stDft{\tLetBoth{x}{t}{u}}}{\st{\sta^\prime}{\tLetBoth{x}{t^\prime}{u}}}}

% \infrule[let-par]
% {\reduction{\stDft{u}}{\st{\sta^\prime}{u^\prime}} \andalso x \notin \fv{u}}
% {\reduction{\stDft{\tLetPar{x}{t}{u}}}{\st{\sta^\prime}{\tLetPar{x}{t}{u^\prime}}}}

  % \infrule[let-par]
  % {\reduction{\stevctx{u}}{\stevctx{u^\prime}} \andalso x \notin \fv{u}}
  % {\reduction{\stevctx{\tLetPar{x}{t}{u}}}{\stevctx{\tLetPar{x}{t}{u^\prime}}}}

\caption{Operational Semantics}
\label{fig:reduction}

\end{wide-rules}

==> figures/subtyp.tex <==
\begin{wide-rules}

  \textbf{Subtyping \quad $\subDft{T}{U}$}

  \begin{multicols}{2}

    \infax[\ruledef{refl}]
    {\subDft{T}{T}}

    \infrule[\ruledef{trans}]
    {\subDft{T_1}{T_2} \andalso \subDft{T_2}{T_3}}
    {\subDft{T_1}{T_3}}

    \infrule[\ruledef{tvar}]
    {X <: S \in \G}
    {\subDft{X}{S}}

    \infax[\ruledef{top}]
    {\subDft{T}{\top}}

    \infrule[\ruledef{fun}]
    {\subDft{U_2}{U_1} \\
      \sub{\G, {x}:_D {U_2}}{T_1}{T_2}}
    {\subDft{\forall(x :_{{D}} U_1) T_1}{\forall(x :_{{D}} U_2) T_2}}

    \infrule[\ruledef{tfun}]
    {\subDft{S_2}{S_1} \\
      \sub{\G, X <: S_2}{T_1}{T_2}}
    {\subDft{\tTForall{X}{S_1}{T_1}}{\tTForall{X}{S_2}{T_2}}}

    \infrule[\ruledef{capt}]
    {\subDft{C_1}{C_2} \\
      \subDft{S_1}{S_2}}
    {\subDft{\tCap{C_1}{S_1}}{\tCap{C_2}{S_2}}}

    \infrule[\ruledef{boxed}]
    {\subDft{T_1}{T_2}}
    {\subDft{\tBox{T_1}}{\tBox{T_2}}}

  \end{multicols}

  % \textbf{Reader detection \quad $\isrdr{\G}{\cdot}$}

  % \begin{multicols}{3}

  %   \infax[\ruledef{rd-reader}]
  %   {\isrdr{\G}{C\,\tRdr{S}}}

  %   \infrule[\ruledef{rd-widen}]
  %   {X <: S \in \G \\ \isrdr{\G}{C\,S}}
  %   {\isrdr{\G}{C\,X}}

  %   \infrule[\ruledef{rd-var}]
  %   {x : T \in \G \\ \isrdr{\G}{T}}
  %   {\isrdr{\G}{x}}

  % \end{multicols}

  \textbf{Subcapturing \quad $\subDft{C_1}{C_2}$}

  \begin{multicols}{4}

    \infrule[\ruledef{sc-trans}]
    {\subDft{C_1}{C_2} \\ \subDft{C_2}{C_3}}
    {\subDft{C_1}{C_3}}

    \infrule[\ruledef{sc-var}]
    {x : \tCap{C}{S} \in \G}
    {\subDft{\set{x}}{C}}

    \infrule[\ruledef{sc-elem}]
    {x \in C}
    {\subDft{\set{x}}{C}}

    \infrule[\ruledef{sc-set}]
    {\overline{\subDft{\set{x}}{C_2}}^{x \in C_1}}
    {\subDft{C_1}{C_2}}

%    \newruletrue
%    \infrule[\ruledef{sc-read}]
%    {\subDft{\set{x}}{C}}
%    {\subDft{\set{x^{?}}}{C}}
%    \newrulefalse

  \end{multicols}

  \begin{multicols}{2}
    \newruletrue
    \infax[\ruledef{sc-rdr-cap}]
    {\subDft{\set{\rdroot}}{\set{\univ}}}
    % {\subDft{\set{\rdroot}}{C}}

    \infrule[\ruledef{sc-reader}]
    {\isrdr{\G}{x}}
      % \subDft{\set{\rdroot}}{C}}
    {\subDft{\set{x}}{\set{\rdroot}}}
    \newrulefalse
  \end{multicols}

  where $\new{\isrdr{\G}{x}} \quad\triangleq\quad (x : T \in \G) \wedge (\sub{\G}{T}{\tRdr{S}\capt C})$ for some $T, C, S$
  \\

  % \begin{align*}
  %   &\isrdr{\G}{x} \quad &\text{if $x : T \in \G$ and $\isrdr{\G}{T}$}\tag*{(\textsc{rd-var})}\label{rd-var} \\
  %   &\isrdr{\G}{C\,X} \quad &\text{if $X <: S \in \G$ and $\isrdr{\G}{C\,S}$}\tag*{(\textsc{rd-widen})}\label{rd-widen} \\
  %   &\isrdr{\G}{C\,\tRdr{S}} \quad &\text{}\tag*{(\textsc{rd-reader})}\label{rd-reader} \\
  % \end{align*}

  \caption{Subtyping and subcapturing rules}
  \label{fig:subtyp}

\end{wide-rules}

==> figures/typ.tex <==
\begin{wide-rules}

\textbf{Context \quad $\G$}

\begin{equation*}
	\G \quad ::= \quad \emptyset \OR \G, X <: S \OR \G, x \new{:_{D}} T \quad \text{if $x \notin \set{\univ{}, \rdroot{}}$}
\end{equation*}

\textbf{Typing \quad $\typDft{t}{T}$}

\begin{multicols}{2}

  \infrule[\ruledef{var}]
  {x : S\capt C \in \G}
  {\typ{\G}{x}{S\capt \set{x}}}

  % \infrule[ex]
  % {x^\alpha : \pEx\,\tCap{C_s}{S} \in \G}
  % {\typDft{x^\pEx}{\tCap{\set{x^\pEx}}{S}}}

  \infrule[\ruledef{sub}]
  {\typDft{t}{T} \\
  \subDft{T}{U}}
  {\typDft{t}{U}}

  \infrule[\ruledef{abs}]
  {\typ{\G, x:_D U}{t}{T} \\
    \wfTyp{\G}{U} \andalso
    \wfTyp{\G}{D}}
  {\typDft{\lambda(x:_D U). t}{\tCap{\cv{t}\!\setminus\!x}{\forall(x:_D U) T}}}

  \infrule[\ruledef{tabs}]
  {\typ{\G, {X} <: {S}}{t}{T} \andalso \wfTyp{\G}{S}}
  {\typDft{\tTLambda{X}{S}{t}}{\tCap{\cv{t}}{\tTForall{X}{S}{T}}}}

  \infrule[\ruledef{app}]
  {\typM{}{\G}{x}{\tCap{C}{\forall(z {:_D} T) U}} \\
    \typ{\G}{y}{T} \andalso \new{\ninter{\G}{y}{D}}}
  {\typDft{x\ y}{\fSubst{z}{y}{U}}}

  % \infrule[app-$!$]
  % {\typ{\G}{x}{\tCap{C}{\forall(z {:_!} T) U}} \\
  %   \typ{\G}{y}{T} \andalso \ninter{\G}{x}{y}}
  % {\typDft{x\ y}{[y/z]{U}}}

  % \infrule[app-$!$]
  % {\typDft{x}{\tCap{C}{\forall(z \new{:_!} T)U}} \\
  %   \typDft{y}{T} \andalso \new{\ninter{\G}{x}{y}}}
  % {\typDft{x\ y}{[y/z]{U}}}

  % \infrule[app-\pEx{}]
  % {\typDft{x}{C_f\, \tForall{z^\pEx}{\tCap{\excs{C}}{S}}{T}}\\
  %   \typDft{y}{\tCap{C_s}{S}} \andalso \ninter{\G}{x}{y}}
  % {\typDft{x\,y}{[y/z] T}}

  % \infrule[app-{!}]
  % {\typDft{x}{\tCap{C}{\tForall{z}{\tCap{\set{{!}}}{S}}{U}}}\\
  %   \typDft{y}{\tCap{C}{S}} \andalso \ninter{\G}{x}{y}}
  % {\typDft{x\ y}{[y/z]U}}

  \infrule[\ruledef{tapp}]
  {\typDft{x}{\tCap{C}{\tTForall{X}{S}{T}}}}
  {\typDft{x[S]}{\fSubst{X}{S} {U}}}

  \infrule[\ruledef{box}]
  {\typDft{x}{\tCap C S} \\ C \subseteq \dom{\G}}
  {\typDft{\tBox{x}}{\tBox{\tCap C S}}}

  \infrule[\ruledef{unbox}]
  {\typDft{x}{\tBox{\tCap C S}} \\ C \subseteq \dom{\G}}
  {\typDft{\tUnbox{C}{x}}{\tCap{C}{S}}}

\end{multicols}

\begin{multicols}{2}

\infrule[\ruledef{let}]
{\typDft{s}{T}\\
  \typ{\G, {x :_{\set{}} T}}{t}{U}\andalso
  x \notin \fv{U} \\
  % \wfTyp{\G}{m} \\
  % \ninter{\G}{{\cs{T}}}{D} \andalso
  \new{\ninter{\G}{s}{t} \quad\text{if $m = \parmode$}}}
{\typDft{\tLetMode{m}{x}{s}{t}}{U}}


  \newruletrue
  \infrule[\ruledef{dvar}]
  {\typDft{y}{S} \\
    \typ{\G, x :_{D} \tCap{\set{\univ}}{\tRef{S}}}{t}{U}\\
    x \notin \fv{U} \andalso \wfTyp{\G}{D}}
  {\typDft{\tLetVar{x}{y}{t}}{U}}
  \newrulefalse

\end{multicols}

% \infrule[let-$!$]
% {\typDft{s}{T} \andalso \ninter{\G}{\cv{s}}{\cv{t}/{x^*}} \\
%   \typ{\G, \new{x :_\epsilon T}}{t}{U}\andalso
%   x \notin \fv{U}}
% {\typDft{\tLetPar{x}{s}{t}}{U}}

\begin{multicols}{3}

  \newruletrue
  \infrule[\ruledef{reader}]
  {\typDft{x}{\tRef{S}\capt C}}
  {\typDft{\reader x}{\tRdr{S}\captset{x}}}

  \infrule[\ruledef{read}]
  {\typDft{x}{\tCap{C}{\tRdr{S}}}}
  {\typDft{\tRead{x}}{S}}

  \infrule[\ruledef{write}]
  {\typDft{x}{\tCap{C}{\tRef{S}}}\\
    \typDft{y}{S}}
  {\typDft{\tWrite{x}{y}}{S}}
  \newrulefalse

\end{multicols}

\caption{Typing rules}
  \label{fig:typ}

\end{wide-rules}


==> sections/metatheory/ninter.tex <==
\subsection{Non-Interference Guarantee}

In this section, we prove the non-interference guarantee promised by the calculus is achieved.
First of all, we define the notion of non-interference on the operational semantics level.
We start by defining the \emph{trace} of a reduction step.
\begin{definition}[Trace of reduction]
	The trace $\mathcal{T}$ of a reduction step $\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}$ is a set of logging records for variable accesses:
  $\set{(x_1, p_1), \cdots, (x_n, p_n)}$.
  A record $(x, p)$ indicates $x_1$ is accessed at permission $p_1$,
  where $p$ could be either $\pRd{}$ or $\pWr{}$.

  We define the function $\fTrace{\cdot}$ to extract the trace from a derivation of reduction:
  \begin{equation*}
    \begin{split}
      &\fTrace{\reduction{\stDft{\tRead{x}}}{\st{\sta^\prime}{t}}} \quad &= \quad &\set{(x, \pRd{})} & \\
      &\fTrace{\reduction{\stDft{\tWrite{x}{y}}}{\st{\sta^\prime}{t}}} \quad &= \quad &\set{(x, \pWr{})} & \\
      &\fTrace{\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}} \quad &= \quad &\fTrace{\reduction{\stDft{u}}{\st{\sta^\prime}{u^\prime}}} &\quad\text{if there is a sub-derivation $\reduction{\stDft{u}}{\st{\sta^\prime}{u^\prime}}$} \\
      &\fTrace{\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}} \quad &= \quad &\varemptyset &\quad\text{otherwise} \\
    \end{split}
  \end{equation*}
  It is easily generalised to a series of reduction steps $\fTrace{t_1 \red \cdots \red t_n}$
  by taking the union of records at each step.
\end{definition}

We further define the notion of \emph{non-interference} between traces.
\begin{definition}[Non-Interfering Traces]
  The two traces $\mathcal{T}_0$ and $\mathcal{T}_1$ are considered non-interfering (written $\noninter{\mathcal{T}_0}{\mathcal{T}_1}$),
  iff there does not exist $x$ such that $(x, \pWr{}) \in \mathcal{T}_i$
  and $(x, p) \in \mathcal{T}_{1 - i}$.
\end{definition}


% We start by defining the relation $\mathcal{T} \sqsubseteq_{\G} F$,
% which states that the variables accessed in the trace $\mathcal{T}$ does not exceed the the footprint $F$.
% \begin{definition}[Variable Access Subsumption]
%   The subsumption $\mathcal{T} \sqsubseteq_{\G} F$ asserts that
%   the variables accessed in $\mathcal{T}$ do not exceed ones predicted in $F$ under the aliasing context described by $\G$.
% 	\begin{multicols}{3}
%     \infrule[elem]
%     {x^p \in F}
%     {\set{(x, p)} \sqsubseteq_{\G} F}

%     \infrule[var]
%     {x :_\epsilon \tCap{C}{S} \andalso C^p \sqsubseteq_\G F}
%     {\set{(x, p)} \sqsubseteq_{\G} F}

%     \infrule[set]
%     {\mathcal{T}_1 \sqsubseteq_\G F \andalso \mathcal{T}_2 \sqsubseteq_\G F}
%     {\mathcal{T}_1 \cup \mathcal{T}_2 \sqsubseteq_{\G} F}
%   \end{multicols}
% \end{definition}

\begin{definition}[Store query]
	We define the following store query operations:
  \begin{itemize}
  \item \emph{Immutable variable lookup.} $\sta(\tVal{x}) = v$ iff $\tVal{x} = v \in \sta$;
  \item \emph{Mutable variable lookup.} $\sta(\tVar{x}) = v$ iff $\sta = \sta_1, \tSet{x} = v, \sta_2$ and $\tSet{x} \notin \dom{\sta_2}$;
  \item \emph{Bound immutable variables.} $\bval{\sta} = \set{ x \ | \ \tVal{x} \mapsto v \in \sta }$;
  \item \emph{Bound mutable variables.} $\bvar{\sta} = \set{ x \ | \ \tVar{x} \mapsto v \in \sta }$.
  \end{itemize}
\end{definition}

\begin{definition}[Footprint on store]
  We define the footprint $\fClosure{\sta}{t}$ of term $t$ in the store $\sta$:
  \begin{equation*}
    \begin{split}
      &\fClosure{\sta, e}{x} \quad &= \quad &\set{x}, \quad &\text{if ${x} \in \bvar{\sta}$ or $x \in \dom{e}$}, \\
      &\fClosure{\sta, e}{x} \quad &= \quad &\fClosure{\sta, e}{\cv{v}}, \quad &\text{if $\sta(\tVal{x}) = v$}, \\
      &\fClosure{\sta, e}{x^?} \quad &= \quad &\set{x^?}, \quad &\text{if $x \in \bvar{\sta}$ and $x \in \dom{e}$}, \\
      &\fClosure{\sta, e}{x^?} \quad &= \quad &\fClosure{\sta, e}{\cv{v}^{??}}, \quad &\text{if $\sta(\tVal{x}) = v$}, \\
      &\fClosure{\sta, e}{*} \quad &= \quad &\set{*}, \quad &\\
      % &\fClosure{\sta, e}{*} \quad&= \quad &\set{*}, \quad & \\
      &\fClosure{\sta, e}{C_1 \cup C_2} \quad&= \quad &\fClosure{\sta, e}{C_1} \cup \fClosure{\sta, e}{C_2}. \quad & \\
    \end{split}
  \end{equation*}
\end{definition}

\begin{definition}[Authority]
	An authority $A$ in a store $\sta$ is a mapping $\bvar{\sta} \rightarrow \mathcal{P}$ from the mutable variables to the set of permissions.
  Here $\mathcal{P}$ denotes the powerset of $\set{\pRd, \pWr}$.
\end{definition}

\begin{definition}[Authority of Term]
	We define the authority of a term $\fAuth{e}{\sta}{\cv{t}}$ under a store $\sta$ and an evaluation context $e$ with
  \begin{equation*}
    \begin{split}
      &\fAuth{e}{\sta}{x} \quad &= \quad &[x \mapsto \varemptyset \ | \ x \in \bvar{\sta}] \circ [x \mapsto \set{\pWr{}}], \quad &\text{if ${x} \in \bvar{\sta}$}, \\
      &\fAuth{e}{\sta}{x} \quad &= \quad &\fAuth{e}{\sta}{\cv{v}}, \quad &\text{if $\sta(\tVal{x}) = v$}, \\
      &\fAuth{e}{\sta}{x} \quad &= \quad &\fAuth{e}{\sta}{\cv{t}}, \quad &\text{if $e(\tVal{x}) = t$}, \\
      &\fAuth{e}{\sta}{x^?} \quad &= \quad &[x \mapsto \varemptyset \ | \ x \in \bvar{\sta}] \circ [x \mapsto \set{\pRd{}}], \quad &\text{if $x \in \bvar{\sta}$}, \\
      &\fAuth{e}{\sta}{x^?} \quad &= \quad &\fAuth{e}{\sta}{\cv{v}^{??}}, \quad &\text{if $\sta(\tVal{x}) = v$}, \\
      &\fAuth{e}{\sta}{x^?} \quad &= \quad &\fAuth{e}{\sta}{\cv{t}^{??}}, \quad &\text{if $e(\tVal{x}) = t$}, \\
      % &\fAuth{e}{\sta}{*} \quad&= \quad &\set{*}, \quad & \\
      &\fAuth{e}{\sta}{C_1 \cup C_2} \quad&= \quad &\fAuth{e}{\sta}{C_1} \sqcup \fAuth{e}{\sta}{C_2}. \quad & \\
    \end{split}
  \end{equation*}
  Here, $\mathcal{A_1} \sqcup \mathcal{A_2}$ denotes the union of the two authorities,
  which unions the permissions for each variable, i.e.
  \begin{equation*}
    \mathcal{A}_1 \sqcup \mathcal{A}_2 = [x \mapsto A_1(x) \cup A_2(x) \ | \ x \in \dom{A_1} (= \dom{A_2}) ].
  \end{equation*}
\end{definition}

% \begin{definition}[Focusing on a footprint]
%   The focus $F \sqcap \mathcal{D}$ on a footprint is a subset of $F$ with only captured references on variables in $\mathcal{D}$.
% \end{definition}

\begin{definition}[Subauthority]
	An authority $A$ is considered a subauthority of $B$ (written $A \sqsubseteq B$),
  iff $\forall x \in \dom{B}, A(x) \subseteq B(x)$.
\end{definition}

\begin{definition}[Embedding of an authority]
	The embedding $\fEmbed{A}$ of an authority $A$ is the capture set corresponding to it.
  It is defined as:
  \begin{equation*}
    \fEmbed{A} = \bigcup_{x \in \dom{A}} \fEmbed{x \mapsto A(x)},
  \end{equation*}
  where
  \begin{equation*}
    \fEmbed{x \mapsto P} =
    \begin{cases}
      \set{x},  &\text{if $\pWr \in P$}, \\
      \set{x^?},  &\text{if $P = \set{\pRd}$}, \\
      \set{}, &\text{otherwise}. \\
    \end{cases}
  \end{equation*}
\end{definition}

\begin{definition}[Non-Interfering authorities]
	Two authorities $A_0$ and $A_1$ with the same domain $\mathcal{D} = \dom{A_0} = \dom{A_1}$ are non-interfering (written $\noninter{A_0}{A_1}$),
  iff there does not exist $x \in \mathcal{D}$, s.t. $\pWr \in A_i(x)$ and $A_{1-i} \ne \varemptyset$ ($i = 0,1$).
\end{definition}

\subsubsection{Properties of Typing and Reduction}


\begin{lemma}  \label{lemma:typ-unbox-inv-cs-val}
	If $\match{}{\sta}{\Delta}$,
  $\typ{\Delta}{\tUnbox{C}{x}}{T}$,
  $\sta(x) = \Box \ y$,
  $\sta(\tVal{y}) = v$,
  then $\sub{\Delta}{\cv{v}}{C}$.
\end{lemma}
\TODO{Admitted.}

\begin{lemma}  \label{lemma:footprint-subcapt-subset-flat}
  If $\match{}{\sta}{\Delta}$,
  $\sub{\Delta}{C_1}{C_2}$,
  $* \notin C_2$,
  $\fClosure{\sta}{C_1} \subseteq \fClosure{\sta}{C_2}$.
\end{lemma}

\begin{proof}
	\TODO{To be verified.}
\end{proof}

\begin{lemma}  \label{lemma:typ-unbox-inv-cs-var}
	If $\match{}{\sta}{\Delta}$,
  $\typ{\Delta}{\tUnbox{C}{x}}{T}$,
  $\sta(x) = \Box \ y$,
  $y \in \bvar{\sta}$,
  then $C = \set{y}$.
\end{lemma}
\TODO{Admitted.}

\begin{lemma}[Weakening of footprint]  \label{lemma:footprint-weakening}
  $\fClosure{\sigma}{C} = \fClosure{\sigma, \sigma^\prime}{C}$.
\end{lemma}
\TODO{Admitted.}
% \begin{proof}
% 	By induction on the size of $C$.
%   In each case we conclude immediately.
% \end{proof}

% \begin{lemma}[Lookup inversion: capture set]  \label{lemma:val-lookup-inv-cs}
% 	If
%   (i) $\match{}{\sta}{\Delta}$,
%   (ii) $\sta(\tVal{x}) = v$,
%   (iii) $\typ{\Delta}{x}{\tCap{C}{S}}$,
%   then $\sub{\Delta}{\cv{v}}{C}$.
% \end{lemma}
% \TODO{Admitted.}

\begin{lemma}[Typing strengthening]  \label{lemma:typ-strengthening}
  If $\typ{\G, x: T, \Delta}{t}{U}$,
  then
  (1) $x \notin \fv{t}$ implies $\typ{\G, \Delta}{t}{U}$;
  (2) $x \notin \fv{T}, \fv{U}$ implies $\sub{\G, \Delta}{T}{U}$;
  and (3) $x \notin \fv{C_1}, \fv{C_2}$ implies $\sub{\G, \Delta}{C_1}{C_2}$.
\end{lemma}
\begin{proof}
	By induction on the judgments.

  \emph{Case \textsc{var} for typing}.
  In this case, $t = y$, and $y : \tCap{C}{S} \in \G, x : T, \Delta$.
  Since $x \notin \fv{y} = \set{y}$, $x \neq y$.
  Therefore, $y : \tCap{C}{S} \in \G, \Delta$.
  We conclude by \textsc{var}.

  \emph{Case \textsc{sc-var} for subcapturing.}
  As above.

  \emph{Other cases.}
  We conclude by IH and the same rule.
\end{proof}

\begin{lemma}  \label{lemma:typ-ref-bvars}
	If $\match{}{\sta, e}{\Delta}$,
  and $\typ{\Delta}{x}{\tCap{C}{\tRef{S}}}$,
  then $x \in \bvar{\sta}$.
\end{lemma}
\TODO{Admitted.}

\begin{lemma}  \label{lemma:store-evctx-to-bang-binding}
	If (i) $\match{}{\sta, e}{\Delta}$
  and (ii) $x \in \bvar{\sta}$ or $x \in \dom{e}$,
  $x :_! \tCap{C}{S} \in \Delta$.
\end{lemma}

\begin{proof}
	By induction on the derivation of $\match{}{\sta, e}{\Delta}$.

  \emph{Case \textsc{grow-var}}.
  In this case, $\sta = \sta_0, \tVar{x} = v$ and $\Delta = \Delta_0, x :_! \tCap{\set{*}}{\tRef{S}}$.
  If $x = y$, we conclude immediately.
  Otherwise conclude by IH.

  \emph{Case \textsc{grow-ctx-par}}.
  As above.

  \emph{Case \textsc{empty}}.
  Absurd, since $\bvar{\sta} = \dom{e} = \varemptyset$ and $x \in \varemptyset$.

  \emph{Other cases.}
  By IH.
\end{proof}

\begin{lemma}  \label{lemma:bang-binding-to-store-evctx}
	If (i) $\match{}{\sta, e}{\Delta}$,
  and (ii) $x :_! T \in \Delta$,
  then either $x \in \bvar{\sta}$ or $x \in \dom{e}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of $\match{}{\sta, e}{\Delta}$.

  \emph{Case \textsc{empty}}.
  Absurd. In this case $\Delta = \cdot$ and $x :_! T \in \cdot$ is impossible.

  \emph{Case \textsc{grow-val}}.
  In this case, $\sta = \sta_0, \tVal{x} \mapsto v$ and $\Delta = \Delta_0, y :_\epsilon U$.
  We have $x \ne y$ and conclude by IH.

  \emph{Case \textsc{grow-set}, \textsc{grow-ctx-let} and \textsc{grow-ctx-var}}.
  By IH.

  \emph{Case \textsc{grow-var}}.
  In this case, $\sta = \sta_0, \tVar{y} = v$ and $\Delta = \Delta_0, y :_! \tCap{\set{*}}{\tRef{S}}$.
  If $x = y$ we conclude immediately. Otherwise we conclude by IH.

  \emph{Case \textsc{grow-ctx-par}}.
  As above.
\end{proof}

\begin{lemma}  \label{lemma:eps-binding-to-store}
  If (i) \match{}{\sta, e}{\Delta}
  and (ii) $x :_\epsilon T \in \Delta$
	then $x \in \bval{\sta}$.
\end{lemma}

\begin{proof}
  \TODO{as above}
\end{proof}

\begin{lemma}  \label{lemma:well-typed-cv}
	If $\typDft{t}{T}$,
  then $\cv{t} \subseteq \dom{\G}$.
\end{lemma}

\begin{proof}
	By induction on the derivation.

  \emph{Case \textsc{var}}. Conclude immediately.

  \emph{Other cases.} By IH.
\end{proof}

\begin{lemma}  \label{lemma:value-lookup-cv-depth}
  If (i) $\match{}{\sta, e}{\G}$
  and (ii) $\sta(\tVal{x}) = v$,
  then $\max_{\tau \in \cv{v}}{\fDepth{\G}{\tau}} < \fDepth{\G}{x}$.
\end{lemma}
\begin{proof}
	\TODO{admitted}
\end{proof}

\subsubsection{Properties of Authority}

\begin{lemma}[Commutativity of union]  \label{lemma:auth-union-comm}
	$\forall A_1, A_2. A_1 \sqcup A_2 = A_2 \sqcup A_1$.
\end{lemma}
\begin{proof}
	Trivial by the commutativity of set union.
\end{proof}

\begin{lemma}[Subauthority of union]  \label{lemma:subauth-union}
	$\forall A_1, A_2. A_1 \sqsubseteq A_1 \sqcup A_2$.
\end{lemma}
\begin{proof}
  We can show that for any $x$, $A_1(x) \subseteq (A_1 \sqcup A_2)(x) = A_1(x) \cup A_2(x)$
  and conclude.
\end{proof}

\begin{corollary}  \label{coro:subauth-union-r}
  $\forall A_1, A_2. A_2 \sqsubseteq A_1 \sqcup A_2$.
\end{corollary}
\begin{proof}
	By Lemma \ref{lemma:auth-union-comm} and \ref{lemma:subauth-union}.
\end{proof}

\begin{lemma}[Term authority is monotonic over subset]  \label{lemma:footprint-mono-subset}
	If $C_1 \subseteq C_2$,
  then $\fAuth{e}{\sta}{C_1} \subseteq \fAuth{e}{\sta}{C_2}$.
\end{lemma}
\begin{proof}
	% Trivial because $\fClosure{\sta}{\cdot}$ is homomorphic.
  We have $\fAuth{e}{\sta}{C_2} = \fAuth{e}{\sta}{C_1 \cup C_2} = \fAuth{e}{\sta}{C_1} \sqcup \fAuth{e}{\sta}{C_2}$,
  and conclude by Lemma \ref{lemma:subauth-union}.
\end{proof}

% \begin{fact}[Focus is monotonic over subset]  \label{lemma:focus-mono-subset}
% 	If $F_1 \subseteq F_2$,
%   then $F_1 \sqcap \mathcal{D} \subseteq F_2 \sqcap \mathcal{D}$.
% \end{fact}

% \begin{lemma}  \label{lemma:embed-auth-empty}
% 	If (1) $\match{}{\sta, e}{\Delta}$;
%   (2) $\sub{\Delta}{C}{\varemptyset}$;
%   and (3) $C \subseteq \dom{\sta}$,
%   then $\fEmbed{\fAuth{e}{\sta}{C}} = \varemptyset$.
% \end{lemma}

% \begin{proof}
% 	By induction on the subcapture derivation.

%   \emph{Case \textsc{sc-elem}}. Absurd since $x \in \varemptyset$.

%   \emph{Case \textsc{sc-set}}. By IH.

%   \emph{Case \textsc{sc-var}}.
%   In this case, $C = \set{x}$,
%   $x : \tCap{C_x}{S} \in \Delta$,
%   and $\sub{\Delta}{C_x}{\varemptyset}$.
%   If $x :_! T \in \Delta$,
%   we have $\sub{\Delta}{\set{*}}{\varemptyset}$ which is impossible.
%   Otherwise $x :_\epsilon \tCap{C_x}{S} \in \Delta$
% \end{proof}

\begin{lemma}  \label{lemma:subcapt-embed-auth-qq}
	If $\match{}{\sta}{\Delta}$,
  then $\sub{\Delta}{\fEmbed{\fAuth{e}{\sta}{C^{??}}}}{\fEmbed{\fAuth{e}{\sta}{C}}}$.
\end{lemma}

\begin{proof}
	By induction on $\fAuth{e}{\sta}{C}$.
  In each case we either conclude immediately or by IH.
\end{proof}

\begin{lemma}  \label{lemma:subcapt-qq}
	If $\subDft{C_1}{C_2}$,
  then $\subDft{C_1^{??}}{C_2^{??}}$.
\end{lemma}

\begin{proof}
	By induction on the subcapture derivation.

  \emph{Case \textsc{sc-var}}. Conclude by IH and \textsc{sc-var-$?$}.

  \emph{Case \textsc{sc-elem}}. By the same rule.

  \emph{Case \textsc{sc-set}}. By IH and the same rule.

  \emph{Case \textsc{sc-<:-$?$} and \textsc{sc-var-$?$}}. By IH.
\end{proof}

\begin{lemma}[Embedding of authority is monotonic over subcapture]  \label{lemma:footprint-mono-subcapt}
	If (1) $\match{}{\sta, e}{\Delta}$; (2) $\sub{\Delta}{C_1}{C_2}$;
  and (3) $C_1 \subseteq \dom{\sta}$ and $C_2 \subseteq \dom{\Delta}$,
  then $\G \vdash \fEmbed{\fAuth{e}{\sta}{C_1}} <: \fEmbed{\fAuth{e}{\sta}{C_2}}$.
\end{lemma}
\begin{proof}
  By induction on the lexical order $(\max_{\tau \in C} \fDepth{\Delta}{\tau}, | C |)$.
  % By induction on the subcapture derivation.

  \begin{itemize}
  \item When $\max_{\tau \in C} \fDepth{\Delta}{\tau} = 0$,
    we split the case of the derivation $\sub{\Delta}{C_1}{C_2}$.

    \emph{Case \textsc{sc-elem}}.
    Conclude by Lemma \ref{lemma:footprint-mono-subset}.

    \emph{Case \textsc{sc-set}}. By IH.

    \emph{Case \textsc{sc-var}}.
    In this case we have $C_1 = \set{x}$ and $x : \tCap{C_x}{S} \in \G$.
    Since $\fDepth{\G}{x} = 0$, by Lemma \ref{lemma:value-lookup-cv-depth} we know that
    $C_x$ is either empty, or $C_x = \set{*}$.
    If $x :_! \tCap{C_x}{S} \in \G$, we have $C_x = \set{*}$ and therefore $* \in C_2$, which is impossible.
    Otherwise $x :_\epsilon \tCap{C_x}{S}$.
    If $C_x$ is empty, we conclude immediately since $\fEmbed{\fAuth{e}{\sta}{C_1}} = \varemptyset$.
    Otherwise it is absurd.

    \emph{Case \textsc{sc-var-$?$}}.
    As above.

    \emph{Case \textsc{sc-$<:$-$?$}}.
    By Lemma \ref{lemma:subcapt-embed-auth-qq}, IH and the transitivity of subcapturing.

  \item When $\max_{\tau \in C} \fDepth{\Delta}{\tau} = k$ and $k > 0$.
    We again split the cases of $\sub{\G}{C_1}{C_2}$.

    \emph{Case \textsc{sc-elem}}.
    In this case, $C_1 = \set{x}$ and $x \in C_2$.
    We have $C_1 \subseteq C_2$ and conclude by Lemma \ref{lemma:footprint-mono-subset}.

    \emph{Case \textsc{sc-set}}. By IH.

    \emph{Case \textsc{sc-var}}.
    In this case,
    $C_1 = \set{x}$,
    $x : \tCap{C_x}{S} \in \G$,
    and $\sub{\G}{C_x}{C_2}$.
    By IH we have $\sub{\G}{\fEmbed{\fAuth{e}{\sta}{C_x}}}{\fEmbed{\fAuth{e}{\sta}{C_2}}}$.
    If $x :_! \tCap{C_x}{S} \in \Delta$,
    $\fEmbed{\fAuth{e}{\sta}{C_1}} = \set{x}$.
    We conclude by \textsc{sc-var} and IH.
    Otherwise, if $x :_\epsilon \tCap{C_x}{S} \in \Delta$,
    we invoke Lemma \ref{lemma:eps-binding-to-store} and show that $x \in \bval{\sta}$.
    Therefore, $\sta(\tVal{x}) = v$ for some $v$.
    $\fEmbed{\fAuth{e}{\sta}{C_1}} = \fEmbed{\fAuth{e}{\sta}{\cv{v}}}$.
    By Lemma \ref{lemma:value-lookup-cv-depth} we have $\max_{\tau \in \cv{v}}{\fDepth{\Delta}{\tau}} < \fDepth{\Delta}{x}$,
    we can therefore invoke IH and conclude.

    \emph{Case \textsc{sc-var-$?$}}. As above and make use of Lemma \ref{lemma:subcapt-qq}.

    \emph{Case \textsc{sc-$<:$-$?$}}.
    In this case, $C_1 = \set{x^{?}}$,
    by IH we have $\sub{\Delta}{\fEmbed{\fAuth{e}{\sta}{\set{x}}}}{\fEmbed{\fAuth{e}{\sta}{C}}}$.
    By Lemma \ref{lemma:subcapt-embed-auth-qq} we have $\sub{\Delta}{\fEmbed{\fAuth{e}{\sta}{\set{x^{?}}}}}{\fEmbed{\fAuth{e}{\sta}{\set{x}}}}$ and we conclude by the transitivity of subcapturing.
  \end{itemize}
\end{proof}

\subsubsection{Lenient Bindings}

Now we develop the theory of lenient bindings in evaluation contexts.

\begin{definition}[Effective domain]
	The effective domain of an evaluation context $e$
  is the set of bindings that is counted in $\cv{\cdot}$.
  Specifically, it is given by the following rules:
  \begin{equation*}
    \begin{split}
      &\domE{{\tLetPar{x}{v}{e}}}{t} \quad &= \quad &\domE{e}{t}, \quad &\text{if $x \notin \cv{\ctx{e}{t}}$}, \\
      &\domE{{\tLetPar{x}{u}{e}}}{t} \quad &= \quad &\set{x} \cup \domE{e}{t}, \quad &\text{otherwise}, \\
      &\domE{{\tLetBoth{x}{e}{u}}}{t} \quad &= \quad &\domE{e}{t}, \quad &\text{} \\
      &\domE{{\tLetVar{x}{e}{u}}}{t} \quad &= \quad &\domE{e}{t}. \quad &\text{} \\
    \end{split}
  \end{equation*}
\end{definition}

\begin{definition}[Exclusive dependency]
  Given an evaluation context $e$ and the focused term $t$,
  the exclusive dependencies $\fDep{e, t}{x}$ of the lenient binding $x$ is defined as:
  \begin{equation*}
    \fDep{e, t}{x} = \set{ y \ | \ y \in \domE{e}{t} \wedge e(y) = t_y \wedge x \in \cv{t_y} }.
  \end{equation*}
  % We define $\fDepN{0}{e, t}{x} = \set{x}$, $\fDepN{k+1}{e, t}{x} = \fDep{e, x}{\fDepN{k}{e, t}{x}}$,
  % and $\fDepN{*}{e, t}{x} = \bigcup_{i=0}^{\infty} {\fDepN{i}{e, t}{x}}$.
\end{definition}

\begin{definition}[Shared dependency]
  Given the evaluation context $e$ and the focused term $t$,
  the shared dependencies $\fDepS{e, t}{x}$ of the lenient binding $x$ is defined as:
  \begin{equation*}
    \fDepS{e, t}{x} = \set{ y \ | \ y \in \domE{e}{t} \wedge e(y) = t_y \wedge x^{?} \in \cv{t_y} }.
  \end{equation*}
\end{definition}

\begin{lemma}  \label{lemma:evctx-cv}
  If $t$ is not a value,
	then $\cv{t} \subseteq \evctx{t}$.
\end{lemma}

\begin{proof}
	By induction on $e$.
\end{proof}

\begin{lemma}[Single exclusive dependency]  \label{lemma:lazy-binding-single-dep}
	Given an evaluation context $e$ and a focused term $t$,
  if $\match{}{\sta, e}{\Delta_1, \Delta_2}$ ($\dom{\Delta_1} = \dom{\sta}$ and $\dom{\Delta_2} = \dom{e}$),
  and $\typ{\Delta_1}{\evctx{t}}{T}$ then $\forall x. | \fDep{e, t}{x} | \le 1$.
\end{lemma}

\begin{proof}
  Proof by contradiction.
  Proceed by assuming that $| \fDep{e, t}{x} | \ge 2$,
  which implies that there exists $x_i, x_j \in \domE{e}{t}$ and $t_i = e(x_i)$, $t_j = e(t_j)$, s.t.
  $x \in \cv{t_i}$ and $x \in \cv{t_j}$.
  The evaluation context could be written in the form $e = \ctx{e_1}{\tLetPar{x_i}{t_i}{\ctx{e_2}{\tLetPar{x_j}{t_j}{e_3}}}}$.
  From $\typ{\Delta_1}{\evctx{t}}{T}$
  we could show that $\ninter{\Delta_1, \Delta_2}{\cv{t_i}}{\cv{\ctx{e_2}{\tLetPar{x_j}{t_j}{e_3[t]}}/x_i}}$.
  We have $x \in \cv{t_i}$
  and $x \in \cv{\tLetPar{x_j}{t_j}{e_3[t]}} \subseteq \cv{\ctx{e_2}{\tLetPar{x_j}{t_j}{e_3[t]}}}$ (by Lemma \ref{lemma:evctx-cv}).
  Therefore we show that $\fClosure{\Delta_1, \Delta_2}{\cv{\tLetPar{x_j}{t_j}{e_3[t]}}} \cap \fConflict{\Delta_1, \Delta_2}{\fConflict{\Delta_1, \Delta_2}{\cv{\ctx{e_2}{\tLetPar{x_j}{t_j}{e_3[t]}}}}} \ne \varemptyset$
  and derive a contradiction.
\end{proof}

\begin{lemma}[Exclusive dependency forbids shared ones]  \label{lemma:exclusive-dep-no-shared}
	Given an evaluation context $e$ and a focused term $t$,
  if $\match{}{\sta, e}{\Delta_\sta, \Delta_e}$ and $\typ{\Delta_\sta}{\evctx{t}}{T}$,
  then $\fDep{e, t}{x} \ne varemptyset$ implies $\fDepS{e, t}{x} = \varemptyset$.
\end{lemma}

\begin{proof}
	If $\fDep{e, t}{x} \ne \varemptyset$,
  then exists $y_i$ s.t. $\fDep{e, t}{x}$ and in other words $x \in \cv{e(y_i)}$.
  If $\fDepS{e, t}{x} \ne \varemptyset$ we also have $x^{?} \in \cv{e(y_j)}$.
  Then $e$ could be written in the form of
  either $\ctx{e_1}{\tLetPar{y_i}{t_i}{\ctx{e_2}{\tLetPar{y_j}{t_j}{e_3}}}}$
  or $\ctx{e_1}{\tLetPar{y_j}{t_j}{\ctx{e_2}{\tLetPar{y_i}{t_i}{e_3}}}}$.
  In both case we derive an contradiction on the non-interfering condition.
\end{proof}

\begin{lemma}[Menationable lenient bindings]
	Given an evaluation context $e$ and a focused term $t$ (and $t$ is not a value),
  if (i) $\match{}{\sta, e}{\Delta_\sta, \Delta_e}$
  (ii) $\typ{\Delta_\sta}{\evctx{t}}{T}$,
  and (iii) $x \in \fv{t}$,
  then $\fDep{e, t}{x} = \fDepS{e, t}{x} = \varemptyset$.
\end{lemma}

\begin{proof}
  Proof by contradiction.
  If $\fDep{e, t}{x} = \set{x_i}$.
  The evaluation context could be written in the form of
  $e = \ctx{e_1}{\tLetPar{x_i}{t_i}{e_2}}$.
  Since the term is well-typed we can show that $\ninter{\Delta_1, \Delta_2}{\cv{t_i}}{\cv{\ctx{e_2}{t}}/x}$
  and we derive a contradiction when $x \in \fv{t}$.
  In the same way we prove $\fDepS{e, t}{x} = \varemptyset$.
\end{proof}

% \begin{lemma}[Mentionable dependency]
% 	Given an evaluation context $e$ and a focused term $t$ (and $t$ is not a value), for given any $x$,
%   there is at most one $y$ s.t. $y \in \fDepN{*}{e, t}{x}$ and $\fDep{e, t}{y} = \varemptyset$.
% \end{lemma}

% \begin{proof}
%   Proof by contradiction.
%   Assuming that there exists $y_1, y_2$ that meet the conditions.
%   From $y_i \in \fDepN{*}{e, t}{x}$ we can derive that
%   $y_1 \in \fDepN{i}{e, t}{x}$ and $y_2 \in \fDepN{j}{e, t}{x}$ for some $i$ and $j$.
%   Without the loss of generality we assume that $i < j$ (and $i = j$ is impossible according to Lemma \ref{lemma:lazy-binding-single-dep}).
%   Since $\fDepN{i}{e, t}{x} = \set{x}$ we have $\fDepN{j}{e, t}{x} = \varemptyset$
%   and derive a contradiction.
% \end{proof}

% \begin{definition}[Reachable lazy bindings]
%   Given the evaluation context $e$ and the focused term $t$,
%   we define the reachable lazy bindings $\fReachLazy{e, t}{x}$
%   as $\fReachLazy{e, t}{x} = \set{ y \ | \ x \in \fDepN{*}{e, t}{y} }$.

%   It is extended to sets via $\fReachLazy{e, t}{C} = \bigcup{x \in C \cap \domE{e}{t}} \fReachLazy{e, t}{x}$.
% \end{definition}

% \begin{lemma}  \label{lemma:reach-lenient-decompose}
%   Given the evaluation context $e$ and the focused term $t$,
%   for any variable $x \in \dom{e}$,
%   we have $\fReachLazy{e, t}{x} = \set{x} \cup \bigcup_{y \in \cv{e(x)} \cap \dom{e}} \fReachLazy{e, t}{y}$.
% \end{lemma}

% \begin{proof}
% 	For any $y \in \fReachLazy{e, t}{x}$,
%   we have $x \in \fDepN{*}{e, t}{y}$.
%   Either $y = x$,
%   or $\exists z. x \in \fDep{e, t}{z}$,
%   which implies that $z \in \cv{e(x)}$.
%   We therefore conclude.
% \end{proof}

\begin{definition}[Reachable lenient bindings]
  Given an evaluation context $e$ and the focused term $t$,
  the lenient bindings reachable from $x$, written $\fReachLazy{e, t}{x}$,
  is defined as the following:
  \begin{equation*}
    \fReachLazy{e, t}{x} = \set{ y \ | \ x \in \fDep{e, t}{y} } \cup \set{ y^{?} \ | \ x \in \fDepS{e, t}{y} }.
  \end{equation*}

  We define
  $\fReachLazy{e, t}{x^{?}} = \left( \fReachLazy{e, t}{x} \right)^{??}$,
  $\fReachLazyN{0}{e, t}{\tau} = \set{\tau}$,
  $\fReachLazyN{i+1}{e, t}{\tau} = \fReachLazy{e, t}{\fReachLazyN{i}{e, t}{\tau}}$,
  and $\fReachLazyN{*}{e, t}{\tau} = \bigcup_{i=0}^\infty \fReachLazyN{i}{e, t}{\tau}$.
\end{definition}

\begin{lemma}  \label{lemma:reach-to-dep-seq}
	If $x \in \fReachLazyN{k}{e, t}{y}$,
  there exists a sequence $x_0, \cdots, x_k$
  such that
  (i) $x = x_0$,
  (ii) $x_k = y$,
  and (iii) $\forall i, x_{i+1} \in \fDep{e, t}{x_i}$.
\end{lemma}

\begin{proof}
	By induction on $k$.
\end{proof}

\begin{lemma}  \label{lemma:exc-dep-seq-subseq}
  Given the store $\sta$, the evaluation context $e$ and the focused term $t$,
	If (i) $\match{}{\sta, e}{\Delta_\sta, \Delta_e}$,
  (ii) $\typ{\Delta_\sta}{\evctx{t}}{T}$,
  and for a lenient binding $x \in \domE{e}{t}$ there are two sequences
  $x_0, \cdots, x_k$ and $y_0, \cdots, y_l$ ($x_0 = y_0 = x$)
  such that $\forall i, x_{i+1} \in \fDep{e, t}{x_i}$ and the same for $y_i$,
  and $\fDep{e, t}{x_k} = \varemptyset$,
  then $y_0, \cdots, y_l$ is a subsequence of $x_0, \cdots, x_k$.
\end{lemma}

\begin{proof}
  First, we show that $\forall i = 0, \cdots, \min(k, l). x_i = y_i$.
  $x_0 = y_0$ holds trivially.
  For any $i = j + 1$, we have $x_j = y_j$ by IH.
  If $x_j \ne y_j$ we have $| \fDep{e, t}{x_i} | \ge 2$,
  from which a contradiction is derived by Lemma \ref{lemma:lazy-binding-single-dep}.

  Next, we show that $l \le k$.
  If $k < l$, we have $x_{k+1} \in \fDep{e, t}{x_k} = \varemptyset$ which is contradictory.
  % The same contradiction can be derived for the case of $k > l$.
  % We therefore conclude the proof.
\end{proof}

\begin{corollary}  \label{lemma:exc-dep-seq-eqseq}
  Given the store $\sta$, the evaluation context $e$ and the focused term $t$,
	If (i) $\match{}{\sta, e}{\Delta_\sta, \Delta_e}$,
  (ii) $\typ{\Delta_\sta}{\evctx{t}}{T}$,
  and for a lenient binding $x \in \domE{e}{t}$ there are two sequences
  $x_0, \cdots, x_k$ and $y_0, \cdots, y_l$ ($x_0 = y_0 = x$)
  such that $\forall i, x_{i+1} \in \fDep{e, t}{x_i}$ and the same for $y_i$,
  and $\fDep{e, t}{x_k} = \fDep{e, t}{y_l} = \varemptyset$,
  then $y_0, \cdots, y_l$ and $x_0, \cdots, x_k$ are identical.
\end{corollary}

\begin{lemma}  \label{lemma:reach-q-to-dep-seq}
	If $x^{?} \in \fReachLazyN{k}{e, t}{y}$,
  there exists a sequence $x_0, \cdots, x_k$
  such that
  (i) $x = x_0$,
  (ii) $x_k = y$,
  and (iii) $\forall i, x_{i+1} \in \fDep{e, t}{x_i} \cup \fDepS{e, t}{x_i}$
  and there exists at least one $i$ such that $x_{i+1} \in \fDepS{e, t}{x_i}$.
\end{lemma}

\begin{proof}
  By induction on $k$.
\end{proof}

\begin{lemma}  \label{lemma:reach-qq-to-dep-seq}
	If $x^{?} \in \fReachLazyN{k}{e, t}{y^{?}}$,
  there exists a sequence $x_0, \cdots, x_k$
  such that
  (i) $x = x_0$,
  (ii) $x_k = y$,
  and (iii) $\forall i, x_{i+1} \in \fDep{e, t}{x_i} \cup \fDepS{e, t}{x_i}$.
\end{lemma}

\begin{proof}
  We have $x^{?} \in {\fReachLazyN{k}{e, t}{y}}^{??}$,
  from which we know that $x \in \fReachLazyN{k}{e, t}{y}$ or $x^{?} \in \fReachLazyN{k}{e, t}{y}$.
  We conclude by Lemma \ref{lemma:reach-to-dep-seq} and Lemma \ref{lemma:reach-q-to-dep-seq}.
\end{proof}

\begin{lemma}  \label{lemma:lenient-bindings-ninter}
	If (i) $\match{}{\sta, e}{\Delta_1, \Delta_2}$,
  (ii) $\dom{\Delta_1} = \dom{\sta}$ and $\dom{\Delta_2} = \dom{e}$,
  and (iii) $\typ{\Delta_1}{\evctx{t}}{T}$,
  then for any $x, y \in \domE{e}{t}$ ($x \ne y$),
  we have $\ninter{\Delta_1, \Delta_2}{\cv{e(x)}/y}{\cv{e(y)}/x}$.
\end{lemma}

\TODO{admitted}

\begin{definition}[Non-interfering lenient bindings]
  Two sets of lenient bindings $L_1$ and $L_2$ are non-interfering (written $\ninterLB{L_1}{L_2}$),
  iff there does not exist $x \in L_1$ such that $x^* \in L_2$.
\end{definition}

\subsubsection{Non-Interference Lemma}

\begin{lemma}[Preservation of variable authority]  \label{lemma:authority-pres-principal}
	If
  (i) $\match{}{\sta, e}{\Delta}$,
  (ii) $\typ{\Delta}{t}{T}$,
  (iii) $\reduction{\stDft{\evctx{t}}}{\st{\sta^\prime}{\evctx{t^\prime}}}$,
  and $e$ is the principal evaluation context of the reduction,
  % then given $\mathcal{D} \subseteq \bvar{\sta}$,
  then
  $\fAuth{e}{\sta^\prime}{\cv{t^\prime}} \sqsubseteq \fAuth{e}{\sta}{\cv{t}}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the judgment.

  \emph{Case \textsc{apply}}.
  In this case $t = x\,y$,
  $\sta(\tVal{x}) = \lambda(z: T) s$,
  $\sta^\prime = \sta$,
  and $t^\prime = [y/z] s$.
  % Therefore,
  $\fAuth{e}{\sta}{\cv{t}} = \fAuth{e}{\sta}{\set{x, y}} = \fAuth{e}{\sta}{\cv{s}/z} \sqcup \fAuth{e}{\sta}{y}$.
  On the other hand,
  $\fAuth{e}{\sta}{\cv{[y/z] s}} = \fAuth{e}{\sta}{[y/z]\cv{s}}$.
  We have $[y/z]\cv{s} \subseteq \cv{s}/z \cup \set{y}$.
  By Lemma \ref{lemma:footprint-mono-subset},
  we have $\fAuth{e}{\sta}{[y/z]\cv{s}} \sqsubseteq \fAuth{e}{\sta}{\cv{s}/z \cup \set{y}} = \fAuth{e}{\sta}{\cv{s}/z} \sqcup \fAuth{e}{\sta}{y}$.
  We therefore show that $\fAuth{e}{\sta}{{\cv{t^\prime}}} \sqsubseteq \fAuth{e}{\sta}{\cv{t}}$ and conclude.
  % We conclude by Lemma \ref{lemma:focus-mono-subset}.

  \emph{Case \textsc{tapply}}. As above.

  % \emph{Case \textsc{tapply}}.
  % In this case $t = x[S]$,
  % $\sta(\tVal{x}) = \lambda[X <: S^\prime] s$,
  % $\sta^\prime = \sta$,
  % $t^\prime = [S/X] s$.
  % Note that $\cv{[S/X] s} = \cv{s} = \cv{t}$.
  % We conclude by Lemma \ref{lemma:focus-mono-subset}.

  \emph{Case \textsc{open}}.
  In this case $t = \tUnbox{C}{x}$,
  $\sta(\tVal{x}) = \Box{}\ y$,
  $t^\prime = y$,
  and the $\sta$ stays unchanged.
  $\cv{t} = C \cup \set{x}$
  and $\cv{t^\prime} = \set{y}$.
  % We inspect the derivation of $\typ{\Delta}{t}{T}$:
  % it starts with an \textsc{unbox} rule,
  % followed by a series of \textsc{sub} rule.
  % By induction on the number of \textsc{sub} rules,
  % we can show that $\typ{\Delta}{x}{\Box \ \tCap{C_x}{S_x}}$ where $\sub{\Delta}{C_x}{C}$ $\sub{\Delta}{S_x}{T}$.
  % By Lemma \ref{lemma:lookup-box-inv} we have $\typ{\Delta}{y}{\tCap{C_x}{S_x}}$.
  If $y \in \bval{\sta}$, and $\sta(\tVal{y}) = v$,
  we invoke Lemma \ref{lemma:typ-unbox-inv-cs-val},
  and show that $\sub{\Delta}{\cv{v}}{C}$.
  By Lemma \ref{lemma:footprint-subcapt-subset-flat},
  we have $\fAuth{e}{\sta}{\cv{v}} \sqsubseteq \fAuth{e}{\sta}{C}$.
  Note that $\fAuth{e}{\sta}{t^\prime} = \fAuth{e}{\sta}{\cv{v}}$ and
  $\fAuth{e}{\sta}{\cv{t}} = \fAuth{e}{\sta}{C} \sqcup \fAuth{e}{\sta}{x} = \fAuth{e}{\sta}{C}$.
  We therefore conclude this sub-case.
  Otherwise, $y \in \bvar{\sta}$.
  In this case $\fAuth{e}{\sta}{\cv{t}} = \fAuth{e}{\sta}{\cv{t^\prime}}$.

  \emph{Case \textsc{let-value}}.
  In this case, $t = \tLetBoth{x}{v}{s}$,
  $\sta^\prime = \sta, \tVal{x} \mapsto v$,
  and $t^\prime = s$.
  We have $\cv{t} = [x\mapsto \cv{v}]\cv{s}$,
  and $\cv{t^\prime} = \cv{s}$.
  If $x \notin \cv{s}$,
  we have $\cv{t} = \cv{t^\prime}$ and conclude.
  Otherwise if $x \in \cv{s}$,
  note that $\cv{s} = \cv{s}/x \cup \set{x}$,
  and $[x\mapsto \cv{v}]\cv{s} = \cv{s}/x \cup \cv{v}$.
  By Lemma \ref{lemma:footprint-weakening} we have $\fAuth{e}{\sta^\prime}{\cv{t^\prime}} = \fAuth{e}{\sta}{\cv{s}/x} \sqcup \fAuth{e}{\sta^\prime}{\cv{v}}$ and conclude.

  \emph{Case \textsc{rename}}. As above.

  \emph{Case \textsc{var-value}}.
  In this case, $t = \tLetVar{x}{v}{s}$,
  $\sta^\prime = \sta, \tVar{x} \mapsto v$,
  and $t^\prime = s$.
  We have $\cv{t} = \cv{v} \cup \cv{s}/x$,
  and $\cv{t^\prime} = \cv{s}$.
  If $x \notin \cv{s}$, we have $\cv{t^\prime} \subseteq \cv{t}$ and conclude immediately by Lemma \ref{lemma:footprint-mono-subset}.
  Otherwise if $x \in \cv{s}$,
  $\cv{t} = \cv{s}/x \cup \cv{v}$,
  $\cv{t^\prime} = \cv{s}/x \cup \set{x}$.
  Therefore,
  $\fAuth{e}{\sta^\prime}{\cv{t^\prime}} \sqsubseteq \fAuth{e}{\sta^\prime}{\cv{s}/x} \circ [\set{x} \mapsto \set{\pRd, \pWr}]$.
  Therefore,
  we have $\fAuth{e}{\sta^\prime}{\cv{t^\prime}} \sqsubseteq \fAuth{e}{\sta^\prime}{\cv{s}/x}$ and conclude.
  % Since $x \notin \bvar{\sta}$, $\fClosure{\sta^\prime}{\cv{t^\prime}} \sqcap \mathcal{D} = \fClosure{\sta^\prime}{\cv{t^\prime}/x} \sqcap \mathcal{D}$.
  % We conclude by Lemma \ref{lemma:footprint-weakening} and Lemma \ref{lemma:footprint-mono-subset}.

  \emph{Case \textsc{lookup}}.
  As above.

  \emph{Case \textsc{lift-set}}.
  In this case,
  $t = \tWrite{x}{y}$,
  $\sta(\tVal{y}) = v$,
  $\sta^\prime = \sta, \tSet{x} = v$,
  and $t^\prime = v$.
  By inverting the judgment $\typ{\Delta}{\tWrite{x}{y}}{T}$,
  we will see it starts with a \textsc{write} rule,
  followed by a series of \textsc{sub} rules.
  Therefore we have $\typ{\Delta}{y}{S_0}$ and $\sub{\Delta}{S_0}{T}$.
  By Lemma \ref{lemma:value-lookup-inv-cs}
  we can show that $\sub{\Delta}{\cv{v}}{\varemptyset}$.
  By Lemma \ref{lemma:footprint-mono-subcapt} we have
  $\sub{\Delta}{\llbracket \fAuth{e}{\sta}{\cv{v}} \rrbracket}{\llbracket \fAuth{e}{\sta}{\varemptyset} \rrbracket}$.
  From this, we can show that $\fEmbed{\fAuth{e}{\sta}{\cv{v}}} = \varemptyset$,
  and therefore $\fAuth{e}{\sta}{\cv{v}} = [x \mapsto \varemptyset \ | \ x \in \bvar{\sta}]$.
  By Lemma \ref{lemma:footprint-weakening},
  we have $\fAuth{e}{\sta^\prime}{\cv{t^\prime}} = [x \mapsto \varemptyset \ | \ x \in \bvar{\sta^\prime}]$ and therefore conclude.

  \emph{Case \textsc{read}}. As above.

  % \emph{Case \textsc{let-ctx}}. By IH.

  % \emph{Case \textsc{let-par}}.
  % In this case
  % $t = \tLetPar{x}{s}{u}$,
  % and $\typ{\Delta}{t}{T}$.
  % To invoke IH we have to show that $\typ{\Delta}{u}{U}$ for some $U$.
  % By inspecting the derivation of $\typ{\Delta}{t}{T}$
  % we can show that $\typ{\Delta, x: U_1}{u}{U_0}$ for some $U_0$.
  % Now invoke Lemma \ref{lemma:typ-strengthening} to show that $\typ{\Delta}{u}{U_0}$.
  % Now we conclude by IH.
\end{proof}

\begin{lemma}  \label{lemma:evctx-structure}
	If $\ctx{e_1}{t_1} = \ctx{e_2}{t_2}$,
  then one of the following holds:
  (1) $e_1$ is part of $e_2$, i.e. $t_1 = \ctx{e}{t_2}$ and $\ctx{e_1}{e} = e_2$;
  (2) $e_2$ is part of $e_1$, i.e. $t_2 = \ctx{e}{t_1}$ and $\ctx{e_2}{e} = e_1$;
  (3) $e_1$ and $e_2$ diverges, i.e.
  $\ctx{e_1}{t_1} = \ctx{e}{\tLetPar{x}{\ctx{e_1^\prime}{t_1}}{\ctx{e_2^\prime}{t_2}}} = \ctx{e_2}{t_2}$
  or $\ctx{e_1}{t_1} = \ctx{e}{\tLetPar{x}{\ctx{e_2^\prime}{t_2}}{\ctx{e_1^\prime}{t_1}}} = \ctx{e_2}{t_2}$.
\end{lemma}

\begin{proof}
	By induction on $\min{(| e_1 |, | e_2 |)}$.

  \emph{When $e_1 = []$.}
  The case (1) holds,
  since $t_1 = \ctx{e_2}{t_1}$ and $\ctx{e_1}{e_2} = e_2$.

  \emph{When $e_2 = []$}. As above.

  \emph{When $e_1 = \tLet{x}{e_1^\prime}{s}$}.
  Because of the equality, $e_2 = \tLet{x}{e_2^\prime}{s}$ for some $e_2^\prime$.
  We invoke IH and in each case we conclude.

  \emph{When $e_1 = \tLetVar{x}{e_1^\prime}{s}$}. As above.

  \emph{When $e_1 = \tLetBoth{x}{e_1^\prime}{s}$}.
  If $e_2 = \tLetBoth{x}{e_2^\prime}{s}$, we invoke IH and conclude.
  Otherwise, $e_2 = \tLetBoth{x}{u}{e_2^\prime}$.
  We therefore show case (3) and conclude.

  \emph{When $e_1 = \tLetBoth{x}{u}{e_1^\prime}$}.
  As above.
\end{proof}

\begin{lemma}
	If
  (i) $\match{}{\sta, e}{\Delta}$,
  (ii) $\typ{\Delta}{t}{T}$,
  (iii) $\reduction{\stDft{\ctx{e_1}{\ctx{e_2}{t}}}}{\st{\sta^\prime}{\ctx{e_1}{\ctx{e_2}{t^\prime}}}}$,
  and $\ctx{e_1}{e_2}$ is the principal evaluation context of the reduction,
  % then given $\mathcal{D} \subseteq \bvar{\sta}$,
  then
  $\fAuth{e_1}{\sta^\prime}{\cv{\ctx{e_2}{t^\prime}}} \sqsubseteq \fAuth{e_1}{\sta}{\cv{\ctx{e_2}{t}}}$.
\end{lemma}

\begin{proof}
  By induction on the structure of $e_2$.

  \emph{Case $e_2 = []$}.
  Conclude by Lemma \ref{lemma:authority-pres-principal}.

  \emph{Case $e_2 = \tLet{x}{e_2^\prime}{s}$}.
  \TODO{Continue here.}
\end{proof}

\begin{lemma}[Preservation of Authority]  \label{lemma:authority-pres}
	If
  (i) $\match{}{\sta, e}{\Delta}$,
  (ii) $\typ{\Delta}{t}{T}$,
  (iii) $\reduction{\stDft{\ctx{e}{t}}}{\st{\sta^\prime}{\ctx{e^\prime}{t^\prime}}}$,
  then
  $\fAuth{e^\prime}{\sta^\prime}{\cv{t^\prime}} \sqsubseteq \fAuth{e}{\sta}{\cv{t}}$.
\end{lemma}

\begin{lemma}  \label{lemma:wf-store-var-defined}
	If (i) $\match{}{\sta}{\Delta}$,
  and (ii) $\sta(\tVar{x}) = v$,
  then $x \in \bvar{\sta}$.
\end{lemma}
\TODO{Admitted.}

\begin{lemma}[Trace is bounded by footprint]
	If
  (1) $\match{}{\sta}{\Delta}$,
  (2) $\typ{\Delta}{t}{T}$,
  (3) $\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}$;
  (4) $\mathcal{T} = \fTrace{\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}}$;
  (5) $F = \fClosure{\sta}{\cv{t}}$,
  then $\mathcal{T} \sqsubseteq F$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the reduction.

  \emph{Case \textsc{read}}.
  In this case, $\mathcal{T} = \set{(x, \pRd{})}$,
  and $\sta(\tVar{x}) = v$.
  By Lemma \ref{lemma:wf-store-var-defined},
  we show that $x \in \bvar{\sta}$.
  Therefore, $F = \fClosure{\sta}{x^?} = \set{x^?}$ and we conclude.

  \emph{Case \textsc{write}}.
  In this case, $t = \tWrite{x}{y}$,
  and $\mathcal{T} = \set{(x, \pWr{})}$.
  By inspecting the derivation of $\typ{\Delta}{t}{T}$,
  we can show that $\typ{\Delta}{x}{\tCap{C_0}{\tRef{S_0}}}$.
  By Lemma \ref{lemma:typ-ref-bvars} we show that $x \in \bvar{\sta}$. \TODO{reduction rules are updated.}
  Therefore, $F = \set{x}$ and we conclude.

  \emph{Case \textsc{let-ctx} and \textsc{let-par}}.
  In these cases, we invert the typing judgment, invoke the IH and conclude.

  \emph{Other cases.}
  In other cases we have $\mathcal{T} = \varemptyset$ and therefore conclude immediately.
\end{proof}

Now we start defining the \emph{non-interference} when evaluating the parallel-let bindings.
\begin{definition}[Tracing parallel-let evaluation]
	Given a series of reduction
  $\st{\sta}{t} \redt \st{\sta^\prime}{t^\prime}$,
  we define the left-trace of evaluating the parallel-let binding labelled with $x$ as:
  \begin{equation*}
    \begin{split}
      &\fTraceX{(x, L)}{{(\st{\sta}{t} \redt \st{\sta^\prime}{t^\prime})} \red (\st{\sta^\prime}{t^\prime} \redt \st{\sta^{\prime\prime}}{t^{\prime\prime}})} \quad &= \quad &\fTraceX{(x, L)}{\st{\sta}{t} \redt \st{\sta^\prime}{t^\prime}} \\
      & \quad &\cup \quad &\fTraceX{(x, R)}{\st{\sta^\prime}{t^\prime} \redt \st{\sta^{\prime\prime}}{t^{\prime\prime}}} \\
      &\fTraceX{(x, L)}{\reduction{\stDft{\tLetPar{x}{t}{u}}}{\st{\sta^\prime}{\tLetPar{x}{t^\prime}{u}}}} \quad &= \quad &\fTrace{\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}} \\
      &\fTraceX{(x, L)}{\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}} \quad &= \quad & \varemptyset \\
    \end{split}
  \end{equation*}

  And we similarly define the right-trace.
\end{definition}

\begin{definition}[Non-interference of footprint]
  $\ninterf{\Delta}{F_1}{F_2}$ iff $\fConflict{\Delta}{F_1} \cap F_2 = \fConflict{\Delta}{F_2} \cap F_1 = \varemptyset$.
\end{definition}

We use $\ninter{\Delta, \sta, e}{C_1}{C_2}$ to denote $\ninterf{\Delta}{\fClosure{\sta, e}{C_1}}{\fClosure{\sta, e}{C_2}}$.

\begin{fact}
	$\ninter{\Delta}{C_1}{C_2}$ iff $\ninterf{\Delta}{\fClosure{\Delta}{C_1}}{\fClosure{\Delta}{C_2}}$.
\end{fact}

\begin{fact}[Symmetry of Footprint Non-Interference]  \label{lemma:ninterf-symm}
	$\ninterf{\Delta}{F_1}{F_2}$ implies $\ninterf{\Delta}{F_2}{F_1}$.
\end{fact}

% \begin{lemma}
% 	If
%   (1) $\match{}{\sta, e}{\Delta}$,
%   (2) $\fConflict{\Delta}{C_1} \cap C_2 = \varemptyset$,
%   and (3) $\sub{\Delta}{C_0}{C_1}$,
%   then $\fConflict{\Delta}{C_0} \cap C_2 = \varemptyset$.
% \end{lemma}

% \begin{proof}
% 	By induction on the derivation of $\sub{\Delta}{C_0}{C_1}$.

%   \emph{Case \textsc{sc-elem}}.
%   In this case, $C_0 = \set{x}$ and $x \in C_1$.
%   Therefore, $\fConflict{\Delta}{C_0} \subseteq \fConflict{\Delta}{C_1}$ and we conclude.

%   \emph{Case \textsc{sc-var}}.
%   In this case, we have $C_0 = \set{x}$, $x : \tCap{C_x}{S} \in \Delta$
%   and $\sub{\Delta}{C_x}{C_1}$.
% \end{proof}

% \begin{lemma}
% 	If
%   (1) $\match{}{\sta, e}{\Delta}$,
%   (2) $\fConflict{\Delta}{\fClosure{\Delta}{C_1}} \cap \fClosure{\Delta}{C_2} = \varemptyset$,
%   then $\fConflict{\Delta}{\fClosure{\sta, e}{C_1}} \cap \fClosure{\sta, e}{C_2} = \varemptyset$.
% \end{lemma}

% \begin{proof}
% 	By induction on $\fClosure{\Delta}{C_1}$.

%   \emph{Case 1}.
%   In this case, $C_1 = \set{x}$, $x :_! T \in \Delta$ and $\fClosure{\Delta}{C_1} = \set{x}$.
%   By Lemma \ref{lemma:bang-binding-to-store-evctx}
%   we show that $x \in \bvar{\sta}$ or $x \in \dom{e}$.
%   Therefore $\fClosure{\sta, e}{C_1} = \set{x}$ and we conclude.

%   \emph{Case 2}.
%   In this case, $C_1 = \set{x}$, $x :_\epsilon \tCap{C}{S} \in \Delta$
%   and $\fClosure{\Delta}{C_1} = \fClosure{\Delta}{C}$.
% \end{proof}

\begin{lemma}  \label{lemma:reach-star}
	If $F \ne \varemptyset$,
  $* \in \fConflict{\G}{F}$.
\end{lemma}

\begin{proof}
	By induction on $\fConflict{\G}{F}$. In each case we conclude either immediately or by IH.
\end{proof}

\begin{lemma}  \label{lemma:all-qq-implies-ninter}
	If $\forall \tau \in C_1, C_2$, $\tau = x^?$ for some $x :_! T \in \Delta$,
  then $\ninter{\Delta, \sta, e}{C_1}{C_2}$.
\end{lemma}

\begin{proof}
  By the definition of $\fConflict{\Delta}{\cdot}$ we have
  $\fConflict{\Delta}{\fClosure{\sta, e}{C_1}} = \fConflict{\Delta}{\fClosure{\sta, e}{C_2}} = \set{*}$,
  and $* \notin \fClosure{\sta, e}{C_1} \cup \fClosure{\sta, e}{C_2}$.
  We therefore conclude.
\end{proof}

\begin{lemma}  \label{lemma:frac-reachable-implies-base-reachable}
	If $x^{?} \in \fConflict{\G}{F}$
  then $x \in \fConflict{\G}{F}$.
\end{lemma}

\begin{proof}
	By induction on $\fConflict{\G}{F}$.
  In each case either there is a contradiction,
  or we conclude immediately,
  or we conclude by IH.
\end{proof}

\begin{lemma}  \label{lemma:ninter-qq}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  and (2) $\ninterf{\Delta}{\fClosure{\Delta}{C_1}}{F_2}$,
  then $\ninterf{\Delta}{\fClosure{\Delta}{C_1^{??}}}{F_2}$.
\end{lemma}

\begin{proof}
  By induction on $\fClosure{\Delta}{C_1}$.

  \emph{Case 1}.
  In this case, $C_1 = \set{x}$ and $x :_! T \in \Delta$.
  We have $\ninterf{\Delta}{\set{x}}{F_2}$.
  Also, $\fClosure{\Delta}{\set{x^{?}}} = \set{x^{?}}$.
  Now we prove the two conditions for $\ninterf{\Delta}{\set{x^{?}}}{F_2}$
  by contradiction.
  First, assume that $\fConflict{\Delta}{\set{x^{?}}} \cap F_2 \ne \varemptyset$.
  Then we have $* \in F_2$.
  By Lemma \ref{lemma:reach-star} we have $* \in \fConflict{\Delta}{\set{x}}$
  and therefore it contradicts with the premise.
  Second, assume that $\set{x^{?}} \cap \fConflict{\Delta}{F_2} \ne \varemptyset$,
  which implies that $x^{?} \in \fConflict{\Delta}{F_2}$.
  By Lemma \ref{lemma:frac-reachable-implies-base-reachable}
  we show that $x \in \fConflict{\Delta}{F_2}$
  and therefore derive a contradiction.

  \emph{Case 2}. By IH.

  \emph{Case 3}.
  In this case, $C_1 = \set{x^{?}}$ and $x :_! T \in \Delta$.
  We have $\ninterf{\Delta}{\set{x^{?}}}{F_2}$.
  Note that $\set{x^{?}}^{??} = \set{x^{?}}$
  and we conclude immediately.

  \emph{Case 4}.
  As above.

  \emph{Case 5}.
  We conclude immediately.

  \emph{Case 6}. By IH.
\end{proof}

\begin{corollary}  \label{coro:ninter-qq}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  and (2) $\ninter{\Delta}{C_1}{C_2}$,
  then $\ninter{\Delta}{C_1}{C_2}$.
\end{corollary}

\begin{lemma}  \label{lemma:sta-ninter-qq}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  and (2) $\ninterf{\Delta}{\fClosure{\sta, e}{C_1}}{F_2}$,
  then $\ninterf{\Delta}{\fClosure{\sta, e}{C_1^{??}}}{F_2}$.
\end{lemma}

\begin{proof}
	By induction on $\fClosure{\sta, e}{C_1}$. As in Lemma \ref{lemma:ninter-qq}.
\end{proof}

\begin{corollary}  \label{coro:sta-ninter-qq}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  and (2) $\ninter{\Delta, \sta, e}{C_1}{C_2}$,
  then $\ninter{\Delta, \sta, e}{C_1}{C_2}$.
\end{corollary}

\begin{lemma}  \label{lemma:ninterf-subcapt}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  (2) $\ninterf{\Delta}{\fClosure{\Delta}{C_1}}{F_2}$,
  (3) $\sub{\Delta}{C_0}{C_1}$,
  and (4) $C_0 \subseteq \dom{\sta}$,
  then $\ninterf{\Delta}{\fClosure{\Delta}{C_0}}{F_2}$.
\end{lemma}

\begin{proof}
  By induction on the derivation of $\sub{\Delta}{C_0}{C_1}$.

  \emph{Case \textsc{sc-elem}}.
  In this case, $C_0 = \set{x}$ and $x \in C_1$.
  Therefore, we have $\fClosure{\Delta}{C_0} \subseteq \fClosure{\Delta}{C_1}$ and conclude.

  \emph{Case \textsc{sc-set}}.
  We conclude by IH.

  \emph{Case \textsc{sc-var}}.
  In this case, $C_0 = \set{x}$,
  $x : \tCap{C_x}{S} \in \Delta$,
  and $\sub{\Delta}{C_x}{C_1}$.
  If $x :_\epsilon \tCap{C_x}{S} \in \Delta$,
  we have $\fClosure{\Delta}{C_0} = \fClosure{\Delta}{C_x}$ and conclude by IH.
  Otherwise, if $x :_! \tCap{C_x}{S} \in \Delta$,
  since $x \in \dom{\sta}$, we can show that $C_x = \set{*}$.
  Therefore, $* \in C_1$ and we have $\ninterf{\Delta}{\set{*}}{F_2}$.
  By Lemma \ref{lemma:reach-star} we have either $* \in \fConflict{\Delta}{F_2}$, or $F_2 = \varemptyset$.
  In the first case there is a contradiction while in the second case we conclude immediately.

  \emph{Case \textsc{sc-var-$?$}}. As above.

  \emph{Case \textsc{sc-$<:$-$?$}}.
  In this case, $C_0 = \set{x^{?}}$
  and $\sub{\Delta}{\set{x}}{C_1}$.
  By IH we have $\ninterf{\Delta}{\fClosure{\Delta}{\set{x}}}{F_2}$.
  We conclude by Lemma \ref{lemma:ninter-qq}.
\end{proof}

\begin{lemma}[Non-Interference of footprint: from typing to reduction]
  \label{lemma:ninterf-footprint-typing-to-store-aux}
	If
  (1) $\match{}{\sta, e}{\Delta}$,
  and (2) $\ninterf{\Delta}{\fClosure{\Delta}{C_1}}{F_2}$,
  then (3) $\ninterf{\Delta}{\fClosure{\sta, e}{C_1}}{F_2}$.
\end{lemma}

\begin{proof}
  By induction on the lexical order $(\max_{\tau \in C_1} \fDepth{\Delta}{\tau}, | C_1 |)$.
  % By induction on $\fClosure{\Delta}{C_1}$.

  \begin{itemize}
  \item When $\max_{\tau \in C_1} \fDepth{\Delta}{\tau} = k$ and $k > 0$.

  \emph{Case 1}.
  In this case, $C_1 = \set{x}$ and $x :_! T \in \Delta$.
  By Lemma \ref{lemma:bang-binding-to-store-evctx} we have $x \in \bvar{\sta}$ or $x \in \dom{e}$.
  Therefore $\fClosure{\sta, e}{C_1} = \fClosure{\Delta}{C_1} = \set{x}$ and we conclude.

  \emph{Case 2}.
  In this case, $C_1 = \set{x}$ and $x :_\epsilon \tCap{C_x}{S} \in \Delta$.
  By Lemma \ref{lemma:eps-binding-to-store} we have $x \in \bval{\sta}$.
  Therefore, $\sta(\tVal{x}) = v$ for some $v$.
  By Lemma \ref{lemma:value-typing-inv-cs} we have $\sub{\Delta}{\cv{v}}{C_x}$.
  By Lemma \ref{lemma:ninterf-subcapt} we can show that $\ninterf{\Delta}{\fClosure{\Delta}{\cv{v}}}{F_2}$.
  By Lemma \ref{lemma:value-lookup-cv-depth} we have $\max_{\tau \in \cv{v}}{\fDepth{\Delta}{\tau}} < \fDepth{\Delta}{x}$.
  Therefore we can invoke IH and show that $\ninterf{\Delta}{\fClosure{\sta, e}{\cv{v}}}{F_2}$ and conclude.

  \emph{Case 3}. As in Case 1.

  \emph{Case 4}. As in Case 2.

  \emph{Case 5}. Conclude immediately.

  \emph{Case 6}. By IH.
  
  \item When $\max_{\tau \in C_1} \fDepth{\Delta}{\tau} = 0$.
    We proceed by splitting the cases of $\fClosure{\Delta}{C_1}$

    \emph{Case 2.}
    In this case, $C_1 = \set{x}$ and $x :_\epsilon \tCap{C_x}{S} \in \Delta$.
    We have $\fDepth{\Delta}{x} = 0$ and therefore either $C_x = \set{}$ or $C_x = \set{*}$.
    We can show that $\sta(\tVal{x}) = v$ for some $v$.
    If $C_x = \set{}$, we invoke Lemma \ref{lemma:value-lookup-cv-depth}
    and show that $\max_{\tau \in \cv{v}} \fDepth{\Delta}{\tau} < 0$
    and therefore $\cv{v} = \varemptyset$ and we conclude.
    Otherwise if $C_x = \set{*}$,
    by Lemma \ref{lemma:reach-star} we show that
    either $F_2$ is empty or $* \in \fConflict{\Delta}{F_2}$.
    In the first case we could conclude
    and in the second case
    we have $(\fClosure{\Delta}{x} = \set{*}) \cap \fConflict{\Delta}{F_2} \ne \varemptyset$
    and $\ninterf{\Delta}{\fClosure{\Delta}{x}}{F_2}$ will not hold.

  \end{itemize}

\end{proof}

\begin{corollary}  \label{coro:ninterf-footprint-typing-to-store}
	If (i) $\match{}{\sta, e}{\Delta}$,
  and (ii) $\ninterf{\Delta}{\fClosure{\Delta}{C_1}}{\fClosure{\Delta}{C_2}}$,
  then $\ninterf{\Delta}{\fClosure{\sta, e}{C_1}}{\fClosure{\sta, e}{C_2}}$.
\end{corollary}

\begin{proof}
	By Lemma \ref{lemma:ninterf-footprint-typing-to-store-aux} and Fact \ref{lemma:ninterf-symm}.
\end{proof}

\begin{definition}[Dealiasing lenient bindings]
  We use $\dealiasLB{e}{C}{C^\prime}$ to denote one step of lenient binding dealiasing in the evaluation context $e$.
  It is defined as $\dealiasLB{e}{C}{C/x \cup \cv{t}}$ if $x \in C \wedge e(x) = t$,
  or $\dealiasLB{e}{C}{C/{x^{?}} \cup \cv{t}^{??}}$ if $x^{?} \in C \wedge e(x) = t$.
\end{definition}

\begin{lemma}
	If
  (i) $\match{}{\sta, e}{\Delta_\sta, \Delta_e}$;
  (ii) $\typ{\Delta_\sta}{\evctx{t}}{T}$;
  (iii) $\ninter{\Delta, \sta, e}{C_1}{C_2}$;
  (iv) $\fReachLazyN{*}{e, t}{C_1} \bowtie \fReachLazyN{*}{e, t}{C_2}$;
  (v)
  $\forall x \in \fReachLazyN{*}{e, t}{C_1}. \ninter{\Delta, \sta, e}{\cv{e(x)}}{C_2/x}$
  $\wedge \forall x^{?} \in \fReachLazyN{*}{e, t}{C_1}. \ninter{\Delta, \sta, e}{\cv{e(x)}^{??}}{C_2/x}$
  and vice versa;
  and (vi) $\dealiasLB{e}{C_1}{C_1^\prime}$,
  then
  (i) $\ninter{\Delta, \sta, e}{C_1^\prime}{C_2}$;
  (ii) $\fReachLazyN{*}{e, t}{C_1^\prime} \bowtie \fReachLazyN{*}{e, t}{C_2}$;
  and (iii) $\forall x \in \fReachLazy{e, t}{C_1^\prime}. \ninterf{\Delta, \sta, e}{\cv{e(x)}}{C_2/x}$ and vice versa.
\end{lemma}

\begin{proof}
  By inverting the judgment $\dealiasLB{e}{C_1}{C_1^\prime}$ we have two cases.
  In the first case $x \in C_1$, $e(x) = t$ and $C_1^\prime = C_1/x \cup \cv{t}$.
  Now we prove the conclusions one by one.

  \emph{Conclusion (i).}
  Since we have $\ninter{\Delta, \sta, e}{C_1/x}{C_2}$, what we have to show is $\ninter{\Delta, \sta, e}{\cv{t}}{C_2}$.
  From premise (v) we have $\ninter{\Delta, \sta, e}{\cv{t}}{C_2/x}$.
  From premise (iv) we can show that $x \notin C_2$, from which we show that $C_2/x = C_2$ and we conclude.

  \emph{Conclusion (ii).}
  We have $\fReachLazy{e, t}{C_1/x} \subseteq \fReachLazy{e, t}{C_1}$.
  Also, we can show that $\fReachLazyN{*}{e, t}{x} = \set{x} \cup \fReachLazyN{*}{e, t}{\cv{t}}$.
  Therefore we have $\fReachLazyN{*}{e, t}{\cv{t}} \subseteq \fReachLazyN{*}{e, t}{C_1}$.
  Now we can show that $\fReachLazy{e, t}{C_1^\prime} \subseteq \fReachLazy{e, t}{C_1}$ and conclude.

  \emph{Conclusion (iii)}.
  In the first direction, since previously we have shown that $\fReachLazyN{*}{e, t}{C_1^\prime} \subseteq \fReachLazyN{*}{e, t}{C_1}$
  we conclude immediately.
  In the second direction, given $y \in \fReachLazy{e, t}{C_2}$,
  we would like to show that $\ninter{\Delta, \sta, e}{C_1^\prime/y}{\cv{e(y)}}$.
  We could already show that $\ninter{\Delta, \sta, e}{(C_1/x)/y}{\cv{e(y)}}$,
  and the remaining to be shown is $\ninter{\Delta, \sta, e}{\cv{t}/y}{\cv{e(y)}}$.
  In the next we show that $x \notin \cv{e(y)}$.
  If $x \in \cv{e(y)}$ we have $x \in \fReachLazy{e, t}{y}$ and there is a contradiction.
  Therefore $e(y)/x = e(y)$, and now we have to show that $\ninter{\Delta, \sta, e}{\cv{t}/y}{\cv{e(y)}/x}$.
  Now we conclude by Lemma \ref{lemma:lenient-bindings-ninter} and Lemma \ref{coro:ninterf-footprint-typing-to-store}.
  Given $y^{?} \in \fReachLazyN{*}{e, t}{C_2}$,
  we have to show that $\ninter{\Delta, \sta, e}{C_1^\prime/y}{\cv{e(y)}^{??}}$.
  We would already have $\ninter{\Delta, \sta, e}{(C_1/x)/y}{\cv{e(y)}^{??}}$
  and the remaining to be shown is $\ninter{\Delta, \sta, e}{\cv{t}}{\cv{e(y)}^{??}}$.
  Since $x \notin \cv{e(y)}^{??}$,
  this follows from Lemma \ref{lemma:lenient-bindings-ninter} and Lemma \ref{coro:ninterf-footprint-typing-to-store}.

  In the second case, $x^{?} \in C_1$, $e(x) = t$ and $C_1^\prime = C_1/x \cup \cv{t}^{??}$.

  \emph{Conclusion (i)}.
  Since $\ninter{\Delta, \sta, e}{C_1/{x^{?}}}{C_2}$ what we need to show is $\ninter{\Delta, \sta, e}{\cv{t}^{??}}{C_2}$.
  From premise (iv) we can show that $x \notin C_2$
  and from premise (v) we have $\ninter{\Delta, \sta, e}{\cv{t}}{C_2/x}$.
  Now we conclude.

  \emph{Conclusion (ii)}. Similarly to the first case.

  \emph{Conclusion (iii)}.
  For the first direction we can show that $\fReachLazyN{*}{e, t}{C_1^\prime} \subseteq \fReachLazyN{*}{e, t}{C_1}$
  and conclude.
  For the second direction, we inspect each $\tau \in \fReachLazyN{*}{e, t}{C_2}$
  and split into $\tau = y$ and $\tau = y^?$.
  In the first case we have $y \in \fReachLazyN{*}{e, t}{C_2}$.
  We would like to show that $\ninter{\Delta, \sta, e}{C_1^\prime/y}{\cv{e(y)}}$.
  $\ninter{\Delta, \sta, e}{(C_1/x)/y}{\cv{e(y)}}$ already holds
  and the remaining to be proven is $\ninter{\Delta, \sta, e}{\cv{t}^{??}/y}{\cv{e(y)}}$.
  By Lemma \ref{lemma:lenient-bindings-ninter} and Lemma \ref{coro:ninterf-footprint-typing-to-store}
  we can show that
  $\ninter{\Delta, \sta, e}{\cv{t}^{??}/y}{\cv{e(y)}/x}$.
  We also have $x \notin \cv{e(y)}$ (otherwise $x \in \fReachLazyN{*}{e, t}{y}$ and a contradiction is derived),
  so $\cv{e(y)}/x = \cv{e(y)}$ and we conclude.
  In the second case we have $y^{?} \in \fReachLazyN{*}{e, t}{C_2}$.
  Similarly what we have to prove is $\ninter{\Delta, \sta, e}{\cv{t}^{??}/y}{\cv{e(y)}^{??}}$.
  % We conclude by Lemma \ref{lemma:all-qq-implies-ninter}.
  We invoke Lemma \ref{lemma:lenient-bindings-ninter} and Lemma \ref{coro:ninterf-footprint-typing-to-store} again
  and show that $\ninter{\Delta, \sta, e}{\cv{t}/y}{\cv{e(y)}/x}$.
  By Lemma \ref{coro:sta-ninter-qq} we show that $\ninter{\Delta, \sta, e}{\cv{t}^{??}/y^?}{\cv{e(y)}^{??}/x^{?}}$.
\end{proof}

\begin{lemma}  \label{lemma:dealias-lb-auth}
	If $A = \fEmbed{\fAuth{e}{\sta}{C}}$,
  then exists $\dealiasLBN{e}{C}{C^\prime}$ such that $\fClosure{\sta, e}{C^\prime} = A$.
\end{lemma}

\begin{proof}
	By induction on $\fAuth{e}{\sta}{C}$.

  \emph{Case 1}. In this case, $A = \fConflict{\sta, e}{C}$ and we conclude immediately.
  
  \emph{Case 2}. In this case, $\sta(\tVal{x}) = v$ and $A = \fEmbed{\fAuth{e}{\sta}{\cv{v}}}$.
  We invoke IH and conclude.

  \emph{Case 3}. In this case, $e(x) = t$ and $A = \fEmbed{\fAuth{e}{\sta}{\cv{t}}}$.
  Let $C_1 = \cv{t}$, we first invoke IH to show that exists $\dealiasLBN{e}{C_1}{C_1^\prime}$
  such that $\fClosure{\sta, e}{C_1^\prime} = A$.
  Also, the rewriting $\dealiasLB{e}{\set{x}}{\cv{t}}$ is derivable as well.
  We therefore conclude.

  \emph{Case 4 and 5}. As in Case 1 and 2.

  \emph{Case 6}.
  Let $C_1 = \cv{t}^{??}$.
  We invoke IH to show that there exists $\dealiasLB{e}{C_1}{C_1^\prime}$
  such that $\fClosure{\sta, e}{C_1^\prime} = A$.
  And we derive $\dealiasLB{e}{\set{x^{?}}}{\cv{t}^{??}}$ and conclude.

  \emph{Case 7}. By IH.
\end{proof}

% \begin{definition}[Expansion of footprint]
%   The expansion $\fExpand{\sta, e}{F}$ of a footprint $F$
%   on the store contexts $\sta, e$ is defined as:

%   \begin{equation*}
%     \begin{split}
%       &\fExpand{\sta, e}{x} \quad &= \quad &\set{x}, \quad &\text{if $x \in \dom{\sta}$} \\
%       &\fExpand{\sta, e}{x} \quad &= \quad &\fExpand{\sta, e}{\fClosure{\sta, e}{\cv{t}}}, \quad &\text{if $e(x) = t$} \\
%       &\fExpand{\sta, e}{x^?} \quad &= \quad &\set{x^{?}}, \quad &\text{if $x \in \dom{\sta}$} \\
%       &\fExpand{\sta, e}{x^?} \quad &= \quad &\fExpand{\sta, e}{\fClosure{\sta, e}{\cv{t}^{??}}}, \quad &\text{if $e(x) = t$} \\
%       &\fExpand{\sta, e}{F_1 \cup F_2} \quad &= \quad &\fExpand{\sta, e}{F_1} \cup \fExpand{\sta, e}{F_2}, \quad & \\
%     \end{split}
%   \end{equation*}
% \end{definition}

% \begin{lemma}[Expansion of a footprint is the embedding of the authority]
% 	$\fExpand{\sta, e}{\fClosure{\sta, e}{C}} = \fEmbed{\fAuth{e}{\sta}{C}}$.
% \end{lemma}

% \begin{proof}
% 	By induction on $\fAuth{e}{\sta}{C}$.

%   \emph{Case 1}.
%   In this case, $C = \set{x}$ and $x \in \bvar{\sta}$.
%   Therefore we have $x \in \dom{\sta}$
%   and we can show that $\fExpand{\sta, e}{\fClosure{\sta, e}{C}} = \fEmbed{\fAuth{e}{\sta}{C}} = \set{x}$
%   and conclude.

%   \emph{Case 2}.
%   As above.

%   \emph{Case 3}.
%   In this case, $C = \set{x}$, $x \in \dom{e}$ and $e(x) = t$.
%   We have $\fEmbed{\fAuth{e}{\sta}{C}} = \fEmbed{\fAuth{e}{\sta}{\cv{t}}}$.
%   Also, we have $\fExpand{\sta, e}{\fClosure{\sta, e}{C}} = \fExpand{\sta, e}{\set{x}} = \fExpand{\sta, e}{\fClosure{\sta, e}{\cv{t}}}$.
%   We conclude by IH.

%   \emph{Case 4, 5 and 6}.
%   As in Case 1, 2 and 3.

%   \emph{Case 7}.
%   By IH.
% \end{proof}

% \begin{lemma}
% 	If (i) $\match{}{\sta, e}{\Delta_1, \Delta_2}$,
%   (ii) $\dom{\Delta_1} = \dom{\sta}$ and $\dom{\Delta_2} = \dom{e}$,
%   and (iii) $\typ{\Delta_1}{\evctx{t}}{T}$,
%   then for any $x, y \in \domE{e}{t}$ ($x \ne y$),
%   we have $\ninterf{\Delta_1, \Delta_2}{\fClosure{\sta, e}{\cv{e(x)}/y}}{\fClosure{\sta, e}{\cv{e(y)}/x}}$.
% \end{lemma}

% \begin{lemma}
% 	If
%   (1) $\match{}{\sta, e}{\Delta_1, \Delta_2}$ (and $\dom{\Delta_1} = \dom{\sta}$, $\dom{\Delta_2} = \dom{e}$, let $\Delta = \Delta_1, \Delta_2$),
%   (2) $\typ{\Delta_1}{\evctx{t}}{T}$,
%   (3) $\ninterf{\Delta}{F_1}{F_2}$,
%   (4) $\forall x \in \fReachLazy{e, t}{F_2 \cap \domE{e}{t}}. \ninterf{\Delta}{F_1/x}{\fClosure{\sta, e}{e(x)}}$
%   and vice versa,
%   then $\ninterf{\Delta}{\fExpand{\sta, e}{F_1}}{F_2}$.
% \end{lemma}

% \begin{lemma}[Non-Interference of parallel-let binding evaluation]
%   If
%   (1) $\match{}{\sta}{\Delta}$,
%   (2) $\typ{\Delta}{\tLetPar{x}{t}{u}}{T}$,
%   then given the series of reduction
%   $\mathcal{R} = \st{\sta}{\tLetPar{x}{t}{u}} \red \st{\sta_1}{\tLetPar{x}{t_1}{u_1}} \red \cdots \st{\sta_k}{\tLetPar{x}{t_k}{u_k}} \red \st{\sta^\prime}{\tLetPar{x}{v}{u^\prime}}$,
%   the left trace $\fTraceX{(x, L)}{\mathcal{R}}$ and the right one $\fTraceX{(x, R)}{\mathcal{R}}$ are non-interfering.
% \end{lemma}

% \subsubsection{Legacy Proof}

% \begin{lemma}[Mutable variable lookup inversion]  \label{lemma:value-typing-ref-impossible}
% 	It is not possible to derive $\typDft{v}{\tCap{C}{\tRef{S}}}$.
%   If $\match{}{\sigma}{\Delta}$ and $\typ{\Delta}{x}{\tCap{C}{\tRef{S}}}$,
%   $x :_! \tCap{C_x}{\tRef{S_x}} \in \Delta$,
%   $\sub{\Delta}{C_x}{C}$
%   and $\sub{\Delta}{S_x}{S}$.
% \end{lemma}
% \TODO{Assumed. Should be easy.}
% % \begin{proof}
% % 	By inspecting the derivation of the typing judgment.
% %   No applicable rules to derive such a judgment.
% % \end{proof}

% \begin{lemma}[Inversion of typing under an evaluation context]  \label{lemma:evctx-typ-inv}
%   If $\typDft{\evctx{t}}{T}$,
%   then $t$ is typeable in $\G$.
% \end{lemma}
% \TODO{Assumed.}

% \begin{lemma}[Inversion of write typing]  \label{lemma:typ-write-inv}
% 	If $\typDft{\tWrite{x}{y}}{T}$,
%   we have $\typDft{x}{\tCap{C_x}{\tRef{S_0}}}$,
%   $\typDft{y}{S_0}$
%   and $\subDft{S_0}{T}$.
% \end{lemma}

% \begin{proof}
% 	By induction on the number of \textsc{sub} derivations.
% \end{proof}

% \begin{lemma}[Inversion of read typing]  \label{lemma:typ-read-inv}
% 	If $\typDft{\tRead{x}}{T}$,
%   we have $\typDft{x}{\tCap{C_x}{\tRef{S_0}}}$,
%   and $\subDft{S_0}{T}$.
% \end{lemma}
% \TODO{Assumed.}

% \begin{lemma}[Term abstraction lookup inversion: capture set]  \label{lemma:lookup-fun-inv-capset}
% 	If $\match{\G}{\sigma}{\Delta}$;
%   $\Delta(x) = \tCap{C}{\forall(z: U) T}$,
%   and $\sigma(x) = \lambda(z : U^\prime) t$,
%   then $\sub{\G, \Delta}{\cv{t}/z}{C}$.
% \end{lemma}
% \TODO{Assumed. Should be an easy one.}

% % \begin{definition}[Flat environment]
% % 	An environment $\G$ is \textbf{flat}
% %   iff any exclusive bindings in it captures $\set{*}$, i.e. $\forall x :_! \tCap{C}{S} \in \G, C = \set{*}$.
% % \end{definition}

% % \begin{lemma}{Matching environment is flat}
% % 	If $\match{}{\sigma}{\Delta}$,
% %   $\Delta$ is flat.
% % \end{lemma}
% % \TODO{Assumed.}

% % \textbf{Remarks.}
% % When stating the monotone lemma below, we require the environment to be \emph{flat}.
% % A flat environment essentially means an environment without \emph{grouping}.
% % When grouping is involved, the monotone statement has to be made more complicatedly:
% % $\set{x}$ should be considered a sub-footprint of $\set{r}$,
% % if $x$ is allocated on $r$ (e.g. $x :_! \tCap{\set{r}}{S} \in \G$).
% % The subset relation will not be sufficient.

% \begin{lemma}[Footprint is monotonic over subcapturing]
% 	If $\subDft{C_1}{C_2}$,
%   $\subDft{\fClosure{\G}{C_1}}{\fClosure{\G}{C_2}}$.
% \end{lemma}

% \begin{proof}
% 	By induction on the derivation of subcapturing.

%   \emph{Case \textsc{sc-elem}}.
%   In this case, we have $C_1 = \set{x}$, and $x \in C_2$.
%   We can show that $\fClosure{\G}{C} = \fClosure{\G}{C \cup \set{x}} = \fClosure{\G}{C} \cup \fClosure{\G}{x}$,
%   and conclude.

%   \emph{Case \textsc{sc-set}}.
%   We conclude by IH and the fact that $\fClosure{\G}{\cdot}$ is homomorphic.

%   \emph{Case \textsc{sc-var}}.
%   In this case, $C_1 = \set{x}$, $x : \tCap{C_x}{S} \in \G$ and $\subDft{C_x}{C_2}$.
%   By IH we have $\subDft{\fClosure{\G}{C_x}}{\fClosure{\G}{C_2}}$.
%   If $x :_! \tCap{C_x}{S} \in \G$, $\fClosure{\G}{x} = \set{x}$.
%   We conclude by IH and the \textsc{sc-var} rule.
%   If $x :_\epsilon \tCap{C_x}{S} \in \G$, $\fClosure{\G}{x} = \fClosure{\G}{C_x}$ and we conclude immediately.
% \end{proof}

% \begin{lemma}[Footprint is monotonic over subset]  \label{lemma:footprint-mono-subset}
% 	If $C_1 \subseteq C_2$,
%   $\fClosure{\G}{C_1} \subseteq \fClosure{\G}{C_2}$.
% \end{lemma}

% \begin{proof}
% 	We can show that $\fClosure{\G}{C_2} = \fClosure{\G}{C_1 \cup C_2} = \fClosure{\G}{C_1} \cup \fClosure{\G}{C_2}$
%   and conclude.
% \end{proof}

% \begin{lemma}
%   If (1) $\match{}{\sigma}{\Delta}$;
%   (2) $\typ{\Delta}{\evctx{t}}{T}$;
%   (3) $\reduction{\stevctx{t}}{\stctx{\ctx{\sigma^\prime}{\evctx{t^\prime}}}}$,
%   then $\mathcal{T} = \fTrace{\reduction{\stevctx{t}}{\stctx{\ctx{\sigma^\prime}{\evctx{t^\prime}}}}}$ $\sqsubseteq \fClosure{\Delta}{\cv{t}}$.
% \end{lemma}

% \begin{proof}
%   Proceed by induction on the derivation of the reduction.

%   \emph{Case \textsc{lift-set}}.
%   In this case, $t = \tWrite{x}{y}$.
%   $\mathcal{T} = \set{(x, \pWr{})}$,
%   and $\fClosure{\Delta}{\cv{t}} = \fClosure{\Delta}{\set{x, y}} = \fClosure{\Delta}{x} \cup \fClosure{\Delta}{y}$.
%   By Lemma \ref{lemma:evctx-typ-inv} we have $\typ{\G, \Delta}{\tWrite{x}{y}}{U}$ for some $U$.
%   Now invoke Lemma \ref{lemma:typ-write-inv},
%   we have $\typ{\Delta}{x}{{\tCap{C_x}{\tRef{S_0}}}}$,
%   $\typ{\Delta}{y}{S_0}$
%   and $\sub{\Delta}{S_0}{U}$.
%   By Lemma \ref{lemma:value-typing-ref-impossible}
%   we show that $x \in \bvar{\sigma}$,
%   therefore $x :_! \tCap{C_x}{\tRef{S_0}} \in \Delta$.
%   Now we can show that $\fClosure{\Delta}{x} = {x}$
%   Therefore $\mathcal{T} \sqsubseteq \fClosure{\Delta}{\cv{t}}$.

%   \emph{Case \textsc{read}}.
%   In this case $t = \tRead{x}$.
%   $\mathcal{T} = \set{(x, \pRd{})}$.
%   By Lemma \ref{lemma:evctx-typ-inv},
%   $\typ{\Delta}{\tRead{x}}{U}$ for some $U$.
%   Now invoke Lemma \ref{lemma:typ-read-inv},
%   we have $\typ{\Delta}{x}{\tCap{C_x}{\tRef{S_0}}}$.
%   By Lemma \ref{lemma:value-typing-ref-impossible},
%   we show that $x :_! \tCap{C_x}{\tRef{S_0}} \in \Delta$.
%   Now we can prove that $\mathcal{T} \sqsubseteq \fClosure{\Delta}{\cv{t}}$ and conclude.

%   \emph{Other cases.}
%   In these cases $\mathcal{T} = \varemptyset$
%   we therefore conclude immediately.
% \end{proof}

% \begin{lemma}
%   If (1) $\match{}{\sigma}{\Delta}$;
%   (2) $\typ{\Delta}{\evctx{t}}{T}$;
%   and (3) $\reduction{\stevctx{t}}{\stctx{\ctx{\sigma^\prime}{\evctx{t^\prime}}}}$,
%   $\Delta \vdash \fClosure{\Delta}{\cv{t^\prime}}/\bvar{t} <: \fClosure{\Delta}{\cv{t}}/\bvar{t}$.
% \end{lemma}

% \begin{proof}
%   By induction on the derivation of the reduction relation.

%   \emph{Case \textsc{apply}}.
%   In this case,
%   $t = x\,y$,
%   $\sigma(x) = \lambda(z: U)s$,
%   $\sigma^\prime = []$, and $t^\prime = [y/z]s$.
%   Therefore $\bvar{t} = \bvar{t^\prime} = \varemptyset$.
%   By Lemma \ref{lemma:evctx-typ-inv},
%   we have $\typ{\Delta}{x\,y}{T_0}$ for some $T_0$.
%   By inspecting the derivation of $\typ{\Delta}{x\,y}{T_0}$,
%   we know that it is derived by \textsc{app} followed by a series of \textsc{sub}.
%   We can show that $\Delta(x) = {\tCap{C_x}{\forall(z: U_0) T_1}}$,
%   by inverting the typing of $x$.
%   By Lemma \ref{lemma:lookup-fun-inv-capset},
%   we have $\sub{\Delta}{\cv{s}/z}{C_x}$.
%   We have $\cv{t^\prime} = \cv{[y/z] {s}} = [y/z]\cv{s} \subseteq \cv{s}/z \cup \set{y}$.
%   By Lemma \ref{lemma:footprint-mono-subset} and the fact that $\fClosure{\Delta}{\cdot}$ is homomorphic,
%   $\fClosure{\Delta}{\cv{t^\prime}} \subseteq \fClosure{\Delta}{\cv{s}/z} \cup \fClosure{\Delta}{y}$.
%   On the other hand,
%   we can show that $\fClosure{\Delta}{\cv{t}} = \fClosure{\G}{x} \cup \fClosure{\G}{y} = \fClosure{\G}{C_x} \cup \fClosure{\G}{y}$.
%   We already know that $\sub{\Delta}{{\cv{s}/z}}{C_x}$,
% \end{proof}

==> sections/metatheory/soundness-v1.tex <==
\subsection{Strengthening, Refining, Weakening and Permutation}

\begin{lemma}[Refining preserves length]
	\label{lemma:refine-len-eq}
  $\G_1 \refined \G_2$ implies that $|\G_1| =\ |\G_2|$.
\end{lemma}

\begin{proof}
	By straightforward induction on the derivation.
\end{proof}

\begin{lemma}[Refining is transitive]
  \label{lemma:refine-trans}
	If $\G_1 \refined \G_2$
  and $\G_2 \refined \G_3$
  then $\G_1 \refined \G_3$.
\end{lemma}

\begin{proof}
	By straightforward induction on $|\G_1|$.
\end{proof}

\begin{lemma}[Refining preserves non-interference]
  \label{lemma:refining-pres-ninter}
  Given $\G_r \refined \G$,
  $\ninter{\G}{\fFootprint{\G}{C_1}}{F_2}$
  implies
  $\ninter{\G_r}{\fFootprint{\G_r}{C_1}}{F_2}$.
\end{lemma}

\begin{proof}
	Straightforward based on the definition of the non-interference check.
  Note that $\fFootprint{\G_r}{C_1} = \fFootprint{\G}{C_1}$.
\end{proof}

\begin{lemma}[Refining Preserves Typing]
  \label{lemma:typ-refining}
  Given inert environments $\G, \G_r$,
  if
  (i) $\G_r \refined \G$,
  and (ii) $\typ{\G}{t}{T}$,
  then $\typ{\G_r}{t}{T}$.
\end{lemma}

\begin{proof}
	By induction on the typing judgment.

  \emph{Case \textsc{prom}}.
  Then $\typ{\G^\prime}{t}{T}$,
  where $\G^\prime = \G_1, x :_{!D^\prime} P, \G_2$,
  $\G = \G_1, x :_{!D} P, \G_2$,
  and $\ninter{\G_1}{D^\prime}{\fFootprint{\G_1}{\cv{P}}}$.
  Now we inspect $\G_r$ and see that
  $\G_r = \G_{r1}, x :_{!D_r} P, \G_{r2}$ for some $\G_{r1}, \G_{r2}$.
  By the inertness of $\G_r$,
  $\ninter{\G_{r1}}{D_r}{\fFootprint{\G_{r1}}{\cv{P}}}$.
  Let $D_r^\prime = D_r \cup D^\prime$.
  Note that $\G_{r1} \refined \G_1$.
  By Lemma \ref{lemma:refining-pres-ninter}
  we show that
  $\ninter{\G_{r1}}{D^\prime}{\fFootprint{\G_1}{\cv{P}}}$.
  Therefore, we have
  $\ninter{\G_{r1}}{D^\prime \cup D_r}{\fFootprint{\G_1}{\cv{P}}}$.
  Let $\G_r^\prime = \G_{r1}, x :_{!D_r^\prime} P, \G_{r2}$.
  We have $\G_r^\prime$ is inert by repeated application of Lemma \ref{lemma:refining-pres-ninter}.
  Now we invoke IH to show that
  $\typ{\G_r^\prime}{t}{T}$,
  and finally conclude by (\textsc{prom}).

  \emph{Case \textsc{let}}.
  Then $t = \tLetMode{m}{x}{s}{u}$,
  $\typ{\G}{s}{U}$ for some $U$,
  and $\typ{\G, x :_m U}{u}{T}$.
  If $m = {!D}$,
  we additionally have
  $\ninter{\G}{D}{\fFootprint{\G}{(\cv{U} \cup \cv{s})}}$.
  If $m = {!D}$,
  we first show
  $\ninter{\G_r}{D}{\fFootprint{\G_r}{(\cv{U} \cup \cv{s})}}$
  by Lemma \ref{lemma:refining-pres-ninter}.
  Now we can conclude this case by IH and (\textsc{let}).

  \emph{Other cases.}
  By IH and the same rule.
\end{proof}

\subsection{Non-Interference}

\begin{lemma}  \label{lemma:ninter-implies-qq}
	$\ninter{\G}{F_1}{F_2}$ implies $\ninter{\G}{F_1^{??}}{F_2}$.
\end{lemma}

\begin{proof}
	Proof by contradiction.
  We assume that $\ninter{\G}{F_1^{??}}{F_2}$ does not hold,
  and split into two cases.

  \begin{enumerate}
  \item If $x^{?} \in F_1^{??}$, $y \in F_2$ and $x \in \fQ{\G}{y}$.
    Then we have $x \in F_1$ such that $x \in \fQ{\G}{y}$ and thus derive the contradiction.

  \item If $x^{?} \in F_1^{??}$, $y \in F_2$ and $y \in \fQ{\G}{x^?}$.
    In this case we have $\fQ{\G}{x}$ and $x \in F_1$.
    We therefore derive the contradiction too.
  \end{enumerate}
\end{proof}

\begin{lemma}
  \label{lemma:widen-ninter-implies-x-ninter}
  Given an inert environment $\G$,
  if (i) $x :_{!D} T \in \G$
  and (ii) $\ninter{\G}{\fFootprint{\G}{\cv{T}}}{F_2}$,
  then there exists an inert $\G_r$,
  such that
  $\G_r \refined \G$,
  and $\ninter{\G_r}{x}{F_2}$.
\end{lemma}

\begin{proof}
	By induction on $\max_{\tau \in F_2} \fDepth{\G}{\tau}$.
  Proceed by splitting $F_2$ to two sets $F_2^l$ and $F_2^r$,
  where $F_2^l$ is the set of references that are bound before $x$,
  and $F_2^r$ are the references bound otherwise.
  Now we inspect $\G$ and see that
  $\G = \G_1, x :_{!D} T, \G_2$.
  We first set
  $\G^\prime = \G_1, x :_{!D^\prime}, \G_2$,
  where $D^\prime = D \cup F_2^l$.
  $\G^\prime$ is therefore inert
  and $\G^\prime \refined \G$.
  Now we start inspecting members in $F_2^r$.
  $\forall \tau \in F_2^r$,
  we have $\ninter{\G^\prime}{\fFootprint{\G^\prime}{\cv{T}}}{\tau}$ by Lemma \ref{lemma:refining-pres-ninter}.
  Assume that $|\tau|\ :_{!D_\tau} T_\tau \in \G^\prime$,
  we have $\fFootprint{\G^\prime}{\cv{T}} \sqsubseteq D_\tau$,
  which implies that
  $\ninter{\G^\prime}{\fFootprint{\G^\prime}{\cv{T}}}{\fFootprint{\G^\prime}{\cv{T_\tau}}}$.
  Now we can invoke IH to show that
  there exists an inert $\G^{\prime\prime}$ such that
  $\ninter{\G^{\prime\prime}}{x}{\fFootprint{\G^{\prime\prime}}{\cv{T_\tau}}}$,
  and also $\G^{\prime\prime} \refined \G^\prime$.
  Now we inspect $\G^{\prime\prime}$ and see that
  $\G^{\prime\prime} = \G_1^{\prime\prime}, |\tau|\ :_{D_\tau^{\prime}} T_\tau, \G_2^{\prime\prime}$.
  Now we set
  $\G^\prime = \G_1^{\prime\prime}, |\tau|\ :_{D_\tau^\prime \cup \set{x}}, \G_2^{\prime\prime}$.
  We can see that $\G^\prime$ is still inert,
  and $\G^\prime \refined \G$,
  and also $\ninter{\G^{\prime}}{x}{\tau}$.
  Finally, we show that there exists an inert $\G^\prime$,
  such that
  $\G^\prime \refined \G$,
  $\ninter{\G^{\prime}}{x}{F_2^r}$,
  and also $\ninter{\G^{\prime}}{x}{F_2^l}$ by Lemma \ref{lemma:refining-pres-ninter}.
  Now we can conclude this lemma.
\end{proof}

\begin{lemma}[Subcapture preserves non-interference]  \label{lemma:subcapt-pres-ninter}
  Given an inert $\G$,
  if
  (i) $\ninter{\G}{\fFootprint{\G}{C_1}}{F_2}$ (where $F_2 \subseteq \{ x \ | \ x :_! T \in \G \}$),
  (ii) $\sub{\G}{C_0}{C_1}$,
  then
  there exists an inert environment $\G^\prime$
  such that $\G^\prime \refined \G$
  and $\ninter{\G}{\fFootprint{\G}{C_0}}{F_2}$.
\end{lemma}

\begin{proof}
	By induction on the subcapture derivation.

  \emph{Case \textsc{sc-var}}.
  In this case, $C_0 = \set{x}$ for some $x$,
  $x :_m \tCap{C_x}{S_x} \in \G$,
  and $\sub{\G}{C_x}{C_1}$.
  If $* \in C_x$, we have $* \in C_1$,
  and $\fFootprint{\G}{C_1} = \{ x \ | \ x :_! T \in \G \}$.
  Therefore we have $F_2 = \varemptyset$ and conclude immediately.
  Otherwise, $m =\ !{D}$,
  and for some $\G_1, \G_2$
  we have $\G = \G_1, x :_{!D} \tCap{C_x}{S_x}, \G_2$
  and $\ninter{\G_1}{D}{\fFootprint{\G_1}{C_x}}$.
  By IH, we show that $\ninter{\G}{\fFootprint{\G}{C_x}}{F_2}$.
  Now we invoke Lemma \ref{lemma:widen-ninter-implies-x-ninter} and conclude this case.
  % Let $D^\prime = D \cup (F_2 \cap \dom{\G_1})$.
  % We can therefore show that $\ninter{\G_1}{D^\prime}{\fFootprint{\G}{C_x}}$.
  % Let $\G^\prime = \G_1, x :_{!D^\prime} \tCap{C_x}{S_x}, \G_2$
  % and we can show that $\G^\prime$ is inert and $\G^\prime \refined \G$.
  % % We conclude by IH and the fact that $\fFootprint{\G}{x} = \fFootprint{\G}{C_x}$.

  % \emph{Case \textsc{sc-var-$?$}}.
  % As above.

  \emph{Case \textsc{sc-elem}}. Straightforward.

  \emph{Case \textsc{sc-set}}. By repeated IH.

  \emph{Case \textsc{sc-$<:$-$?$}}.
  In this case, $C_0 = \set{x^?}$,
  and $\sub{\G}{x}{C_1}$.
  By IH we have $\ninter{\G}{\fFootprint{\G}{x}}{F_2}$.
  We conclude by Lemma \ref{lemma:ninter-implies-qq}.

  % \TODO{fix!!}
\end{proof}

\subsection{Store and Evaluation Context Typing}

\begin{lemma}[Value typing inversion: capture set]  \label{lemma:value-typing-inv-cs}
	If $\typDft{v}{\tCap{C}{S}}$,
  $\subDft{\cv{v}}{C}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the typing judgment.
\end{proof}

% \begin{lemma}[Binding promotion for $\match{\G}{e}{\Delta}$]
%   \label{lemma:binding-prom-match}
%   Given
%   $\G = \G_1, x :_{!D} T, \G_2$,
%   and $\G^\prime = \G_1, x :_{\epsilon} T, \G_2$,
%   if
%   (i) $\match{\G}{e}{\Delta}$,
%   and (ii) $\ninterfp{\G_1}{D}{\cv{T}}$,
%   then
%   $\match{\G^\prime}{e}{\Delta}$.
% \end{lemma}

% \begin{proof}
% 	By induction on $\match{\G}{e}{\Delta}$.

%   \emph{Case \textsc{ctx-empty}}.
%   Conclude immediately.

%   \emph{Case \textsc{ctx-grow-let} and \textsc{ctx-grow-var}}.
%   By IH.

%   \emph{Case \textsc{ctx-grow-par}}.
%   In this case,
%   $e = \tLetMode{!{D_0}}{y}{s}{e^\prime}$,
%   $\Delta = y :_{!D_0} U, \Delta_0$,
%   $\typ{\G}{s}{U}$,
%   and $\match{\G, y :_{!D_0} U}{e^\prime}{\Delta_0}$.
%   By IH we have $\match{\G^\prime, y :_{!D_0}}{e^\prime}{\Delta_0}$.
%   By applying (\textsc{prom}) we have
%   $\typ{\G^\prime}{s}{U}$.
%   Now we conclude by (\textsc{ctx-grow-par}).
% \end{proof}

% \begin{lemma}[Erasing $!$-annotation for non-interference check]
%   \label{lemma:erase-bang-ninter}
%   Given $\Xi = \G, x :_{!D} T, \Delta$,
%   and $\Xi^\prime = \G, x :_\epsilon T, \Delta$,
%   if
%   (i) $\ninter{\G}{D}{\fFootprint{\G}{\cv{T}}}$
%   and (ii) $\ninterfp{\Xi}{C_1}{C_2}$,
%   then $\ninterfp{\Xi^\prime}{C_1}{C_2}$.
% \end{lemma}

% \begin{proof}
%   Proceed by inspecting the membership of $x^*$ in the footprints.
%   \begin{itemize}
%   \item
%     We first consider the case when $x$ is the member of either footprint.
%     First of all, we can show that $x \in \fFootprint{\Xi}{C_1}$
%     or $x \in \fFootprint{\G}{C_2}$ but not both.
%     This is because if $x$ is a member of both footprints,
%     we have that $x \in {D}$ does not hold
%     by the well-formedness of the environment $\G$.
%     Therefore $\ninterfp{\Xi}{C_1}{C_2}$ cannot be true
%     which is a contradiction.
%     WLOG, we assume that $x \in \fFootprint{\Xi}{C_1}$ but not $C_2$.
%     % We first assume that $x \in \fFootprint{\Xi}{C_1}$ but not $x^?$.
%     Therefore we have $\fFootprint{\Xi^\prime}{C_1} = \left( \fFootprint{\Xi}{C_1} \right)/x \cup \fFootprint{\G}{\cv{T}}$,
%     and $\fFootprint{\Xi^\prime}{C_2} = \fFootprint{\Xi}{C_2}$.
%     We already have that $\ninterfp{\Xi}{C_1}{C_2}$
%     and therefore the remaining to be shown is
%     $\ninter{\Xi^\prime}{\fFootprint{\G}{\cv{T}}}{\fFootprint{\Xi}{C_2}}$.
%     Note that we already have that
%     $\ninter{\Xi}{x}{\fFootprint{\Xi}{C_2}}$.
%     Therefore, $\forall \tau \in \fFootprint{\Xi}{C_2}$,
%     and given that $|\tau|\ :_{!D_\tau} T_\tau \in \Xi$,
%     $x \in {D_\tau} \vee \tau \in {D} \vee |\tau| \in {D}$ holds.
%     If $x \in {D_\tau}$,
%     we can show that $\fFootprint{\G}{\cv{T}} \subseteq \fFootprint{\Xi^\prime}{D_\tau}$.
%     Therefore, we have $\ninter{\Xi^\prime}{\fFootprint{\G}{\cv{T}}}{\tau}$.
%     Otherwise, if $\tau$ or $| \tau | \in \fFootprint{\G}{D}$,
%     we have $\ninter{\G}{\fFootprint{\G}{\cv{T}}}{\tau}$,
%     which implies that $\ninter{\Xi^\prime}{\fFootprint{\G}{\cv{T}}}{\tau}$
%     by weakening.
%     To summarize,
%     $\forall \tau \in \fFootprint{\Xi}{C_2}$
%     we have $\ninter{\Xi^\prime}{\fFootprint{\G}{\cv{T}}}{\tau}$.
%     As a result, $\ninter{\Xi^\prime}{\fFootprint{\G}{\cv{T}}}{\fFootprint{\Xi^\prime}{C_2}}$
%     and we conclude.

%   \item
%     We first prove the case when $x^? \in \fFootprint{\Xi}{C_1}$
%     and $x^? \in \fFootprint{\Xi}{C_2}$.
%   \end{itemize}
% \end{proof}

% \begin{corollary}[Erasing $!$-annotations in an environment]
%   \label{coro:erase-bang-env}
%   Given $\G$ and $\G^\prime$,
%   if (i) $\forall x :_{!D} \tCap{C_x}{S_x} \in \G^\prime$,
%   either $x :_{!D} \tCap{C_x}{S_x} \in \G$,
%   or $x :_\epsilon \tCap{C_x}{S_x} \in \G$
%   and $\G^\prime = \G_1, x :_{!D} \tCap{C_x}{S_x}, \G_2$ for some $\G_1, \G_2$
%   implies $\ninterfp{\G_1}{D}{C_x}$;
%   and (ii) $\ninterfp{\G^\prime}{C_1}{C_2}$,
%   then $\ninterfp{\G}{C_1}{C_2}$.
% \end{corollary}

% \begin{proof}
% 	By repeated application of Lemma \ref{lemma:erase-bang-ninter}.
% \end{proof}

% \begin{lemma}[Evaluation context typing inversion]  \label{lemma:evctx-typing-inversion}
% 	If
%   (i) $\match{}{\sta}{\G}$,
%   (ii) $\typ{\G}{\evctx{t}}{T}$,
%   then
%   there exists $\Delta, U$,
%   such that
%   (i) $\typec{\G}{e}{\Delta}{U}{\cv{t}}{T}$,
%   and (ii) $\typ{\G, \Delta}{t}{U}$.
% \end{lemma}

% \begin{proof}
%   By induction on $e$.

%   \emph{When $e = []$}.
%   In this case, let $\Delta = \varemptyset$
%   and $U = T$.
%   We conclude immediately.

%   \emph{When $e = \tLetMode{\epsilon}{x}{e^\prime}{u}$}.
%   By induction on the typing derivation,
%   we show that
%   $\typ{\G^\prime}{\evpctx{t}}{T_0}$ for some $T_0$,
%   $\typ{\G^\prime, x :_\epsilon T_0}{u}{T}$,
%   and for any $y :_{!D} T_y \in \G$,
%   either $y \in \bvar{\sta}$,
%   or
%   any $\G_1$ and $\G_2$ such that $\G = \G_1, y :_{!D} T_y, \G_2$
%   implies that $\ninterfp{\G}{D}{\cv{T_y}}$.
%   By applying (\textsc{prom}) repeatedly,
%   we can show that
%   $\typ{\G}{\evpctx{t}}{T_0}$.
%   By IH, $\exists \Delta_0, U_0$ such that
%   $\typec{\G}{e^\prime}{\Delta_0}{U_0}{\cv{t}}{T}$.
%   Notice that $\match{\G}{e}{\Delta_0}$,
%   the remaining to be shown is therefore
%   $\forall s$ such that $\cv{s} = \cv{t}$
%   and $\typ{\G, \Delta_0}{s}{U_0}$
%   we have $\typ{\G}{\tLetMode{\epsilon}{x}{\evpctx{t}}{u}}{T}$.
%   For this we conclude by IH, (\textsc{prom}) and (\textsc{let}).
%   % By inspecting the typing judgment we can show that
%   % $\typ{\G}{\evpctx{t}}{T_0}$ for some $T_0$.
%   % Now we conclude by IH.
%   % Proceed by induction on the derivation of
%   % $\typ{\G}{\tLetMode{\epsilon}{x}{\evpctx{t}}{u}}{T}$.
%   % If it is derived by (\textsc{sub}),
%   % we have
%   % $\typ{\G}{\tLetMode{\epsilon}{x}{\evpctx{t}}{u}}{T_0}$
%   % and $\sub{\G}{T_0}{T}$.
%   % We invoke IH and conclude.
%   % If it is derived by (\textsc{prom}),
%   % we have
%   % $\G = \G_1, y :_\epsilon T_y, \G_2$;
%   % $\ninterfp{\G_1}{D}{\cv{T_y}}$;
%   % and $\typ{\G^\prime}{\tLetMode{\epsilon}{x}{\evpctx{t}}{u}}{T}$
%   % where $\G^\prime = \G_1, y :_{!D} T_y, \G_2$.
%   % Now we invoke IH to show that
%   % there exists $\Delta_0, U_0$ such that
%   % $\typec{\G^\prime}{e^\prime}{\Delta_0}{U_0}{\cv{t}}{T}$,
%   % and $\typ{\G^\prime, \Delta_0}{t}{U_0}$.
%   % Now we invoke (\textsc{prom}) again to show that
%   % $\typ{\G, \Delta_0}{t}{U_0}$.
%   % By Lemma \ref{lemma:binding-prom-match},
%   % we have $\match{\G}{e^\prime}{\Delta_0}$.
%   % The remaining to be proven is that
%   % $\forall s$ such that $\cv{s} = \cv{t}$
%   % and $\typ{\G, \Delta_0}{s}{U_0}$ we have $\typ{\G}{\evctx{s}}{T}$.
%   % We therefore conclude this case.
%   % Finally, if it is derived by (\textsc{let}),
%   % we have $\typ{\G}{\evpctx{t}}{T_0}$ for some $T_0$,
%   % and $\typ{\G, x :_\epsilon T_0}{u}{T}$.
%   % By IH, $\exists \Delta_0, U_0$ such that
%   % $\match{\G}{e^\prime}{\Delta_0}$,
%   % and $\typ{\G, \Delta_0}{t}{U_0}$.
%   % We conclude this case by the fact that
%   % $\match{\G}{e}{\Delta_0}$.

%   \emph{When $e = \tLetVar{x}{e^\prime}{u}$}.
%   As above.

%   \emph{When $e = \tLetMode{!D}{x}{e^\prime}{u}$}.
%   Similar to the previous case.
%   The additional fact to be shown is that
%   $\ninterfp{\G^\prime}{D}{\cv{\evpctx{t}}}$ implies that
%   $\ninterfp{\G}{D}{\cv{\evpctx{t}}}$.
%   We conclude by Corollary \ref{coro:erase-bang-env}.

%   \emph{When $e = \tLetMode{!D}{x}{u}{e^\prime}$}.
%   We similarly analyze the typing derivation.
%   % Proceed by induction on the derivation of
%   % $\typDft{\tLetMode{!D}{x}{u}{\evpctx{t}}}{T}$.
%   % The inductive cases can be concluded as in the previous case.
%   % For the base case, we have
%   % $\typ{\G}{u}{T_0}$ for some $T_0$,
%   % and $\typ{\G, x :_{!D} T_0}{\evpctx{t}}{T}$.
%   Then we invoke IH to show that
%   $\exists \Delta_0, U_0$, such that
%   $\typec{\G, x :_{!D} T_0}{e}{\Delta_0}{U_0}{\cv{t}}{T}$,
%   and $\typ{\G, x :_{!D} T_0, \Delta_0}{t}{U}$.
%   Notice that $\match{\G}{e}{x :_{!D} T_0, \Delta_0}$.
%   This case is therefore concluded by IH, (\textsc{let}) and Corollary \ref{coro:erase-bang-env}.
% \end{proof}

\begin{lemma}[Value lookup inversion: capture set]  \label{lemma:value-lookup-inv-cs}
	If (1) $\match{}{\sta; e}{\G; \Delta}$,
  (2) $\sta(\tVal{x}) = v$
  and (3) $\G(x) = \tCap{C}{S}$,
  then $\sub{\G, \Delta}{\cv{v}}{C}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the matching environment.

  \emph{Case \textsc{empty}}. Conclude immediately.

  \emph{Case \textsc{grow-val}}.
  In this case, $\sta = \sta^\prime, \tVal{y} \mapsto v$,
  $e = []$,
  $\Delta = \Delta^\prime, y :_\epsilon T$,
  $\match{}{\sta^\prime, e}{\Delta^\prime}$,
  and $\typ{\Delta^\prime}{v}{T}$.
  If $x \ne y$, we conclude by IH and Lemma \ref{lemma:typing-weakening}.
  Otherwise if $x = y$,
  we conclude by Lemma \ref{lemma:value-typing-inv-cs} and Lemma \ref{lemma:typing-weakening}.

  \emph{Case \textsc{grow-var}}.
  In this case, $\sta = \sta_0, \tVal{y} \mapsto v$,
  $e = []$,
  $\Delta = \Delta_0, y :_{!} \tCap{\set{*}}{\tRef{S}}$.
  Since $x \in \bval{\sta}$, $x \ne y$.
  We therefore conclude by IH and Lemma \ref{lemma:typing-weakening}.

  \emph{Case \textsc{grow-set}}. As above.

  \emph{Case \textsc{grow-ctx-let} and \textsc{grow-ctx-var}}. By IH.

  \emph{Case \textsc{grow-ctx-par}}.
  We conclude by IH and Lemma \ref{lemma:typing-weakening}.

\end{proof}

\begin{definition}[Resolver of an evaluation context]
  The resolver of an evaluation context $e$,
  written $\fEmbed{e}$,
  is a function mapping from a capture set to another capture set
  given by:
  \begin{equation*}
    \begin{split}
      &\fEmbed{[]}(C) \quad &= \quad &C, \quad&\text{} \\
      &\fEmbed{\tLetMode{m}{x}{e}{u}}(C) \quad &= \quad &\fEmbed{e}(C) \cup \cv{u}/x^*, \quad&\text{} \\
      &\fEmbed{\tLetMode{!}{x}{v}{e}}(C) \quad &= \quad &\fEmbed{e}(C)/x^*, \quad&\text{if $x^* \notin \fEmbed{e}(C)$} \\
      &\fEmbed{\tLetMode{!}{x}{t}{e}}(C) \quad &= \quad &\fEmbed{e}(C)/x^* \cup \cv{t}, \quad&\text{} \\
      &\fEmbed{\tLetVar{x}{e}{u}}(C) \quad &= \quad &\fEmbed{e}(C) \cup \cv{u}/x^*. \quad&\text{} \\
    \end{split}
  \end{equation*}
\end{definition}

\begin{lemma}[Correctness of $\fEmbed{e}$ (I)]
  \label{lemma:e-resolver-correctness-1}
	Given evaluation context $e$,
  and any non-value term $t$,
  $\fEmbed{e}(\cv{t}) = \cv{\evctx{t}}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $e$.
\end{proof}

\begin{lemma}[Correctness of $\fEmbed{e}$ (II)]
  \label{lemma:e-resolver-correctness-2}
	Given evaluation context $e$,
  and any term $t$,
  $\fEmbed{e}(\cv{t}) \subseteq \cv{\evctx{t}}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $e$.
\end{proof}

\begin{lemma}[$\fEmbed{e}$ is monotonic over subcapturing]
  \label{lemma:e-resolver-mono-subcapt}
  If $\sub{\G}{C_1}{C_2}$,
  then $\sub{\G}{\fEmbed{e}(C_1)}{\fEmbed{e}(C_2)}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $e$.
\end{proof}

\begin{lemma}[$\fEmbed{e}$ is monotonic over subset]
  \label{lemma:e-resolver-mono-subset}
  If ${C_1} \subseteq {C_2}$,
  then ${\fEmbed{e}(C_1)} \subseteq {\fEmbed{e}(C_2)}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $e$.
\end{proof}

\begin{lemma}[$\fEmbed{e}$ is homomorphic over set union]
  \label{lemma:e-resolver-homo-union}
	$\fEmbed{e}(C_1 \cup C_2) = \fEmbed{e}(C_1) \cup \fEmbed{e}(C_2)$.
\end{lemma}

\begin{proof}
	By straightforward induction on $e$.
\end{proof}

\begin{lemma}[Evaluation context typing inversion and reification (I)]
  \label{lemma:evctx-reification-1}
  If (i) $\G$ is inert,
  and (ii) $\typ{\G}{\evctx{s}}{T}$ (where $s$ is not a value)
  then $\exists \G_r, \Delta, U$ such that
  (i) $\G_r, \Delta$ is inert and $\G_r \refined \G$,
  (ii) $\typ{\G_r, \Delta}{s}{U}$,
  (iii) $\forall s^\prime$ and an inert $\G^\prime$ such that
  (1) $\typ{\G_r, \G^\prime, \Delta}{s^\prime}{U}$;
  and (2) $\sub{\G_r, \G^\prime, \Delta}{\cv{s^\prime}}{\cv{s}}$;
  we can show that
  $\typ{\G_r, \G^\prime}{\evctx{s^\prime}}{T}$.
\end{lemma}

\begin{proof}
	By induction on $e$.

\item \emph{When $e = []$}.
  Set $\Delta = \varemptyset$
  and $U = T$.
  We conclude immediately.

\item \emph{When $e = \tLetMode{\epsilon}{x}{e^\prime}{u}$}.
  Then $\typ{\G}{\tLetMode{\epsilon}{x}{\evpctx{s}}{u}}{T}$.
  We first show that
  $\typ{\G^\prime}{\evpctx{s}}{T_0}$ for some $T_0$
  and $\typ{\G^\prime, x :_\epsilon T_0}{u}{T}$,
  where $\G^\prime$ is inert and $\G^\prime \refined \G$
  by induction on the typing derivation.
  \begin{itemize}
  \item \emph{Case \textsc{let}}.
    Then $\typ{\G}{\evpctx{s}}{T_0}$ for some $T_0$
    and $\typ{\G, x :_\epsilon T_0}{u}{T}$.
    This case is concluded.

  \item \emph{Case \textsc{prom}}.
    Then $\G = \G_1, y :_{!D} Q, \G_2$ for some $\G_1, \G_2$ and $y$,
    $\typ{\G_1, y :_{!D^\prime} Q, \G_2}{\evctx{s}}{T}$,
    $\ninter{\G_1}{D^\prime}{\fFootprint{\G_1}{\cv{Q}}}$,
    and $D \subseteq D^\prime$.
    By IH we show that there exists $\G^\prime$
    such that $\G^\prime \refined \G_1, y :_{!D^\prime}, \G_2$.
    By Lemma \ref{lemma:refine-trans}
    $\G^\prime \refined \G$.
    This case is therefore concluded.

  \item \emph{Case \textsc{sub}}.
    By IH and \textsc{(sub)}.
  \end{itemize}
  By Lemma \ref{lemma:typ-refined-to-general},
  $\typ{\G}{\evpctx{s}}{T_0}$ for some $T_0$
  and $\typ{\G, x :_\epsilon T_0}{u}{T}$.
  We first invoke IH to show
  $\exists \G_r, \Delta_0, U_0$ satisfying the listed properties.
  % (i) $\match{\G}{e^\prime}{\Delta_0}$,
  % (ii) $\typ{\G, \Delta_0}{s}{U_0}$,
  % (iii) $\forall s^\prime, \G^\prime$ such that
  % (1) $\G^\prime$ is inert;
  % (2) $\typ{\G, \G^\prime, \Delta_0}{s^\prime}{U_0}$;
  % and (3) $\sub{\G, \G^\prime, \Delta_0}{\cv{s^\prime}}{\cv{s}}$;
  % we can show that
  % $\typ{\G, \G^\prime}{\evctx{s^\prime}}{T}$.
  Set $\Delta = \Delta_0$ and $U = U_0$.
  % We can show that $\match{\G}{e}{\Delta}$.
  The goal is that
  given $s^\prime$ and inert $\G^\prime$ such that
  $\typ{\G_r, \G^\prime, \Delta_0}{s^\prime}{U_0}$;
  and $\sub{\G_r, \G^\prime, \Delta_0}{\cv{s^\prime}}{\cv{s}}$,
  by IH we show that $\typ{\G_r, \G^\prime}{\evpctx{s^\prime}}{T_0}$.
  By weakening, we have $\typ{\G_r, \G^\prime, x :_\epsilon T_0}{u}{T}$,
  and we conclude this case by (\textsc{let}).
  % we have to show that $\typ{\G, \G_1^\prime}{\tLetMode{\epsilon}{x}{\evpctx{s^\prime}}{u}}{T}$.
  % We conclude by IH.

  \emph{When $e = \tLetVar{x}{e^\prime}{u}$}. As above.

  \emph{When $e = \tLetMode{!D}{x}{e^\prime}{u}$}.
  Similarly to the previous case,
  by induction on the typing derivation we first show that
  $\typ{\G^\prime}{\evpctx{s}}{T_0}$ for some $T_0$,
  $\typ{\G^\prime, x :_{!D} T_0}{u}{T}$,
  and $\ninterfp{\G^\prime}{(\cv{T_0} \cup \cv{\evpctx{s}})}{D}$,
  where $\G^\prime$ is inert and $\G^\prime \refined \G$.
  % We first show $\ninterfp{\G}{(\cv{T_0} \cup \cv{\evpctx{s}})}{D}$
  % by Corollary \ref{coro:erase-bang-env}.
  We first show that $\sub{\G^\prime}{\cv{\evpctx{s^\prime}}}{\cv{\evpctx{s}}}$
  by Lemma \ref{lemma:e-resolver-mono-subcapt},
  Lemma \ref{lemma:e-resolver-correctness-1},
  and Lemma \ref{lemma:e-resolver-correctness-2}.
  Now we invoke Lemma \ref{lemma:subcapt-pres-ninter} to show that
  $\exists \G^{\prime\prime}.$
  $\G^{\prime\prime} \refined \G^\prime$
  and $\ninterfp{\G^{\prime\prime}}{\cv{\evpctx{s^\prime}}}{D}$.
  % By Lemma \ref{lemma:typ-refined-to-general}
  % we show that
  % $\typ{\G}{\evpctx{s}}{T_0}$.
  Now we invoke Lemma \ref{lemma:typ-refining}
  to show that
  $\typ{\G^{\prime\prime}}{\evpctx{s}}{T_0}$.
  Now we invoke IH on it to show that
  $\exists \G_r, \Delta_0, U_0$ satisfying the listed property.
  Given $s^\prime, \G_0$,
  such that $\G_0$ is inert,
  $\typ{\G_r, \G_0, \Delta}{s^\prime}{U_0}$
  and $\typ{\G_r, \G_0, \Delta}{\cv{s^\prime}}{\cv{s}}$,
  by IH we show that
  $\typ{\G_r, \G_0}{\evpctx{s^\prime}}{T_0}$.
  By Lemma \ref{lemma:typ-refining} and weakening we show that
  $\typ{\G_r, \G_0, x :_{!D} T_0}{u}{T}$,
  and $\ninterfp{\G_r, \G_0}{\cv{\evpctx{s}}}{D}$.
  Now we invoke (\textsc{let}) to show that
  $\typ{\G_r, \G_0}{\evctx{s^\prime}}{T}$.
  % Now by Lemma \ref{lemma:typ-refined-to-general} we show that
  % $\typ{\G, \G_0}{\evctx{s^\prime}}{T}$ and conclude.

  \emph{When $e = \tLetMode{!D}{x}{u}{e^\prime}$}.
  Similarly to the above case,
  we show that
  $\typ{\G^\prime}{u}{T_0}$ for some $T_0$,
  $\typ{\G^\prime, x :_{!D} T_0}{\evpctx{s}}{T}$,
  and $\ninterfp{\G^\prime}{(\cv{T_0} \cup \cv{u})}{D}$,
  where $\G^\prime$ is inert and $\G^\prime \refined \G$.
  % By (\textsc{prom}) we show that
  % $\typ{\G, x :_{\epsilon} T_0}{\evpctx{s}}{T}$,
  % Note that $\G, x :_{\epsilon} T_0$ is inert.
  We invoke IH on the typing derivation
  to show that $\exists \G_r, \Delta_0, U_0$ satisfying the listed properties.
  We set $\Delta = x :_{!D} T_0, \Delta_0$.
  Note that $\G_r, \Delta$ is inert by Lemma \ref{lemma:refining-pres-ninter}.
  For $s^\prime, \G_0$ satisfying those properties,
  by IH we have
  $\typ{\G_r, x :_{!D} T_0}{\evpctx{s^\prime}}{T_0}$.
  By Lemma \ref{lemma:typ-refining} and weakening,
  we can show that
  $\typ{\G_r, \G_0}{u}{T_0}$,
  $\typ{\G_r, \G_0, x :_{!D} T_0}{\evpctx{s^\prime}}{T_0}$,
  and $\ninterfp{\G_r, \G_0}{(\cv{T_0} \cup \cv{u})}{D}$.
  By (\textsc{let}) we have
  $\typ{\G_r, \G_0}{\evctx{s^\prime}}{T}$.
  % Now we conclude by Lemma \ref{lemma:typ-refined-to-general}.
\end{proof}

% \begin{lemma}[Evaluation context typing inversion and reification (I)]  \label{lemma:evctx-reification-1}
%   Given an inert environment $\G_1$,
%   $\typ{\G_1, \G_2}{\evctx{s}}{T}$ (where $s$ is not a value) implies
%   that $\exists \Delta, U$ such that
%   (i) $\match{\G_1, \G_2}{e}{\Delta}$,
%   (ii) $\typ{\G_1, \G_2, \Delta}{s}{U}$,
%   (iii) $\forall s^\prime$ and an inert $\G_1^\prime$ such that
%   (1) $\typ{\G_1, \G_1^\prime, \G_2, \Delta}{s^\prime}{U}$;
%   (2) $\sub{\G_1, \G_1^\prime}{\cv{s^\prime} \cap \dom{\G_1, \G_1^\prime}}{\cv{s} \cap \dom{\G_1, \G_1^\prime}}$;
%   and (3) ${\cv{s^\prime} - \dom{\G_1, \G_1^\prime}} \subseteq {\cv{s} - \dom{\G_1, \G_1^\prime}}$,
%   we can show that
%   then $\typ{\G_1, \G_1^\prime, \G_2}{\evctx{s^\prime}}{T}$.
% \end{lemma}

% \begin{proof}
% 	By induction on $e$.

%   \begin{itemize}
%   \item \emph{When $e = []$}.
%     Set $\Delta = \varemptyset$
%     and $U = T$.
%     We conclude immediately.

%   \item \emph{When $e = \tLetMode{\epsilon}{x}{e^\prime}{u}$}.
%     Let $\G = \G_1, \G_2$.
%     Then $\typ{\G}{\tLetMode{\epsilon}{x}{\evpctx{s}}{u}}{T}$.
%     By induction on the typing derivation,
%     we can show that
%     $\typ{\G^\prime}{\evpctx{s}}{T_0}$ for some $T_0$
%     and $\typ{\G^\prime, x :_\epsilon T_0}{u}{T}$,
%     where $\G^\prime$ is upgraded from $\G$.
%     By repeated application of (\textsc{prom}),
%     we show that $\typ{\G}{\evpctx{s}}{T_0}$,
%     on which we invoke IH.
%     Then, $\exists \Delta_0, U_0$,
%     such that $\match{\G}{e^\prime}{\Delta_0}$,
%     $\typ{\G, \Delta_0}{s}{U_0}$,
%     and $\forall s^\prime, \G_3$ such that
%     $\typ{\G_1, \G_1^\prime, \G_2, \Delta_0}{s^\prime}{U}$,
%     $\sub{\G_1, \G_1^\prime}{\cv{s^\prime} \cap \dom{\G_1, \G_1^\prime}}{\cv{s} \cap \dom{\G_1, \G^\prime}}$,
%     and ${\cv{s^\prime} - \dom{\G_1, \G_1^\prime}} \subseteq {\cv{s} - \dom{\G_1, \G_1^\prime}}$,
%     we have $\typ{\G_1, \G_1^\prime, \G_3}{\evpctx{s}}{T_0}$.
%     Now we show that $\typ{\G_1, \G_1^\prime, \G_3, x :_\epsilon T_0}{u}{T}$ by repeated (\textsc{prom}), weakening,
%     and conclude by IH.

%   \item \emph{When $e = \tLetVar{x}{e^\prime}{u}$}. As above.

%   \item \emph{When $e = \tLetMode{!D}{x}{e^\prime}{u}$}.
%     Similarly to the previous cases.
%     But we have to additionally show that
%     $\ninterfp{\G_1, \G_1^\prime, \G_2}{D}{\cv{\evpctx{s^\prime}}}$
%     from $\ninterfp{\G^\prime}{D}{\cv{\evpctx{s}}}$
%     (note that $\G^\prime$ is defined as above).
%     We first prove that
%     $\ninterfp{\G_1, \G_1^\prime, \G_2}{D}{\cv{\evpctx{s}}}$ by Corollary \ref{coro:erase-bang-env} and weakening.
%     By Lemma \ref{lemma:e-resolver-correctness-1}
%     and Lemma \ref{lemma:e-resolver-correctness-2}
%     we show that $\cv{\evpctx{s}} = \fEmbed{e^\prime}(\cv{s})$,
%     and $\cv{\evpctx{s^\prime}} \subseteq \fEmbed{e^\prime}(\cv{s^\prime})$.
%     Let $\G^+ = \G_1, \G_1^\prime, \G_2$.
%     It suffices to show that
%     $\ninterfp{\G^+}{D}{\fEmbed{e^\prime}(\cv{s^\prime})}$.
%     We first invoke Lemma \ref{lemma:e-resolver-mono-subset}
%     to show that
%     $\fEmbed{e^\prime}(\cv{s^\prime} - \dom{\G_1, \G_1^\prime}) \subseteq \fEmbed{e^\prime}(\cv{s^\prime} - \dom{\G_1, \G_1^\prime})$,
%     from which it follows directly that
%     $\ninterfp{\G^+}{D}{\fEmbed{e^\prime}(\cv{s^\prime} - \dom{\G_1^\prime})}$.
%     Then we invoke Lemma \ref{lemma:e-resolver-mono-subcapt}
%     to show that
%     $\sub{\G_1, \G_1^\prime}{\fEmbed{e^\prime}(\cv{s^\prime} \cap \dom{\G_1, \G_1^\prime})}{\fEmbed{e^\prime}(\cv{s} \cap \dom{\G_1, \G_1^\prime})}$.
%     By Lemma \ref{lemma:subcapt-pres-ninter} we show that
%     $\ninterfp{\G^+}{D}{\fEmbed{e^\prime}(\cv{s^\prime} \cap \dom{\G_1})}$.
%     This case is therefore concluded.

%   \item \emph{When $e = \tLetMode{!D}{x}{u}{e^\prime}$}.
%     Similarly to the previous case,
%     by induction on the typing derivation we can show that
%     $\typ{\G^\prime}{u}{T_0}$,
%     $\typ{\G^\prime, x :_{!D} T_0}{\evpctx{s}}{T}$,
%     and $\ninterfp{\G^\prime}{D}{\cv{T_0}}$.
%     By applying (\textsc{prom}) repeatedly,
%     we have $\typ{\G, x :_{!D} T_0}{\evpctx{s}}{T}$.
%     Now we set $\Delta = x :_{!D} T_0, \Delta_0$
%     Note that $\match{\G}{e}{\Delta}$ and conclude by IH similarly.
%     % Now we invoke IH on it to show that
%     % $\exists \Delta_0, U_0$,
%     % such that $\match{\G, x :_{!D} T_0}{e^\prime}{\Delta_0}$,
%     % $\typ{\G, x :_{!D} T_0, \Delta_0}{s}{U_0}$,
%     % and $\forall s^\prime$ such that
%     % $\typ{\G, x :_{!D} T_0, \Delta_0}{s^\prime}{U}$,
%     % $\sub{\G_1}{\cv{s^\prime} \cap \dom{\G_1}}{\cv{s} \cap \dom{\G_1}}$,
%     % and ${\cv{s^\prime} - \dom{\G_1}} \subseteq {\cv{s} - \dom{\G_1}}$,
%     % we have $\typ{\G, x :_{!D} T_0}{\evpctx{s^\prime}}{T}$.
%     % We set $\Delta = x :_{!D} T_0, \Delta_0$,
%     % and $U = U_0$.
%     % We can first show that $\match{\G}{e}{\Delta}$.
%     % % By induction on the derivation, we can show that $\match{\G}{e}{\Delta}$ by
%     % % IH and (\textsc{prom}) in each case.
%     % Now we show that $\forall s^\prime$ such that
%     % $\typ{\G, x :_{!D} T_0, \Delta_0}{s^\prime}{U}$,
%     % $\sub{\G_1}{\cv{s^\prime} \cap \dom{\G_1}}{\cv{s} \cap \dom{\G_1}}$,
%     % and ${\cv{s^\prime} - \dom{\G_1}} \subseteq {\cv{s} - \dom{\G_1}}$,
%     % we have $\typ{\G}{\tLetMode{!D}{x}{u}{\evpctx{s^\prime}}}{T}$.
%     % Similarly to the previous case,
%     % we can show that $\ninterfp{\G^\prime}{D}{\cv{T_0}}$
%     % implies $\ninterfp{\G}{D}{\cv{T_0}}$
%     % and conclude this case.
%   \end{itemize}
% \end{proof}

% \begin{lemma}[Lifting $!$-bindings]
% 	If
%   (i) $\match{}{\sta; e}{\G; \Delta}$;
%   (ii) $\typ{\G}{\evctx{\tLetMode{!D}{x}{v}{u}}}{T}$;
%   (iii) $\typ{\G}{{\tLetMode{!D}{x}{v}{u}}}{U}$,
%   then $\exists U_0$,
%   such that
%   (i) $\match{}{\sta, \tVal{x} \mapsto v}{\G, x :_\epsilon U_0}$,
%   and (ii) $\typ{\G}{\evctx{u}}{T}$.
% \end{lemma}

\begin{lemma}[Dealiasing $!$-binding preserves non-interference]
  \label{lemma:dealias-bang-pres-ninter}
	If
  (i) $\G$ is inert,
  (ii) $x :_{!D} \tCap{C}{S} \in \G$ (and $* \notin C$),
  and (iii) $\ninter{\G}{x}{F_2}$ ($F_2 \subseteq \domR{\G}$),
  then there exists inert $\G^\prime$,
  $\G^\prime \refined \G$
  and $\ninter{\G^\prime}{\fFootprint{\G^\prime}{C}}{F_2}$.
\end{lemma}

\begin{proof}
  By induction on $\max_{\tau \in F_2} \fDepth{\G}{\tau}$.
  Let $\G^\prime = \G$.
  $\forall \tau \in F_2$ and $|\tau|\ :_{!D_\tau} C_\tau S_\tau \in \G$,
  $\tau \in D \vee |\tau|\ \in D \vee x \in D$.
  If $\tau \in D \vee |\tau|\ \in D_\tau$,
  we have $\ninter{\G^\prime}{\fFootprint{\G^\prime}{C}}{\tau}$.
  Otherwise, we have $x \in D$.
  Therefore, we have $\ninter{\G^\prime}{x}{\fFootprint{\G^\prime}{C_\tau}}$.
  By the wellformedness of $\G$, we have
  $\max{\tau \in C_\tau} \fDepth{\G}{\tau} < \fDepth{\G}{\tau}$,
  and therefore we can invoke IH to show that
  $\exists \G^{\prime\prime}$ such that
  $\G^{\prime\prime} \refined \G^\prime$,
  and $\ninter{\G^{\prime\prime}}{\fFootprint{\G^{\prime\prime}}{C}}{\fFootprint{\G^{\prime\prime}}{C_\tau}}$.
  Let $D_\tau^\prime = D_\tau \cup \fFootprint{\G^{\prime\prime}}{C_\tau}$.
  We set $\G^\prime = \G^{\prime\prime}$
  and further set the binding of $|\tau|$ to $|\tau|\ :_{!D^\prime_\tau} C_\tau\,S_\tau$.
  Therefore $\G^\prime \refined \G$
  and $\G^\prime$ is still inert.
  Therefore we can conclude this case.
\end{proof}

\begin{lemma}[Dealiasing general bindings preserves non-interference]
  \label{lemma:dealiasing-general-pres-ninter}
	If
  (i) $\G$ is inert,
  (ii) $x :_{m} \tCap{C}{S} \in \G$ (and $* \notin C$ if $m =\ {!D}$)
  and (iii) $\ninter{\G}{\fFootprint{\G}{x}}{F_2}$ ($F_2 \subseteq \domR{\G}$),
  then there exists a inert $\G^\prime$,
  $\G^\prime \refined \G$
  and $\ninter{\G^\prime}{\fFootprint{\G^\prime}{x}}{F_2}$.
\end{lemma}

\begin{proof}
	If $m = \epsilon$,
  we have $\fFootprint{\G}{x} = \fFootprint{\G}{C}$.
  We therefore conclude immediately.
  Otherwise, we conclude by Lemma \ref{lemma:dealias-bang-pres-ninter}.
\end{proof}

\begin{lemma}[Evaluation context typing inversion and reification (II)]
  \label{lemma:evctx-reficaition-2}
	If (i) $\G$ is inert,
  and (ii) $\typ{\G}{\evctx{s}}{T}$,
  then $\exists \G_r, \Delta, U$
  such that
  (i) $\G_r, \Delta$ is inert and $\G_r \refined \G$,
  (ii) $\typ{\G_r, \Delta}{s}{U}$,
  and (iii) $\forall s^\prime, \G^\prime$ such that
  $\G_r, \G^\prime$ is inert,
  $\typ{\G_r, \G^\prime, \Delta}{s^\prime}$,
  and $\exists x :_{m} \tCap{C}{S} \in \G. * \notin C \wedge \cv{s^\prime} = \cv{s}[x \mapsto C]$,
  then $\typ{\G_r, \G^\prime}{\evctx{s}}{T}$.
\end{lemma}

\begin{proof}
	Proof proceeds the same way as Lemma \ref{lemma:evctx-reification-1},
  except that Lemma \ref{lemma:dealiasing-general-pres-ninter} should be used.
\end{proof}

\subsection{Substitution}

\subsubsection{Term Substitution}

\begin{lemma}[Term substitution preserves subtyping]
  \label{lemma:term-subst-pres-sub}
	If
  (i) $\sub{\G, x :_m P, \Delta}{T}{U}$,
  (ii) $\typ{\G}{x^\prime}{P}$,
  then $\sub{\G, \theta\Delta}{\theta T}{\theta U}$,
  where $\theta = [x^* \mapsto x^{*\prime}]$.
\end{lemma}

\begin{definition}
	We define $C_1 \sqsubseteq C_2$ as a specialized set inclusion relation
  where $\set{x^?} \sqsubseteq \set{x}$ is accepted.
\end{definition}

\begin{lemma}
  \label{lemma:inert-subcapt-sqsubset}
	Given an inert environment $\G$,
  $\sub{\G}{C_1}{C_2}$ implies
  $\fFootprint{\G}{C_1} \sqsubseteq \fFootprint{\G}{C_2}$.
\end{lemma}

\begin{proof}
	By straightforward induction on the subcapture derivation.
\end{proof}

\begin{lemma}
  \label{lemma:inert-subst-sqsubset}
	Given an inert environment $\G$,
  and $\theta = [x^* \mapsto x^{*\prime}]$,
  if $\typM{\epsilon}{\G}{x^\prime}{P}$,
  then $\fFootprint{\G, \theta\Delta}{\theta C} \sqsubseteq \fFootprint{\G, x :_\epsilon P, \Delta}{C}$.
\end{lemma}

\begin{proof}
	By induction on $\Delta$.

  \emph{Case $\Delta = \varemptyset$}.
  We first consider the case when $x \in C$.
  Therefore, $\fFootprint{\G}{\theta C} = \fFootprint{\G}{(C/x)} \cup \fFootprint{\G}{\cv{P^\prime}}$
  (if $x^\prime :_\epsilon P^\prime \in \G$),
  and $\fFootprint{\G}{C} = \fFootprint{\G}{(C/x)} \cup \fFootprint{\G}{\cv{P}}$.
  By inspecting the typing judgment we can show that $\sub{\G}{\cv{P^\prime}}{\cv{P}}$.
  Now we conclude by Lemma \ref{lemma:inert-subcapt-sqsubset}.
  The cases when $x^? \in C$ and $x^* \notin C$ is concluded similarly.

  \emph{Case $\Delta = \Delta^\prime, y :_\epsilon T$}.
  We have $\fFootprint{\G, x :_\epsilon P, \Delta}{y} = \fFootprint{\G, x :_\epsilon P, \Delta^\prime}{\cv{T}}$,
  and $\fFootprint{\G, \theta\Delta}{y} = \fFootprint{\G, \theta\Delta^\prime}{\theta\cv{T}}$.
  This case is therefore concluded by IH.

  \emph{Case $\Delta = \Delta^\prime, y :_{!D} T$}.
  We have $\fFootprint{\G, x :_\epsilon P, \Delta}{y} = \set{y}$,
  and $\fFootprint{\G, \theta\Delta}{y} = \set{y}$.
  We therefore conclude this case by IH as well.
\end{proof}

% \begin{lemma}[Term substitution preserves $\sqsubseteq$]
%   \label{lemma:term-subst-pres-sqsubset}
% 	Given an inert environment $\G$,
%   and $\theta = [x^* \mapsto x^{*\prime}]$,
%   if (i) $\typM{\epsilon}{\G}{x^\prime}{P}$,
%   and (ii) $\fFootprint{\G, x :_\epsilon P, \Delta}{C_1} \sqsubseteq \fFootprint{\G, x :_\epsilon P, \Delta}{C_2}$
%   then $\fFootprint{\G, \theta\Delta}{\theta C_1} \sqsubseteq \fFootprint{\G, \theta\Delta}{\theta C_2}$.
% \end{lemma}

% \begin{proof}
% 	By induction on $\Delta$.

%   \emph{When $\Delta = \varemptyset$}.
% \end{proof}

% \begin{lemma}[Term substitution preserves non-interference ($\epsilon$)]
%   \label{lemma:term-subst-pres-ninter}
%   Given an inert environment $\G$,
%   and $\theta = [x^* \mapsto x^{*\prime}]$,
%   if (i) $\ninterfp{\G, x :_\epsilon P, \Delta}{C_1}{C_2}$,
%   and (ii) $\typM{\epsilon}{\G}{x^\prime}{P}$,
%   then $\exists \G_r$ such that
%   $\G_r$ is inert,
%   $\G_r \refined \G$,
%   and $\ninterfp{\G_r, \theta\Delta}{(\theta C_1)}{(\theta C_2)}$.
% \end{lemma}

% \begin{proof}
% 	By induction on $|\Delta|$.

%   \emph{Case $\Delta = \varemptyset$}.
%   We first assume that $x$ is in both $C_1$ and $C_2$.
%   Then $\fFootprint{\G}{\theta C_i} = \fFootprint{\G}(C_i/x) \cup \fFootprint{\G}{x^\prime}$.
%   Note that $\fFootprint{\G, x :_\epsilon P}{C_i} = \fFootprint{\G}{C_i/x} \cup \fFootprint{\G}{\cv{P}}$.
%   By inspecting $\typM{\epsilon}{\G}{x^\prime}{P}$ we have that
%   $x :_\epsilon P^\prime \in \G$ and $\sub{\G}{P^\prime}{P}$,
%   from which we can show that $\sub{\G}{\cv{P^\prime}}{\cv{P}}$.
%   Also, $\fFootprint{\G}{\theta C_i} = \fFootprint{\G}(C_i/x) \cup \fFootprint{\G}{\cv{P^\prime}}$.
%   This case can therefore be concluded by Lemma \ref{lemma:subcapt-pres-ninter}.
%   The cases when $x^*$ is only in one of $C_i$ and when $x^?$ is a member of $C_i$
%   can be concluded similarly.

%   \emph{Case $\Delta = \Delta^\prime, y :_\epsilon T$}.
%   In this case,
%   $\fFootprint{\G, x :_\epsilon P, \Delta^\prime, y :_\epsilon T}{y} = \fFootprint{\G, x :_\epsilon P, \Delta^\prime}{\cv{T}}$
%   and $\fFootprint{\G, \theta\Delta^\prime, y :_\epsilon \theta T}{y} = \fFootprint{\G, \theta\Delta^\prime}{\theta\cv{T}}$.
%   We can therefore conclude by IH if $y^*$ is in either of $C_i$.

%   \emph{Case $\Delta = \Delta^\prime, y :_{!D} T$}.
%   We first prove the case when $y \in C_1$ and $y^* \notin C_2$.
%   In this case,
%   we have $\ninter{\G, x :_\epsilon P, \Delta, y :_{!D} T}{y}{\fFootprint{\G, x :_\epsilon P, \Delta}{C_2}}$.
%   By the wellformedness of the environment,
%   $y^* \notin \fFootprint{\G, x :_\epsilon P, \Delta}{C_2}$.
%   therefore the above condition is equivalent to
%   $\forall \tau \in \fFootprint{\G, x :_\epsilon P, \Delta}{C_2}$,
%   $\tau \in {D}$ or
%   $|\tau| \in {D}$,
%   which means that $\fFootprint{\G, x :_\epsilon P, \Delta}{C_2} \sqsubseteq {D}$.
%   And it suffices to show that
%   $\ninter{\G, \theta\Delta, y :_{!\theta D} T}{y}{\fFootprint{\G, \theta\Delta}{\theta C_2}}$,
%   which is equivalent to
%   $\fFootprint{\G, \theta\Delta}{\theta C_2} \sqsubseteq {\theta D}$.
%   Note that since $D \subseteq \domR{\G, \Delta}$,
%   we can show that $\theta \Delta = \Delta$.
%   % $\forall \tau \in \fFootprint{\G, \theta\Delta}{C_2}$,
%   % $\tau \in \fFootprint{\G, \theta\Delta}{\theta D}$ or
%   % $|\tau| \in \fFootprint{\G, \theta\Delta}{\theta D}$.
%   By Lemma \ref{lemma:inert-subst-sqsubset},
%   we have $\fFootprint{\G, \theta\Delta}{\theta C_2} \sqsubseteq \fFootprint{\G, x :_\epsilon P, \Delta}{C_2}$.
%   Since $\sqsubseteq$ is transitive,
%   now we can show that $\fFootprint{\G, \theta\Delta}{\theta C_2} \sqsubseteq {\theta D}$
%   and conclude this case.
%   When $y^*$ is a member of both $C_1, C_2$,
%   we can show that $y^? \in C_1, C_2$ but not $y$,
%   otherwise a contradiction can be derived.
%   We can conclude this case similarly to the previous one.
% \end{proof}

% \begin{lemma}[Term substitution preserves typing ($\epsilon$)]
%   \label{lemma:term-subst-pres-typing}
%   Given an inert environment $\G$,
%   if
%   (i) $\typ{\G, x :_\epsilon P, \Delta}{t}{T}$,
%   and (ii) $\typM{\epsilon}{\G}{x^\prime}{P}$,
%   then
%   $\typ{\G, [x^* \mapsto x^{*\prime}] \Delta}{[x^* \mapsto x^{*\prime}]t}{[x^* \mapsto x^{*\prime}]T}$.
% \end{lemma}

% \begin{proof}
% 	Let $\theta = [x^* \mapsto x^{*\prime}]$.
%   Proof proceeds by induction on the typing derivation.

%   \emph{Case \textsc{var}}.
%   In this case, $t = y$ for some $y$,
%   $y : \tCap{C}{S} \in (\G, x :_\epsilon P, \Delta)$,
%   and $T = \tCap{\set{y}}{S}$.
%   The goal is to show that
%   $\typ{\G, \theta\Delta}{\theta y}{\tCap{\set{\theta y}}{\theta S}}$.
%   \begin{itemize}
%   \item \emph{When $x = y$}.
%     $P = \tCap{C}{S}$
%     and the goal becomes $\typ{\G, \theta\Delta}{x^\prime}{\tCap{\set{x^\prime}}{S}}$
%     (note that $\theta S = S$ by the well-formedness of $\G$)
%     and we conclude by (\textsc{var}).

%   \item \emph{When $x \ne y$}.
%     Now we inspect where $y$ is bound.
%     If $y \in \dom{\G}$,
%     we have $x \notin \fv{\tCap{C}{S}}$ by the well-formedness of $\G$
%     and therefore $\theta \tCap{C}{S} = \tCap{C}{S}$
%     and we conclude by (\textsc{var}).
%     Otherwise if $y \in \dom{\Delta}$,
%     we have $\theta \tCap{C}{S} = \tCap{\theta C}{\theta S}$
%     and we conclude by (\textsc{var}) as well.
%   \end{itemize}

%   \emph{Case \textsc{sub}}.
%   By IH, Lemma \ref{lemma:term-subst-pres-sub}
%   and (\textsc{sub}).

%   \emph{Case \textsc{abs} and \textsc{tabs}}.
%   By IH and the same rule.

%   \emph{Case \textsc{app}}.
%   Then
%   $t = y_1\, y_2$ for some $y_1, y_2$,
%   $\typ{\G, x :_\epsilon P, \Delta}{y_1}{C\,\forall(z: U)T^\prime}$
%   and $\typ{\G, x :_\epsilon P, \Delta}{y_2}{U}$.
%   Now we invoke IH to show that
%   $\typ{\G, \theta\Delta}{\theta y_1}{\theta(C\,\forall(z: U)T^\prime)}$,
%   and $\typ{\G, \theta\Delta}{\theta y_2}{\theta U}$.
%   By (\textsc{app}) we show that
%   $\typ{\G, \theta\Delta}{\theta(y_1\,y_2)}{[z \mapsto \theta y_2]T^\prime}$.
%   Now we conclude by the fact that $[z \mapsto \theta y_2]T^\prime = \theta([z \mapsto y_2] T^\prime)$.

%   \emph{Case \textsc{tapp}}.
%   As above.

%   \emph{Case \textsc{box}}.
%   Then $t = \Box y$,
%   $\typ{\G, x :_\epsilon P, \Delta}{y}{\tCap{C}{S}}$,
%   $T = \Box \tCap{C}{S}$,
%   and $C \subseteq \dom{\G, x :_\epsilon P, \Delta}$.
%   By IH we have
%   $\typ{\G, \theta\Delta}{\theta y}{\theta(\tCap{C}{S})}$.
%   If $x \notin C$, we have $\theta C = C$
%   and invoke (\textsc{box}) to conclude this case.
%   Otherwise, $\theta C = C/x \cup x^\prime$.
%   We can show that $\theta C \subseteq \dom{\G, \theta\Delta}$
%   and again conclude by (\textsc{box}).

%   \emph{Case \textsc{unbox}}.
%   As above.

%   \emph{Case \textsc{let}}.
%   In this case, $t = \tLetMode{m}{y}{s}{u}$,
%   $\typ{\G, x :_\epsilon P, \Delta}{s}{U}$,
%   $\typ{\G, x :_\epsilon P, \Delta, y :_m U}{u}{T}$,
%   $y \notin \fv{T}$,
%   and $\ninterfp{\G, x :_\epsilon P, \Delta}{(\cv{U} \cup \cv{s})}{D}$ if $m = \ !D$.
%   By IH we have
%   $\typ{\G, \theta\Delta}{\theta s}{\theta U}$,
%   and $\typ{\G, \theta\Delta, y :_{\theta m} \theta U}{\theta u}{\theta T}$,
%   and also $y \notin \fv{T}$ since $y$ is fresh.
%   To invoke (\textsc{let}) again,
%   the remaining to be shown is that
%   $\ninter{\G, \theta\Delta}{\fFootprint{\G, \theta\Delta}{\theta(\cv{U} \cup \cv{s})}}{\theta D}$.
%   Now we invoke Lemma \ref{lemma:term-subst-pres-ninter}
%   to show that $\exists \G_r$
%   such that
%   $\G_r$ is inert,
%   $\G_r \refined \G$,
%   $\ninterfp{\G_r, \theta\Delta}{\fFootprint{\G_r, \theta\Delta}{\theta(\cv{U} \cup \cv{s})}}{\theta D}$.
%   By Lemma \ref{lemma:typ-refining},
%   we have
%   $\typ{\G_r, \theta\Delta}{\theta s}{\theta U}$,
%   and $\typ{\G_r, \theta\Delta, y :_{\theta m} \theta U}{\theta u}{\theta T}$.
%   By (\textsc{let}),
%   we can show that
%   $\typ{\G_r, \theta\Delta}{\theta t}{\theta T}$.
%   Now we conclude this case by Lemma \ref{lemma:typ-refined-to-general}.

%   \emph{Case \textsc{prom}}.
%   There is $\G_r \refined \G, x :_{\epsilon} P, \Delta$,
%   and in $\G_r$ is obtained by upgrading the non-conflicting domain
%   of one binding $y$ in $\G, x :_{\epsilon} P, \Delta$.
%   We split the cases based on where $y$ is bound.
%   If $y$ is bound in $\G$,
%   then $\G, x :_{\epsilon} P, \Delta = \G_1, y :_{!D} Q, \G_2, x :_{\epsilon} P, \Delta$,
%   and we have $\typ{\G_1, y :_{!D^\prime} Q, \G_2, \theta\Delta}{\theta t}{\theta T}$.
%   We can conclude this case by (\textsc{prom}).
%   Otherwise, if $y$ is bound in $\Delta$,
%   then $\G, x :_{!\epsilon} P, \Delta = \G, x :_{\epsilon} P, \Delta_1, y :_{!D} Q, \Delta_2$.
%   By IH we have
%   $\typ{\G, \theta \Delta_1, y :_{!\theta D^\prime} \theta Q, \Delta_2}{\theta t}{\theta T}$.
% \end{proof}

\begin{lemma}[Term substitution preserves non-interference ($!$)]
  \label{lemma:term-subst-pres-ninter-bang}
  If
  (i) $\ninterfp{\G, x :_{!D} P, \Delta}{C_1}{C_2}$
  (ii) $\typM{!D}{\G}{x^\prime}{P}$,
  % and (iii) $\G, x :_{!D} P$ is inert,
  then $\ninterfp{\G, \theta\Delta}{\theta C_1}{\theta C_2}$.
\end{lemma}

\begin{proof}
	Proceed by a case analysis on whether or not $x^*$ is a member of $\fFootprint{\G, x :_{!D} P, \Delta}{C_i}$.

  \begin{itemize}
  \item \emph{When $x^* \in \fFootprint{\G, x :_{!D} P, \Delta}{C_1}$ but not $C_2$}.
    We first assume that $x \in \fFootprint{\G, x :_{!D} P, \Delta}{C_1}$
    but not $x^?$.
    By inspecting the typing judgment $\typM{!D}{\G}{x^\prime}{P}$,
    we can show that $x^\prime :_{!D^\prime} P^\prime$
    where $D \subseteq D^\prime$
    and $\sub{\G}{\cv{P^\prime}}{\cv{P}}$.
    We can show that $\fFootprint{\G, \theta\Delta}{C_1} = (\fFootprint{\G, x :_{!D} P, \Delta}{C_1})/x \cup \set{x^\prime}$.
    From the premise we can already show that
    (i) $\ninter{\G, x :_{!D} P, \Delta}{(\fFootprint{\G, x :_{!D} P, \Delta}{C_1})/x}{\fFootprint{\G, x :_{!D} P, \Delta}{C_2}}$;
    and (ii) $\ninter{\G, x :_{!D} P, \Delta}{\set{x}}{\fFootprint{\G, x :_{!D} P, \Delta}{C_2}}$.
    Now the goal becomes $\ninter{\G, \theta\Delta}{\set{x^\prime}}{\fFootprint{\G, \theta\Delta}{\theta C_2}}$.
    Since $x^* \notin \fFootprint{\G, x :_{!D} P, \Delta}{C_2}$
    we can show that $\fFootprint{\G, \theta\Delta}{\theta C_2} = \fFootprint{\G, x :_{!D} P, \Delta}{C_2}$.
    Let it be $F_2$.
    We have to show that $\forall \tau \in F_2$ where $|\tau|\ :_{!\theta D_\tau} T_\tau \in \G, \theta\Delta$,
    either $\tau \in D^\prime$ or $|\tau| \ \in D^\prime$ or $x^\prime \in \theta D_\tau$.
    Note that $\tau \in D$ or $|\tau| \ \in D$ implies that
    $\tau \in D^\prime$ or $|\tau| \ \in D^\prime$.
    Also, $x \in D_\tau$ implies that $x^\prime \in \theta D_\tau$.
    We can there conclude this case.
    The case when $x^?$ is a member of the footprint follows similarly.

  \item \emph{When $x^*$ is a member of the footprint of $C_2$ but not $C_1$}.
    As above.

  \item \emph{When $x^*$ is a member of both footprints}.
    Then we can first show that $x^?$ is a member of these two footprints
    but not $x$.
    Otherwise a contradiction will be derived.
    Then this case can be concluded as above.
  \end{itemize}
\end{proof}

\begin{lemma}[Term substitution preserves typing ($!$)]
  \label{lemma:term-subst-pres-typing-bang}
  Given an inert environment $\G$,
	if (i) $\typ{\G, x :_{!D} P, \Delta}{t}{T}$,
  and (ii) $\typM{!D}{\G}{x^\prime}{P}$,
  % and (iii) $\G, x :_{!D} P$ is inert,
  then $\typ{\G, \theta\Delta}{\theta t}{\theta T}$,
  where $\theta = [x^* \mapsto x^{*\prime}]$.
\end{lemma}

\begin{proof}
  % The proof follows the same way as proof of Lemma \ref{lemma:term-subst-pres-typing}
  % except that Lemma \ref{lemma:term-subst-pres-ninter-bang} is used in the (\textsc{let}) case.

	Let $\theta = [x^* \mapsto x^{*\prime}]$.
  Proof proceeds by induction on the typing derivation.

  \emph{Case \textsc{var}}.
  In this case, $t = y$ for some $y$,
  $y : \tCap{C}{S} \in (\G, x :_\epsilon P, \Delta)$,
  and $T = \tCap{\set{y}}{S}$.
  The goal is to show that
  $\typ{\G, \theta\Delta}{\theta y}{\tCap{\set{\theta y}}{\theta S}}$.
  \begin{itemize}
  \item \emph{When $x = y$}.
    $P = \tCap{C}{S}$
    and the goal becomes $\typ{\G, \theta\Delta}{x^\prime}{\tCap{\set{x^\prime}}{S}}$
    (note that $\theta S = S$ by the well-formedness of $\G$)
    and we conclude by (\textsc{var}).

  \item \emph{When $x \ne y$}.
    Now we inspect where $y$ is bound.
    If $y \in \dom{\G}$,
    we have $x \notin \fv{\tCap{C}{S}}$ by the well-formedness of $\G$
    and therefore $\theta \tCap{C}{S} = \tCap{C}{S}$
    and we conclude by (\textsc{var}).
    Otherwise if $y \in \dom{\Delta}$,
    we have $\theta \tCap{C}{S} = \tCap{\theta C}{\theta S}$
    and we conclude by (\textsc{var}) as well.
  \end{itemize}

  \emph{Case \textsc{sub}}.
  By IH, Lemma \ref{lemma:term-subst-pres-sub}
  and (\textsc{sub}).

  \emph{Case \textsc{abs} and \textsc{tabs}}.
  By IH and the same rule.

  \emph{Case \textsc{app}}.
  Then
  $t = y_1\, y_2$ for some $y_1, y_2$,
  $\typ{\G, x :_\epsilon P, \Delta}{y_1}{C\,\forall(z: U)T^\prime}$
  and $\typ{\G, x :_\epsilon P, \Delta}{y_2}{U}$.
  Now we invoke IH to show that
  $\typ{\G, \theta\Delta}{\theta y_1}{\theta(C\,\forall(z: U)T^\prime)}$,
  and $\typ{\G, \theta\Delta}{\theta y_2}{\theta U}$.
  By (\textsc{app}) we show that
  $\typ{\G, \theta\Delta}{\theta(y_1\,y_2)}{[z \mapsto \theta y_2]T^\prime}$.
  Now we conclude by the fact that $[z \mapsto \theta y_2]T^\prime = \theta([z \mapsto y_2] T^\prime)$.

  \emph{Case \textsc{tapp}}.
  As above.

  \emph{Case \textsc{box}}.
  Then $t = \Box y$,
  $\typ{\G, x :_\epsilon P, \Delta}{y}{\tCap{C}{S}}$,
  $T = \Box \tCap{C}{S}$,
  and $C \subseteq \dom{\G, x :_\epsilon P, \Delta}$.
  By IH we have
  $\typ{\G, \theta\Delta}{\theta y}{\theta(\tCap{C}{S})}$.
  If $x \notin C$, we have $\theta C = C$
  and invoke (\textsc{box}) to conclude this case.
  Otherwise, $\theta C = C/x \cup x^\prime$.
  We can show that $\theta C \subseteq \dom{\G, \theta\Delta}$
  and again conclude by (\textsc{box}).

  \emph{Case \textsc{unbox}}.
  As above.

  \emph{Case \textsc{let}}.
  In this case, $t = \tLetMode{m}{y}{s}{u}$,
  $\typ{\G, x :_{!D} P, \Delta}{s}{U}$,
  $\typ{\G, x :_{!D} P, \Delta, y :_m U}{u}{T}$,
  $y \notin \fv{T}$,
  and $\ninter{\G, x :_{!D} P, \Delta}{\fFootprint{\G, x :_{!D} P, \Delta}{\cv{U}}}{D_1}$
  and $\ninterfp{\G, x :_{!D} P, \Delta}{\cv{s}}{\cv{u}/x}$
  if $m = \ !D_1$.
  By IH we have
  $\typ{\G, \theta\Delta}{\theta s}{\theta U}$,
  and $\typ{\G, \theta\Delta, y :_{\theta m} \theta U}{\theta u}{\theta T}$,
  and also $y \notin \fv{T}$ since $y$ is fresh.
  To invoke (\textsc{let}) again,
  the remaining to be shown is that
  $\ninter{\G, \theta\Delta}{\fFootprint{\G, \theta\Delta}{\theta\cv{U}}}{\theta D_1}$
  and $\ninterfp{\G, \theta\Delta}{\theta\cv{s}}{\theta{\cv{u}}/x}$.
  Now we invoke Lemma \ref{lemma:term-subst-pres-ninter} twice
  to show that $\exists \G_r$
  such that
  $\G_r$ is inert,
  $\G_r \refined \G$,
  % $\ninterfp{\G_r, \theta\Delta}{\fFootprint{\G_r, \theta\Delta}{\theta(\cv{U} \cup \cv{s})}}{\theta D}$.
  $\ninter{\G_r, \theta\Delta}{\fFootprint{\G, \theta\Delta}{\theta\cv{U}}}{\theta D_1}$
  and $\ninterfp{\G_r, \theta\Delta}{\theta\cv{s}}{\theta{\cv{u}}/x}$.
  By Lemma \ref{lemma:typ-refining},
  we have
  $\typ{\G_r, \theta\Delta}{\theta s}{\theta U}$,
  and $\typ{\G_r, \theta\Delta, y :_{\theta m} \theta U}{\theta u}{\theta T}$.
  By (\textsc{let}),
  we can show that
  $\typ{\G_r, \theta\Delta}{\theta t}{\theta T}$.
  Now we conclude this case by Lemma \ref{lemma:typ-refined-to-general}.

  \emph{Case \textsc{prom}}.
  There is $\G_r \refined \G, x :_{!D} P, \Delta$,
  and in $\G_r$ is obtained by upgrading the non-conflicting domain
  of one binding $y$ in $\G, x :_{!D} P, \Delta$.
  We split the cases based on where $y$ is bound.
  If $y$ is bound in $\G$,
  then $\G, x :_{!D} P, \Delta = \G_1, y :_{!E} Q, \G_2, x :_{!D} P, \Delta$,
  and we have $\typ{\G_1, y :_{!E^\prime} Q, \G_2, \theta\Delta}{\theta t}{\theta T}$.
  We can conclude this case by (\textsc{prom}).
  If $y$ is bound in $\Delta$,
  then $\G, x :_{!D} P, \Delta = \G, x :_{!D} P, \Delta_1, y :_{!E} Q, \Delta_2$.
  By IH we have
  $\typ{\G, \theta \Delta_1, y :_{!\theta E^\prime} \theta Q, \theta\Delta_2}{\theta t}{\theta T}$.
  Now we invoke Lemma \ref{lemma:term-subst-pres-ninter-bang} to show that
  $\ninter{\G, \theta \Delta_1}{\theta E^\prime}{\theta \cv{Q}}$.
  Therefore we can invoke (\textsc{prom}) to conclude this case.
\end{proof}

\begin{lemma}[Term substitution preserves typing ($!-\epsilon$)]
  \label{lemma:term-subst-pres-typing-bang}
  Given an inert environment $\G$,
	if (i) $\typ{\G, x :_{\epsilon} P, \Delta}{t}{T}$,
  and (ii) $\typM{!D}{\G}{x^\prime}{P}$,
  then $\typ{\G, \theta\Delta}{\theta t}{\theta T}$,
  where $\theta = [x^* \mapsto x^{*\prime}]$.
\end{lemma}

\subsection{Main Theorems}

\begin{lemma}[Lookup inversion: unbox]  \label{lemma:lookup-inversion-unbox}
	If
  (i) $\match{}{\sta}{\G}$,
  (ii) $\typ{\G, \Delta}{x}{\Box\ \tCap{C}{S}}$,
  and (iii) $\sta(\tVal{x}) = \Box\ y$,
  then
  $\typ{\G, \Delta}{y}{\tCap{C}{S}}$.
\end{lemma}

\begin{lemma}[Lookup inversion: term abstraction]
  \label{lemma:lookup-inversion-fun}
	If
  (i) $\match{}{\sta}{\G}$,
  (ii) $\typ{\G, \Delta}{x}{C\,\forall(z:_m T) U}$,
  and (iii) $\sta(\tVal{x}) = \lambda(z:_m T^\prime) t$,
  then
  $\typ{\G, \Delta}{T}{T^\prime}$
  and $\typ{\G, \Delta, z : T^\prime}{t}{U}$.
\end{lemma}

\begin{theorem}[Preservation]
  If
  (i) $\match{}{\sta}{\G}$,
  (ii) $\typDft{t}{T}$,
  and (iii) $\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}$,
  then
  $\exists \G^\prime$, such that
  (i) $\match{}{\sta^\prime}{\G^\prime}$,
  and (ii) $\typ{\G^\prime}{t^\prime}{T}$.
\end{theorem}

\begin{proof}
  By case analysis on the reduction derivation.

  \emph{Case \textsc{apply-$!$}}.
  % In this case,
  % $t = \evctx{x\, y}$.
  % We first invoke Lemma \ref{lemma:evctx-typing-inversion},
  % to show that
  % $\exists \Delta, Q$ such that
  % (i) $\match{\G}{e}{\Delta}$,
  % and (ii) $\typ{\G, \Delta}{x\,y}{Q}$.
  Then $t = \evctx{x\, y}$,
  $\sta(\tVal{x}) = \lambda(z:_{!D} U) s$,
  and $t^\prime = \evctx{[y/z] s}$.
  First of all,
  we invoke Lemma \ref{lemma:evctx-reficaition-2},
  and show that
  there exists $\G_r, \Delta, Q$ such that
  $\G_r, \Delta$ is inert,
  $\G_r \refined \G$,
  $\typ{\G_r, \Delta}{x\,y}{Q}$
  and $\forall s^\prime$ such that
  (i) $\typ{\G_r, \Delta}{s^\prime}{Q}$
  and (ii) $\cv{s^\prime} = \cv{s}[z \mapsto \cv{P}]$
  for some $z :_m P \in \G$ and $* \notin \cv{P}$,
  we have $\typ{\G_r}{\evctx{s^\prime}}{Q}$.
  Now we inspect the typing derivation,
  we show that
  $\typ{\G^\prime}{x}{C\,\forall(z:_{!D} U^\prime) Q^\prime}$ (where $Q = [y/z]Q^\prime$),
  and $\typM{!D}{\G^\prime}{y}{U^\prime}$,
  where $\G^\prime$ is inert and $\G^\prime \refined \G_r, \Delta$.
  By Lemma \ref{lemma:lookup-inversion-fun},
  we show that
  $\typ{\G^\prime, z :_m U}{s}{Q^\prime}$
  and $\sub{\G,^\prime}{U^\prime}{U}$.
  % If $m = \epsilon$,
  % we invoke Lemma \ref{lemma:term-subst-pres-typing}
  % to show that
  % $\typ{\G^\prime}{[y/z]s}{[y/z]Q^\prime}$.
  % Otherwise, if $m = !D$,
  Now we invoke Lemma \ref{lemma:term-subst-pres-typing-bang}
  to show that
  $\typ{\G^\prime}{[y/z]s}{[y/z]Q^\prime}$ too.
  By Lemma \ref{lemma:typ-refined-to-general},
  we show that
  $\typ{\G_r, \Delta}{[y/z]s}{Q}$. %in both cases.
  Now that $\cv{[y/z]s} = \set{x, y}[x \mapsto (\cv{s}/z)]$.
  Since $\match{}{\sta}{\G}$,
  we have $C = \cv{s}/z$.
  Now we can invoke the reification lemma to show that
  $\typ{\G_r}{\evctx{s}}{T}$.
  Now we conclude this case by Lemma \ref{lemma:typ-refined-to-general}.

  \emph{Case \textsc{apply-$\epsilon$}}.
  Then $t = \evctx{x\,y}$,
  $\sta(\tVal{x}) = \lambda(z:_\epsilon U) s$,
  $\sta(\tVal{y}) = v$,
  $\sta^\prime = \sta, \tValM{\epsilon} z \mapsto v$,
  and $t^\prime = s$.
  First,
  we invoke Lemma \ref{lemma:evctx-reification-1}
  to show that $\exists \G_r, \Delta, Q$
  such that $\G_r, \Delta$ is inert,
  $\typ{\G_r, \Delta}{x\,y}{Q}$,
  and $\forall s^\prime, \G^\prime$ such that
  $\G_r, \G^\prime$ is inert,
  $\typ{\G_r, \G^\prime, \Delta}{s^\prime}{Q}$,
  and $\cv{s^\prime} = \set{x, y}[z \mapsto \cv{P}]$
  for some $z :_m P \in \G$,
  we have $\typ{\G_r, \G^\prime}{\evctx{s^\prime}}{T}$.
  By inspecting the derivation of
  $\typ{\G_r, \Delta}{x\,y}{Q}$,
  we show that
  $\typ{\G_r, \Delta}{x}{C\,\forall(z:_\epsilon U^\prime) Q^\prime}$,
  and $\typ{\G_r, \Delta}{y}{U^\prime}$.
  By Lemma \ref{lemma:lookup-inversion-fun},
  we have
  $\typ{\G_r, \Delta, z :_\epsilon U}{s}{Q^\prime}$,
  and $\sub{\G_r, \Delta}{U^\prime}{U}$.

  \emph{Case \textsc{tapply}}.
  As above.

  \emph{Case \textsc{open}}.
  In this case,
  $t = \evctx{\tUnbox{C}{x}}$,
  and $\sta(\tVal{x}) = \Box\ {y}$.
  Since $\match{}{\sta}{\G}$,
  $\G$ is inert.
  We can invoke Lemma \ref{lemma:evctx-reification-1},
  to show that
  $\exists \G_r, \Delta, Q$ such that
  (i) $\G_r, \Delta$ is inert and $\G_r \refined \Delta$,
  % $\match{\G}{e}{\Delta}$,
  (ii) $\typ{\G_r, \Delta}{\tUnbox{C}{x}}{Q}$,
  and (iii) $\forall s^\prime$ such that
  $\typ{\G_r, \Delta}{s^\prime}{Q}$ and
  $\sub{\G_r}{\cv{s^\prime}}{C \cup \set{x}}$
  we have $\typ{\G_r}{\evctx{s^\prime}}{T}$.
  By inspecting the typing derivation,
  we can show that
  $\typ{\G_r, \Delta}{x}{\Box\,\tCap{C}{S}}$ for some $S$
  and $C \subseteq \dom{\G, \Delta}$.
  Now we invoke Lemma \ref{lemma:lookup-inversion-unbox}
  and show that $\typ{\G_r, \Delta}{y}{\tCap{C}{S}}$.
  By the well-formedness of $\sta$,
  we have $y \in \dom{\G}$.
  If $y \in \bvar{\G}$,
  we have $y :_{!D} \tCap{\set{*}}{S_y} \in \G$
  and $\sub{\G_r, \Delta}{\set{*}}{C}$,
  which implies that $* \in C$.
  This contradicts with $C \subseteq \dom{\G, \Delta}$.
  Therefore, $y \in \bval{\G}$,
  and we assume that $\sta(\tVal{y}) = v$.
  By Lemma \ref{lemma:value-lookup-inv-cs},
  $\sub{\G_r, \Delta}{\cv{v}}{C}$.
  % Based on the well-formedness of $\G$,
  % $\cv{v} \subseteq \dom{\G}$.
  % By induction on the subcapture derivation,
  % we can show that there exists $C_0 \subseteq C$ such that
  % $C_0 \subseteq \dom{\G}$ and $\sub{\G}{\cv{v}}{C_0}$,
  % and therefore $\sub{\G}{\set{y}}{C_0}$.
  Now we invoke the proposition for reification
  to show that $\typ{\G_r}{\evctx{y}}{T}$,
  and conclude by Lemma \ref{lemma:typ-refined-to-general}.
  % This case is therefore concluded.

  \emph{Case \textsc{lift-set} and \textsc{read}}.
  As above.

  \emph{Case \textsc{let-value}}.
  Then $t = \evctx{\tLetMode{m}{x}{v}{s}}$,
  $\dom{e} \cap \fv{v} = \varemptyset$,
  $t^\prime = \evctx{s}$,
  and $\sta^\prime = \sta, \tVal{x} \mapsto v$.
  Now we invoke Lemma \ref{lemma:evctx-reification-1}
  to show that
  $\exists \G_r, \Delta, Q$ such that
  % $\match{\G}{e}{\Delta}$,
  $\G_r, \Delta$ is inert and $\G_r \refined \G$,
  $\typ{\G_r, \Delta}{\tLetMode{m}{x}{v}{u}}{Q}$,
  and $\forall s^\prime $, and an inert $\G^\prime$ such that
  (i) $\typ{\G_r, \G^\prime, \Delta}{s^\prime}{Q}$;
  (ii) $\sub{\G_r, \G^\prime}{\cv{s^\prime}}{\cv{\tLetMode{m}{x}{v}{s}}}$;
  we have $\typ{\G_r, \G^\prime}{\evctx{s}}{T}$.
  By induction on the derivation of
  $\typ{\G_r, \Delta}{\tLetMode{m}{x}{v}{s}}{Q}$,
  we can show that $\typ{\G_r^\prime}{v}{T_0}$ for some $T_0$ and $\cv{T_0} = \cv{v}$
  and $\typ{\G_r^\prime, x :_m T_0}{s}{Q}$,
  where $\G_r^\prime$ is inert and $\G_r^\prime \refined \G_r, \Delta$.
  By Lemma \ref{lemma:typ-refined-to-general},
  we show that $\typ{\G_r, \Delta, x :_m T_0}{s}{Q}$.
  Since $\cv{v} \cap \dom{e} = \varemptyset$,
  ${\G_r, x :_m T_0}$ is well-formed.
  If $x^* \notin \cv{u}$,
  we have $\cv{s} = \cv{\tLetMode{m}{x}{v}{s}}$,
  and invoke reification to show that
  $\typ{\G_r, x :_m T_0}{s}{Q}$.
  Otherwise, we first assume that $x \in \cv{s}$ but not $x^? \in \cv{s}$.
  We have $\cv{\tLetMode{m}{x}{v}{s}} = \cv{s}/x \cup \cv{v}$.
  And $\cv{s} = \cv{s}/x \cup \set{x}$.
  Note that we have $\sub{\G, x :_m T_0}{x}{\cv{v}}$,
  and therefore we can show that
  $\typ{\G_r, x :_m T_0}{\evctx{s}}{T}$ via reification.
  By Lemma \ref{lemma:typ-refined-to-general},
  we show that
  $\typ{\G, x :_m T_0}{\evctx{s}}{T}$ in both cases.
  We conclude by the fact that $\match{}{\sta^\prime}{\G, x :_m T_0}$.
  The case when $x^? \in \cv{s}$ can be proven similarly.

  \emph{Case \textsc{var-value} and \textsc{lookup}}.
  As above.

  \emph{Case \textsc{rename-$\epsilon$}}.
  Then $t = \evctx{\tLetMode{\epsilon}{x}{y}{s}}$,
  $t^\prime = \evctx{[y/x]s}$,
  $\sta^\prime = \sta$.
  We first invoke Lemma \ref{lemma:evctx-reification-1}
  to show that there exists $\G_r, \Delta, Q$ such that
  $\G_r, \Delta$ is inert,
  $G_r \refined \G$,
  $\typ{\G_r, \Delta}{\tLetMode{\epsilon}{x}{y}{s}}{Q}$,
  and $\forall s^\prime$ such that
  $\typ{\G_r, \Delta}{s^\prime}{Q}$,
  and $\sub{\G_r, \Delta}{\cv{s^\prime}}{\cv{s}}$,
  we have $\typ{\G_r}{\evctx{s^\prime}}{T}$.
  Now we inspect the typing derivation $\typ{\G_r, \Delta}{\tLetMode{\epsilon}{x}{y}{s}}{Q}$,
  from which we can show that
  $\typ{\G_r, \Delta}{y}{P}$ for some $P$,
  and $\typ{\G_r, \Delta, x :_\epsilon P}{s}{Q}$.
  If $y :_\epsilon P^\prime \in \G_r, \Delta$,
  we show that
  $\typ{\G_r, \Delta}{[y/x]s}{Q}$
  (note that $x \notin \fv{Q}$).
  Otherwise, if $y :_{!D} P^\prime \in \G_r, \Delta$
  we invoke Lemma \TODO{jal}
\end{proof}


==> sections/metatheory/soundness-v2.tex <==
\subsection{Soundness}

\subsubsection{Store Typing}

\begin{lemma}[Value typing inversion: capture set]  \label{lemma:value-typing-inv-cs}
	If $\typDft{v}{\tCap{C}{S}}$,
  $\subDft{\cv{v}}{C}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the typing judgment.
\end{proof}

\begin{lemma}[Typing weakening]  \label{lemma:typing-weakening}
  All of the followings hold:
  (1) $\subDft{C_1}{C_2}$ implies $\sub{\G, \Delta}{C_1}{C_2}$;
  (2) $\subDft{T}{U}$ implies $\sub{\G, \Delta}{T}{U}$;
  and (3) $\typDft{t}{T}$ implies $\typ{\G, \Delta}{t}{T}$.
\end{lemma}

\begin{proof}
	For each case it follows from induction on the derivation.
\end{proof}

\begin{lemma}[Value lookup inversion: capture set]  \label{lemma:value-lookup-inv-cs}
	If (1) $\match{}{\sta; e}{\G; \Delta}$,
  (2) $\sta(\tVal{x}) = v$
  and (3) $\G(x) = \tCap{C}{S}$,
  then $\sub{\Delta}{\cv{v}}{C}$.
\end{lemma}

\begin{proof}
	By induction on the derivation of the matching environment.

  \emph{Case \textsc{empty}}. Conclude immediately.

  \emph{Case \textsc{grow-val}}.
  In this case, $\sta = \sta^\prime, \tVal{y} \mapsto v$,
  $e = []$,
  $\Delta = \Delta^\prime, y :_\epsilon T$,
  $\match{}{\sta^\prime, e}{\Delta^\prime}$,
  and $\typ{\Delta^\prime}{v}{T}$.
  If $x \ne y$, we conclude by IH and Lemma \ref{lemma:typing-weakening}.
  Otherwise if $x = y$,
  we conclude by Lemma \ref{lemma:value-typing-inv-cs} and Lemma \ref{lemma:typing-weakening}.

  \emph{Case \textsc{grow-var}}.
  In this case, $\sta = \sta_0, \tVal{y} \mapsto v$,
  $e = []$,
  $\Delta = \Delta_0, y :_{!} \tCap{\set{*}}{\tRef{S}}$.
  Since $x \in \bval{\sta}$, $x \ne y$.
  We therefore conclude by IH and Lemma \ref{lemma:typing-weakening}.

  \emph{Case \textsc{grow-set}}. As above.

  \emph{Case \textsc{grow-ctx-let} and \textsc{grow-ctx-var}}. By IH.

  \emph{Case \textsc{grow-ctx-par}}.
  We conclude by IH and Lemma \ref{lemma:typing-weakening}.

\end{proof}

\begin{lemma}[Variable lookup inversion]  \label{lemma:val-lookup-inv}
	If
  (i) $\match{}{\sta; e}{\G; \Delta}$,
  (ii) $\typ{\G, \Delta}{x}{T}$,
  (iii) $\sta(\tVal{x}) = v$,
  then $\typ{\G, \Delta}{v}{T}$.
\end{lemma}
\TODO{assumed}

\begin{lemma}  \label{lemma:value-typing-star-notin-cv}
  If $\typDft{v}{T}$,
  then $* \notin \cv{v}$.
\end{lemma}

\begin{proof}
	By straightforward induction on the typing judgement.
\end{proof}

\begin{lemma}  \label{lemma:star-notin-eps-binding}
	If $\match{}{\sta}{\G}$ and $x :_\epsilon \tCap{C}{S} \in \G$
  then $* \notin C$.
\end{lemma}

\begin{proof}
  By induction on the derivation of $\match{}{\sta}{\G}$.

  \emph{Case \textsc{empty}}.
  We conclude immediately.

  \emph{Case \textsc{grow-val}}.
  In this case, $\G = \G_0, y :_\epsilon \cv{v}\ S$.
  If $x \ne y$, we conclude by IH.
  Otherwise we conclude by Lemma \ref{lemma:value-typing-star-notin-cv}.

  \emph{Case \textsc{grow-var} and \textsc{grow-set}}.
  By IH.
\end{proof}

\subsubsection{Non-Interference}

\begin{lemma}  \label{lemma:footprint-decrease-depth}
	If $F = \fFootprint{\G}{C}$,
  then $\max_{\tau \in C} \fDepth{\G}{\tau} \le \max_{\tau \in F} \fDepth{\G}{\tau}$.
\end{lemma}

\begin{proof}
	By induction on $\fFootprint{\G}{C}$.

  \begin{enumerate}[(i)]
  \item \emph{When $C = \set{x}$, $x = *$ or $x :_! T \in \G$}.
    In this case, $F = \set{x} = C$
    and we conclude this case.

  \item \emph{When $C = \set{x}$, and $x :_\epsilon \tCap{C_x}{S} \in \G$}.
    In this case, $F = \fFootprint{\G}{C_x}$.
    We conclude by IH and we have $\max_{\tau \in C_x} \fDepth{\G}{\tau} < \fDepth{\G}{x}$.

  \item \emph{When $C = \set{x^?}$}.
    Conclude by IH.

  \item \emph{When $C = \set{\tau_1, \cdots, \tau_n}$}.
    By repeated IH.
  \end{enumerate}
\end{proof}

\begin{lemma}[Strengthening of $\mathcal{F}$]  \label{lemma:footprint-strengthening}
  Given $C$
  and $\G = \G_1, \G_2$,
	if $d = \max_{\tau \in C} \fDepth{\G}{\tau}$,
  and $d < | \G_1 |$,
  then $\fFootprint{\G}{C} = \fFootprint{\G_1}{C}$.
\end{lemma}

\begin{proof}
	By induction on $\fFootprint{\G}{C}$.

  \begin{enumerate}[(i)]
  \item \emph{When $C = \set{x}$, $x :_! T \in \G$ or $x = *$}.
    If $x = *$ we conclude immediately.
    Otherwise, since $\fDepth{\G}{x} < | \G_1 |$
    we can show that $x :_! T \in \G_1$
    and conclude this case.

  \item \emph{When $C = \set{x}$ and $x :_\epsilon \tCap{C_x}{S} \in \G$}.
    In this case, we have $x :_\epsilon \tCap{C_x}{S} \in \G_1$ as well,
    and also $\max_{\tau \in C_x} \fDepth{\G}{\tau} < \fDepth{\G}{x}$.
    Now we invoke IH and conclude.

  \item \emph{When $C = \set{x^?}$}. By IH.

  \item \emph{When $C = \set{\tau_1, \cdots, \tau_n}$}. By repeated IH.
  \end{enumerate}
\end{proof}

\begin{lemma}[Strengthening of $\mathcal{Q}$]  \label{lemma:q-strengthening}
	Given $F$
  and $\G = \G_1, \G_2$,
  if $d = \max_{\tau \in C} \fDepth{\G}{\tau}$,
  and $d < | \G_1 |$,
  then $\fQ{\G}{F} = \fQ{\G_1}{F}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $\fQ{\G}{F}$.
\end{proof}

\begin{corollary}[Strengthening of non-interference]  \label{coro:ninter-strengthening}
	Given $\G = \G_1, \G_2$,
  and $\max_{\tau \in C_1 \cup C_2} \fDepth{\G}{\tau} < | \G_1 |$,
  then
  $\ninterfp{\G}{C_1}{C_2}$ implies $\ninterfp{\G_1}{C_1}{C_2}$.
\end{corollary}

\begin{lemma}  \label{lemma:x-in-fq-implies-cx-sub-fq}
	Given a context $\G$, a footprint $F$ in it and a variable $x :_{!} \tCap{C_x}{S} \in \G$,
  $x \in \fQ{\G}{F}$ implies $\fQ{\G}{C_x} \subseteq \fQ{\G}{F}$.
\end{lemma}

\begin{proof}
	By straightforward induction on $\fQ{\G}{F}$.
\end{proof}

\begin{lemma}  \label{lemma:intf-implies-f-intersect-q}
  $\intfDft{C}$ implies exists $x$, s.t. $x \in \fFootprint{\G}{C}$ and $x \in \fQ{\G}{C}$.
\end{lemma}

\begin{proof}
	By induction on $\intfDft{C}$.

  \emph{Case \textsc{intf-set}}.
  In this case $x \in C$ and $\intfDft{x}$.
  By IH we have $\exists y$ s.t. $y \in \fFootprint{\G}{x}$ and $y \in \fQ{\G}{x}$.
  We conclude by the facts that $\fFootprint{\G}{x} \subseteq \fFootprint{\G}{C}$
  and $\fQ{\G}{x} \subseteq \fQ{\G}{C}$.

  \emph{Case \textsc{intf-var}}.
  In this case, $C = \set{x}$, $x :_m \tCap{C_x}{S} \in \G$ and $\intfDft{C_x}$.
  We split cases on the mode of the binding for $x$.
  If $m = {!}$, we conclude immediately since $x \in \fFootprint{\G}{x}$ and $x \in \fQ{\G}{x}$.
  Otherwise if $m = {\epsilon}$, we invoke IH
  and show that exists $y$
  such that $y \in \fFootprint{\G}{C_x}$
  and $y \in \fQ{\G}{C_x}$.
  We conclude by the facts that $\fFootprint{\G}{C_x} \subseteq \fFootprint{\G}{x}$
  and $\fQ{\G}{C_x} \subseteq \fQ{\G}{x}$.

  \emph{Case \textsc{intf-star}}. We conclude immediately.
\end{proof}

\begin{lemma}  \label{lemma:intf-implies-non-ninter}
	If $x :_! \tCap{C_x}{S} \in \G$ and $\intfDft{C_x}$,
  then $\ninterfp{\G}{x}{x^*}$ does not hold.
\end{lemma}

\begin{proof}
	By the definition of $\ninter{\G}{F_1}{F_2}$.
\end{proof}

\begin{lemma}  \label{lemma:non-intf-implies-ninter}
  If $\intfDft{C}$ does not hold,
  then $\ninterfp{\G}{C}{C}$.
\end{lemma}
\TODO{assumed. tricky.}

\begin{lemma}  \label{lemma:q-sub-fq}
	$\fQ{\G}{C} \subseteq \fQ{\G}{(\fFootprint{\G}{C})}$.
\end{lemma}

\begin{proof}
	By induction on $\fQ{\G}{C}$.

  \begin{enumerate}
  \item In this case $C = \set{x}$ and $x :_! T \in \tCap{C_x}{S}$.
    We have $\fFootprint{\G}{x} = \set{x}$ and therefore conclude immediately.

  \item In this case $C = \set{x}$ and $x :_\epsilon T \in \tCap{C_x}{S}$.
    We have $\fFootprint{\G}{x} = \fFootprint{\G}{C_x}$ and conclude by IH.

  \item In this case we have $C = \set{*}$.
    We conculde immediately.

  \item In this case $C = \set{x^{?}}$.
    We have $\fQ{\G}{x^{?}} = \fQ{\G}{x}$.
    Now we split case on the kind of the binding for $x$.
    If $x :_! T \in \G$, we have $\fQ{\G}{(\fFootprint{\G}{x^{?}})} = \fQ{\G}{x^{?}} = \fQ{\G}{x}$
    and we conclude.
    Otherwise if $x :_\epsilon \tCap{C_x}{S} \in \G$ we have $\fQ{\G}{(\fFootprint{\Gamma}{x^{?}})} = \fQ{\G}{(\fFootprint{\G}{C_x})^{??}} = \fQ{\G}{(\fFootprint{\G}{C_x})}$.
    We conclude by IH.

  \item By repeated IH.
  \end{enumerate}
\end{proof}

\begin{lemma}  \label{lemma:ninter-implies-qq}
	$\ninter{\G}{F_1}{F_2}$ implies $\ninter{\G}{F_1^{??}}{F_2}$.
\end{lemma}

\begin{proof}
	Proof by contradiction.
  We assume that $\ninter{\G}{F_1^{??}}{F_2}$ does not hold,
  and split into two cases.

  \begin{enumerate}
  \item If $x^{?} \in F_1^{??}$, $y \in F_2$ and $x \in \fQ{\G}{y}$.
    Then we have $x \in F_1$ such that $x \in \fQ{\G}{y}$ and thus derive the contradiction.

  \item If $x^{?} \in F_1^{??}$, $y \in F_2$ and $y \in \fQ{\G}{x^?}$.
    In this case we have $\fQ{\G}{x}$ and $x \in F_1$.
    We therefore derive the contradiction too.
  \end{enumerate}
\end{proof}

\begin{lemma}[Subcapture preserves non-interference]  \label{lemma:subcapt-pres-ninter}
  If (i) $\ninterfp{\G}{C_1}{C_2}$,
  and (ii) $\subDft{C_1^\prime}{C_1}$,
  then $\ninterfp{\G}{C_1^\prime}{C_2}$.
\end{lemma}

\begin{proof}
	By induction on $\subDft{C_1^\prime}{C_1}$.

  \emph{Case \textsc{sc-elem}}.
  In this case, $C_1^\prime = \set{x}$ and $x \in C_1$.
  In this case, $\fFootprint{\G}{C_1^\prime} \subseteq \fFootprint{\G}{C_1}$
  and we conclude immediately.

  \emph{Case \textsc{sc-set}}.
  By repeated IH.

  \emph{Case \textsc{sc-var}}.
  In this case, $C_1^\prime = \set{x}$, $x : \tCap{C_x}{S} \in \G$ and $\subDft{C_x}{C_2}$.
  By IH we show that $\ninterfp{\G}{C_x}{C_2}$.
  We do a case analysis on the mode of the binding over $x$.

  \begin{itemize}
  \item \emph{$x :_! \tCap{C_x}{S} \in \G$}.
    Since $\fFootprint{\G}{x} = \set{x}$,
    the goal is to show that $\ninter{\G}{\set{x}}{\fFootprint{\G}{C_2}}$.
    We proceed by trying to derive a contradiction.
    We assume that $\ninter{\G}{\set{x}}{\fFootprint{\G}{C_2}}$ does not hold
    and split into two cases.
    In each case we show that under this assumption
    we derive a contradiction that $\ninterfp{\G}{C_x}{C_2}$ is false.
    \begin{itemize}
    \item If $\exists \tau \in \fFootprint{\G}{C_2}$ such that $x \in \fQ{\G}{\tau}$.
      We invoke Lemma \ref{lemma:x-in-fq-implies-cx-sub-fq} and show that $\fQ{\G}{C_x} \subseteq \fQ{\G}{(\fFootprint{\G}{C_2})}$.
      Then we invoke Lemma \ref{lemma:intf-implies-f-intersect-q} and show that
      exists $z$ such that $z \in \fFootprint{\G}{C_x}$ and $y \in \fQ{\G}{C_x}$.
      And we have $z \in \fQ{\G}{(\fFootprint{\G}{C_2})}$.
      Therefore $z \in \fFootprint{\G}{C_x} \cap \fQ{\G}{(\fFootprint{\G}{C_2})}$
      and the contradiction is derived.

    \item If $\exists \tau \in \fFootprint{\G}{C_2}$ such that $|\tau| \in \fQ{\G}{x}$.
      % Now we do a case analysis on the type of the binding for $x$.
      Since $x :_! \tCap{C_x}{S} \in \G$, then $\fQ{\G}{x} = \set{x} \cup \fQ{\G}{C_x}$.
      Let $y = |\tau|$.
      Then either $y = x$ or $y \in \fQ{\G}{C_x}$.
      If $y = x$, we have $x \in \fFootprint{\G}{C_2}$.
      Therefore, $\ninterfp{\G}{C_x}{x}$.
      Note that $\fQ{\G}{\fFootprint{\G}{x}} = \fQ{\G}{x} = \set{x} \cup \fQ{\G}{C_x}$.
      By Lemma \ref{lemma:intf-implies-f-intersect-q}
      we have $exists z$ such that $z \in \fFootprint{\G}{C_x}$ and $z \in \fQ{\G}{C_x}$.
      Therefore we derive a contradiction.
      Otherwise, if $y \in \fQ{\G}{C_x}$,
      we invoke Lemma \ref{lemma:q-sub-fq} and show that $\fQ{\G}{C_x} \subseteq \fQ{\G}{(\fFootprint{\G}{C_x})}$.
      Therefore we have $y \in \fQ{\G}{(\fFootprint{\G}{C_x})}$ and derive the contradiction.
      % Otherwise, if $x :_\epsilon \tCap{C_x}{S} \in \G$, we have $\fQ{\G}{x} = \fQ{\G}{C_x}$.
      % The contradiction is derived as in the other case but we does not have to consider the sub-case when $y = x$.
      % We invoke Lemma \ref{lemma:q-sub-fq} and show that $\fQ{\G}{x} \subseteq \fQ{\G}{(\fFootprint{\G}{x})}$.
    \end{itemize}

  \item \emph{$x :_\epsilon \tCap{C_x}{S} \in \G$}.
    In this case we have $\fFootprint{\G}{\set{x}} = \fFootprint{\G}{C_x}$
    and therefore conclude immediately by IH.
  \end{itemize}

  \emph{Case \textsc{sc-$<:$-$?$}}.
  In this case, $C_1^\prime = C_0^{??}$ and $\subDft{C_0}{C_1}$.
  By IH we have $\ninterfp{\G}{C_0}{C_2}$.
  We now conclude by Lemma \ref{lemma:ninter-implies-qq} and the fact that $\fFootprint{\G}{C_0^{??}} = (\fFootprint{\G}{C_0})^{??}$.

  \emph{Case \textsc{sc-var-$?$}}.
  In this case we have $C_1^\prime = \set{x}$,
  $x :_m \tCap{C_x}{S} \in \G$,
  and $\subDft{C_x^{??}}{C_1}$.
  By IH we have $\ninterfp{\G}{C_x^{??}}{C_2}$.
  Now we split the cases for $m$.
  % If $m = {!}$, we have $\fQ{\G}{(\fFootprint{\G}{x^{?}})} = \fQ{\G}{\set{x}} = \fQ{\G}{x}$.
  If $m = \epsilon$, we have $\fFootprint{\G}{x^{?}} = (\fFootprint{\G}{C_x})^{??} = \fFootprint{\G}{C_x^{??}}$
  and we conclude immediately.
  If $x :_! \tCap{C_x}{S} \in \G$,
  we have $\fFootprint{\G}{x^{?}} = \set{x^{?}}$.
  The goal to be proven is therefore $\ninter{\G}{x^{?}}{\fFootprint{\G}{C_2}}$.
  To proceed we assume the goal to be false, split into two cases and derive contradiction in both cases.
  \begin{enumerate}
  \item If $\exists y \in \fFootprint{\G}{C_2}$ such that
    $x \in \fQ{\G}{y}$.
    By Lemma \ref{lemma:x-in-fq-implies-cx-sub-fq} we have $\fQ{\G}{C_x} \subseteq \fQ{\G}{(\fFootprint{\G}{C_2})}$.
    Now we invoke Lemma \ref{lemma:intf-implies-f-intersect-q}
    and show that $\exists z$ such that $z \in \fFootprint{\G}{C_x}$ and $z \in \fQ{\G}{C_x} \subseteq \fQ{\G}{\fFootprint{\G}{C_2}}$.
    From this, we show that $z^{?} \in (\fFootprint{\G}{C_x})^{??}$
    and derive the contradiction.

  \item If $\exists y \in \fFootprint{\G}{C_2}$ such that $y \in \fQ{\G}{x^{?}}$.
    Notice that we have $\fQ{\G}{x^{?}} = \fQ{\G}{x} = \set{x} \cup \fQ{\G}{C_x}$.
    Again, we have either $y = x$ or $y \in \fQ{\G}{C_x}$ and split this two cases.
    If $y = x$, we can derive that $\ninterfp{\G}{C_x^{??}}{x}$.
    We invoke Lemma \ref{lemma:intf-implies-f-intersect-q},
    and show that there exists $z$ such that
    $z \in \fFootprint{\G}{C_x}$ and $z \in \fQ{\G}{C_x}$.
    Therefore we have $z^{?} \in \fFootprint{\G}{C_x^{??}}$
    and we derive the contradiction.
    Otherwise, if $y \in \fQ{\G}{C_x} = \fQ{\G}{C_x^{??}}$.
    By Lemma \ref{lemma:q-sub-fq} we have $\fQ{\G}{C_x^{??}} \subseteq \fFootprint{\G}{(\fQ{\G}{C_x^{??}})}$ and therefore $y \in \fFootprint{\G}{(\fQ{\G}{C_x^{??}})}$.
    % By Lemma \ref{lemma:q-sub-fq} we have $\fQ{\G}{x^{?}} \subseteq {\fQ{\G}}$
  \end{enumerate}
\end{proof}

\begin{lemma}  \label{lemma:star-notin-good-env}
	If $\forall x :_\epsilon \tCap{C_x}{S} \in \G. * \notin C_x$ and $* \notin C$,
  then $* \notin \fFootprint{\G}{C}$.
\end{lemma}

\begin{proof}
  By induction on $\fFootprint{\G}{C}$.

  \begin{enumerate}[(i)]
  \item \emph{When $C = \set{x}$, $x :_! T \in \G$ or $x = *$}.
    We conclude immediately since $* \notin \set{x}$.

  \item \emph{When $C = \set{x}$, $x :_\epsilon T \in \G$}.
    % Conclude by Lemma \ref{lemma:star-notin-eps-binding} and IH.
    Conclude by IH and the precondition that $* \notin \cv{T}$.

  \item \emph{When $C = \set{x^?}$}.
    By IH.

  \item \emph{When $C = \set{\tau_1, \cdots, \tau_n}$}.
    By repeated IH.
  \end{enumerate}
\end{proof}

\subsubsection{Evaluation Context Typing}

% \begin{definition}[Evaluation context typing]
%   The typing of an evaluation context, written $\typec{\G; \Delta}{e}{U}{C}{T}$,
%   is defined as
%   $\match{\G}{e}{\Delta}$ and
%   $\forall s$ s.t. $\typ{\G, \Delta}{s}{U}$ and $\ninterfp{\G, \Delta}{\cv{s}}{C}$,
%   we will have $\typDft{\evctx{s}}{T}$.
% \end{definition}

% \begin{lemma}[Evaluation context typing inversion]
%   If $\typDft{\evctx{s}}{T}$,
%   then exists $\Delta, U$ and $C$ such that
%   $\match{\G}{e}{\Delta}$,
%   $\typec{\G; \Delta}{e}{U}{C}{T}$,
%   and $\typ{\G, \Delta}{s}{U}$.
% \end{lemma}

% \begin{proof}
% 	By induction on the structure of $e$.

%   \emph{When $e = []$}.
%   Let $\Delta = \varemptyset, U = T$ and $C = \varemptyset$,
%   and we conclude immediately.

%   \emph{When $e = \tLetMode{\epsilon}{x}{e^\prime}{u}$}.
%   We first inspect the typing judgment $\typDft{\tLetMode{\epsilon}{x}{e^\prime[s]}{u}}{T}$,
%   which shows that $\typDft{e^\prime[s]}{T_0}$ for some $T_0$,
%   and also $\typ{\G, x : T_0}{u}{T}$.
%   Now we invoke IH which shows that there exists
%   $\Delta$, $U_0$ and $C_0$ such that
%   $\typec{\G}{e^\prime}{U_0}{C_0}{T_0}$
%   and $\typ{\G, \Delta}{s}{U_0}$.
%   We can show that $\forall s^\prime$,
%   as long as $\typ{\G, \Delta}{s^\prime}{U_0}$
%   and $\ninterfp{\G, \Delta}{\cv{s^\prime}}{C_0}$,
%   we have $\typ{\G}{e^\prime[s^\prime]}{T_0}$
%   and therefore $\typ{\G}{\evctx{s^\prime}}{T}$.
%   We therefore conclude.

%   \emph{When $e = \tLetVar{x}{e^\prime}{u}$}.
%   As above.

%   \emph{When $e = \tLetMode{!}{x}{e^\prime}{u}$}.

% \end{proof}

\begin{lemma}  \label{lemma:union-subcapt}
	If $\subDft{C_1}{C_2}$ and $\subDft{C_1^\prime}{C_2}$,
  then $\subDft{C_1 \cup C_1^\prime}{C_2}$.
\end{lemma}

\begin{proof}
  By the (\textsc{sc-set}) rule.
\end{proof}

\begin{lemma}  \label{lemma:subcapt-union}
	If $\subDft{C_1}{C_2}$ then $\subDft{C_1}{C_2 \cup C_2^\prime}$.
\end{lemma}

\begin{proof}
	By straightforward induction on the subcapture derivation.
\end{proof}

\begin{corollary}  \label{lemma:subcapt-join}
	If $\subDft{C_1}{C_2}$ and $\subDft{C_1^\prime}{C_2^\prime}$
  then $\subDft{C_1 \cup C_1^\prime}{C_2 \cup C_2^\prime}$.
\end{corollary}

\begin{lemma}[Evaluation context typing inversion]  \label{lemma:evctx-typing-inv}
  If $\typDft{\evctx{s}}{T}$,
  then there exists $\Delta$ and $U$ such that $\match{\G}{e}{\Delta}$,
  and $\typ{\G, \Delta}{s}{U}$.
\end{lemma}

\begin{proof}
	By induction on $e$.

  \emph{When $e = []$}.
  We set $\Delta = \varemptyset$, $U = T$ and conclude immediately.

  \emph{When $e = \tLetMode{m}{x}{e^\prime}{u}$}.
  By inverting the typing judgment $\typDft{\tLetMode{m}{x}{\ctx{e^\prime}{s}}{u}}$,
  we have that
  $\typDft{\ctx{e^\prime}{s}}{T_0}$ for some $T_0$,
  and $\typ{\G, x :_m T_0}{u}{T}$.
  We invoke IH and show that there exists $\Delta_0$ and $U_0$
  such that $\match{\G}{e^\prime}{\Delta_0}$
  and $\typ{\G, \Delta_0}{\ctx{e^\prime}{s}}{U_0}$.
  Now we set $\Delta = \Delta_0$, $U = U_0$ and conclude.

  \emph{When $e = \tLetVar{x}{e^\prime}{u}$}. As above.

  \emph{When $e = \tLetMode{!}{x}{t}{e^\prime}$}.
  We first invert the judgment $\typDft{\tLetMode{!}{x}{t}{\ctx{e^\prime}{s}}}{T}$
  and show that
  $\typDft{t}{T_0}$ for some $T_0$
  and also $\typ{\G, x : T_0}{\ctx{e^\prime}{s}}{T}$.
  We now invoke IH and show that there exists $\Delta_0$ and $U_0$ such that
  $\match{\G, x : T_0}{e^\prime}{\Delta_0}$,
  and $\typDft{\G, x : T_0, \Delta_0}{s}{U_0}$.
  Now we set $\Delta = x : T_0, \Delta_0$, $U = U_0$ and conclude.
\end{proof}

\begin{lemma}  \label{lemma:subcapt-drop-x}
  Given context $\G$,
  if $x \in \dom{\G}$, and for any $y :_m \tCap{C}{S} \in \G$ we have $x^* \notin C$,
  and $\sub{\G}{C_1}{C_2}$,
  then $\sub{\G/x}{C_1/x^*}{C_2/x^*}$.
\end{lemma}

\begin{proof}
	By induction on the subcapture derivation $\sub{\G}{C_1}{C_2}$.

  \emph{Case \textsc{sc-var}}.
  In this case, $C_1 = \set{y}$, $y :_m \tCap{C_y}{S_y} \in \G$,
  and $\subDft{C_y}{C_2}$.
  If $x = y$, then we have $C_1/x = \varemptyset$ and we conclude immediately.
  Otherwise, by IH we show that $\sub{\G/x}{C_y/x}{C_2/x}$.
  Note that since $x \ne y$, $y :_m \tCap{C_y}{S_y} \in \G/x$.
  Also, $C_y/x = C_y$ since $x \notin C_y$ as required in the pre-condition.
  We conclude by (\textsc{sc-var}).

  \emph{Case \textsc{sc-elem}}.
  In this case, $C_1 = \set{\tau}$ and $\tau \in C_2$.
  We can show that $C_x/\tau \subseteq C_2/\tau$ and conclude by (\textsc{sc-elem}).

  \emph{Case \textsc{sc-set}}.
  In this case, $C_1 = \set{y_1, \cdots, y_n}$,
  and for each $i = 1, \cdots, n$ we have $\subDft{\set{y_i}}{C_2}$.
  We conclude by repeated IH and the (\textsc{sc-set}) rule.

  \emph{Case \textsc{sc-$<:$-$?$}}.
  In this case, $C_1 = \set{y^?}$ and $\subDft{\set{y}}{C_2}$.
  If $y = x$ we have $C_1 = \varemptyset$ and conclude.
  Otherwise if $y \ne x$, by IH we show that $\subDft{\set{y}}{C_2/x}$.
  We therefore conclude by (\textsc{sc-$<:$-$?$}).

  \emph{Case \textsc{sc-var-$?$}}.
  In this case, $C_1 = \set{y^?}$, $y :_m \tCap{C_y}{S_y} \in \G$ and $\subDft{C_y^{??}}{C_2}$.
  If $y = x$, we again have $C_1 = \varemptyset$ and conclude immediately.
  Otherwise, by IH we show tha t$\subDft{C_y^{??}/x^*}{C_2/x^*}$.
  Notice that $(C_y^{??}/x^*) = C_y^{??}/x^*$ and we conclude by (\textsc{sc-var-$?$}).
\end{proof}

\begin{lemma}[Evaluation context reification for subcapturing]  \label{lemma:evctx-reification-subcapt}
  If $\sub{\G, \Delta}{\cv{t}}{\cv{u}}$
  and $\match{\G}{e}{\Delta}$,
  then $\sub{\G}{\cv{\evctx{t}}}{\cv{\evctx{u}}}$.
\end{lemma}

\begin{proof}
  By induction on the structure of $e$.

  \emph{When $e = []$}. We conclude immediately.

  \emph{When $e = \tLetMode{m}{x}{e^\prime}{s}$}.
  We have $\match{\G}{e^\prime}{\Delta}$ and invoke IH to show that
  $\sub{\G}{\cv{\ctx{e^\prime}{t}}}{\cv{\ctx{e^\prime}{u}}}$.
  We have either $\cv{\evctx{t}} = \cv{\evctx{u}} = \cv{s}/x^*$,
  or $\cv{\evctx{t}} = \cv{\ctx{e^\prime}{t}} \cup \cv{s}/x^* \wedge \cv{\evctx{u}} = \cv{\ctx{e^\prime}{u}} \cup \cv{s}/x^*$.
  In the first case we conclude by the reflexivity of subcapturing,
  and in the second case we conclude by IH and Lemma \ref{lemma:subcapt-join}.

  \emph{When $e = \tLetVar{x}{e^\prime}{s}$}. As above.

  \emph{When $e = \tLetMode{!}{x}{s}{e^\prime}$}.
  In this case we have $\typDft{s}{T}$, $\Delta = x :_! T, \Delta_0$ and $\match{\G, x :_! T}{e^\prime}{\Delta_0}$.
  We invoke IH and show that $\sub{\G, x :_! T}{\cv{\ctx{e^\prime}{t}}}{\cv{\ctx{e^\prime}{u}}}$.
  Now we split the possible cases of $\cv{\evctx{t}}$ and $\cv{\evctx{u}}$.
  \begin{enumerate}[(i)]
  \item If $s$ is not a value.
    In this case we have $\cv{\evctx{t}} = \cv{s} \cup \cv{\ctx{e^\prime}{t}}/x^*$
    and $\cv{\evctx{u}} = \cv{s} \cup \cv{\ctx{e^\prime}{u}}/x^*$.
    We invoke Lemma \ref{lemma:subcapt-drop-x} to show that
    $\sub{\G}{\cv{\ctx{e^\prime}{t}}/x^*}{\cv{\ctx{e^\prime}{u}}/x^*}$ (note that $x$ is fresh).
    Now we conclude by Lemma \ref{lemma:subcapt-join}.
  \item If $s$ is a value. We further split to the following cases.
    \begin{itemize}
    \item When $x^* \notin \cv{\ctx{e^\prime}{t}}$ and $x^* \notin \cv{\ctx{e^\prime}{u}}$.
      In this case, $\cv{\evctx{t}} = \cv{\ctx{e^\prime}{t}}/x^*$
      and $\cv{\evctx{u}} = \cv{\ctx{e^\prime}{u}}/x^*$.
      We conclude by Lemma \ref{lemma:subcapt-drop-x}.

    \item When $x^* \notin \cv{\ctx{e^\prime}{t}}$ and $x^* \in \cv{\ctx{e^\prime}{u}}$.
      In this case, $\cv{\evctx{t}} = \cv{\ctx{e^\prime}{t}}/x^*$
      and $\cv{\evctx{u}} = \cv{s} \cup \cv{\ctx{e^\prime}{u}}/x^*$.
      We conclude by Lemma \ref{lemma:subcapt-drop-x} and Lemma \ref{lemma:subcapt-union}.

    \item When $x^* \in \cv{\ctx{e^\prime}{t}}$ and $x^* \notin \cv{\ctx{e^\prime}{u}}$.
      In this case, $\cv{\evctx{t}} = \cv{s} \cup \cv{\ctx{e^\prime}{t}}/x^*$
      and $\cv{\evctx{u}} = \cv{\ctx{e^\prime}{u}}/x^*$.
      Since $x \in \cv{\ctx{e^\prime}{t}}$, by inspecting the subcapture derivation
      $\sub{\G, x :_! T}{\cv{\ctx{e^\prime}{t}}}{\cv{\ctx{e^\prime}{u}}}$
      we can show that
      $\sub{\G, x :_! T}{\set{x^*}}{\cv{\ctx{e^\prime}{u}}}$.
      By inspecting this judgement, since $x^* \notin \cv{\ctx{e^\prime}{u}}$,
      if $x^* = x$ then
      $\sub{\G, x :_! \tCap{C_x}{S}}{C_x}{\cv{\ctx{e^\prime}{u}}}$ (note that here we assume that $T = \tCap{C_x}{S_x}$);
      and if $x^* = x^?$ then
      $\sub{\G, x :_! \tCap{C_x}{S}}{C_x^{??}}{\cv{\ctx{e^\prime}{u}}}$.
      By Lemma \ref{lemma:value-typing-inv-cs} we have $\sub{\G, x :_! \tCap{C_x}{S}}{\cv{s}}{C_x}$,
      from which follows that $\sub{\G, x :_! \tCap{C_x}{S}}{\cv{s}}{\cv{\ctx{e^\prime}{u}}}$ (and the same for the case when $x^* = x^?$).
      $\sub{\G, x :_! T}{\cv{s} \cup \cv{\ctx{e^\prime}{t}}}{\cv{\ctx{e^\prime}{u}}}$ by Lemma \ref{lemma:union-subcapt}.
      We proceed by invoking Lemma \ref{lemma:subcapt-drop-x} and show that
      $\subDft{\cv{s} \cup \cv{\ctx{e^\prime}{t}}/x}{\cv{\ctx{e^\prime}{u}}/x}$ (note that $x \notin \cv{s}$).

    \item When $x^* \in \cv{\ctx{e^\prime}{t}}$ and $x^* \in \cv{\ctx{e^\prime}{u}}$.
      In this case, $\cv{\evctx{t}} = \cv{s} \cup \cv{\ctx{e^\prime}{t}}/x^*$
      and $\cv{\evctx{u}} = \cv{s} \cup \cv{\ctx{e^\prime}{u}}/x^*$.
      We conclude by Lemma \ref{lemma:subcapt-drop-x} and Lemma \ref{lemma:subcapt-join}.
    \end{itemize}
  \end{enumerate}
\end{proof}

\begin{lemma}[Plug term back into evaluation context]  \label{lemma:plug-back-evctx}
	If
  (i) $\match{\G}{e}{\Delta}$,
  (ii) $\typDft{\evctx{s}}{T}$,
  (iii) $\typ{\G, \Delta}{s}{U}$,
  (iv) $\typ{\G, \Delta}{s^\prime}{U}$,
  and (v) $\sub{\G, \Delta}{\cv{s^\prime}}{\cv{s}}$,
  then $\typDft{\evctx{s^\prime}}{T}$.
\end{lemma}

\begin{proof}
	By induction on the structure of $e$.

  \emph{When $e = []$}.
  We conclude immediately.

  \emph{When $e = \tLetMode{\epsilon}{x}{e^\prime}{u}{T}$}.
  We invert the typing judgment $\typDft{\tLetMode{\epsilon}{x}{\ctx{e^\prime}{s}}{u}}{T}$
  and show that $\typDft{\ctx{e^\prime}{s}}{T_0}$ for some $T_0$,
  and $\typ{\G, x :_\epsilon T_0}{u}{T}$.
  We invoke IH and show that $\typDft{\ctx{e^\prime}{s^\prime}}{T_0}$
  and therefore conclude by (\textsc{let}).

  \emph{When $e = \tLetVar{x}{e^\prime}{u}$}. As above.

  \emph{When $e = \tLetMode{!}{x}{e^\prime}{u}$}.
  We invert $\typDft{\tLetMode{!}{x}{e^\prime[s]}{u}}$ and show that
  $\typDft{\ctx{e^\prime}{s}}{T_0}$ for some $T_0$,
  $\typ{\G, x :_{!} T_0}{u}{T}$,
  and $\ninterfp{\G}{\cv{\ctx{e^\prime}{s}}}{\cv{u}/x^*}{T}$.
  Now we invoke IH and show that $\typDft{\ctx{e^\prime}{s^\prime}}{T_0}$.
  To invoke (\textsc{let}) the left to be shown is $\ninterfp{\G}{\cv{\ctx{e^\prime}{s^\prime}}}{(\cv{u}/x^*)}$.
  Since we have $\match{\G}{e^\prime}{\Delta}$,
  and $\sub{\G, \Delta}{\cv{s^\prime}}{\cv{s}}$,
  we can invoke Lemma \ref{lemma:evctx-reification-subcapt} and show that
  $\sub{\G}{\cv{\ctx{e^\prime}{s^\prime}}}{\cv{\ctx{e^\prime}{s}}}$.
  Now we invoke Lemma \ref{lemma:subcapt-pres-ninter} and show that
  $\ninterfp{\G}{\cv{\ctx{e^\prime}{s^\prime}}}{\cv{u}/x^*}$ and we conclude.

  \emph{When $e = \tLetMode{!}{x}{u}{e^\prime}$}.
  We invert $\typDft{\tLetMode{!}{x}{e^\prime[s]}{u}}{T}$ and show that
  $\typDft{u}{T_0}$ for some $T_0$,
  $\typ{\G, x :_{!} T_0}{\ctx{e^\prime}{s}}{T}$,
  and $\ninterfp{\G}{\cv{u}}{\cv{\ctx{e^\prime}{s}}/x^*}$.
  We can show that $\Delta = x :_! T_0, \Delta_0$ for some $\Delta_0$
  and $\match{\G, x :_! T_0}{e^\prime}{\Delta_0}$.
  We therefore invoke IH and show that $\typ{\G, x :_{!} T_0}{\ctx{e^\prime}{s^\prime}}{T}$.
  Now to invoke the (\textsc{let}) rule the remaining to be shown is
  $\ninterfp{\G}{\cv{u}}{\cv{\ctx{e^\prime}{s^\prime}}/x^*}$.
  We first reify the evaluation context by invoking Lemma \ref{lemma:evctx-reification-subcapt}
  and show that $\sub{\G, x :_! T}{\cv{\ctx{e^\prime}{s^\prime}}}{\cv{\ctx{e^\prime}{s}}}$.
  Now invoke Lemma \ref{lemma:subcapt-drop-x} and show that
  $\sub{\G}{\cv{\ctx{e^\prime}{s^\prime}}/x^*}{\cv{\ctx{e^\prime}{s}}/x^*}$.
  Now we invoke Lemma \ref{lemma:subcapt-pres-ninter} and conclude.
\end{proof}

\begin{lemma}[Lifting a mutable variable to the store]  \label{lemma:lift-var-to-store}
	If (i) $\match{\G}{e}{\Delta}$ and $\forall x :_\epsilon \tCap{C}{S} \in \G, x \notin C$,
  (ii) $\typDft{\evsctx{\tLetVar{x}{v}{t}}}{T}$,
  and (iii) $\typ{\G, \Delta}{v}{S}$,
  % and (iv) $\typ{\G, \Delta, x :_! \tCap{\set{*}}{\tRef{S}}}{t}{U}$ ($x \notin U$),
  then $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\evsctx{t}}{T}$.
\end{lemma}

\begin{proof}
	By induction on $e$.

  \emph{When $e = []$}. We conclude immediately from the preconditions.

  \emph{When $e = \tLetMode{\epsilon}{y}{e^\prime}{u}$}.
  By inverting the typing judgment $\typDft{\tLetMode{\epsilon}{y}{\evpctx{\tLetVar{x}{v}{t}}}{u}}{T}$
  we show that $\typDft{\evpctx{\tLetVar{x}{v}{t}}}{T_0}$ for some $T_0$
  and $\typ{\G, y :_\epsilon T_0}{u}{T}$.
  Now we invoke IH and show that $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\evpctx{t}}{T_0}$.
  By weakening we have $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}, y :_\epsilon T_0}{u}{T}$
  and conclude by (\textsc{let}) rule.

  \emph{When $e = \tLetVar{y}{e^\prime}{u}$}. As above.

  \emph{When $e = \tLetMode{!}{y}{e^\prime}{u}$}.
  By inverting the typing judgment $\typDft{\tLetMode{!}{y}{\evpctx{\tLetVar{x}{v}{t}}}{u}}{T}$
  we show that $\typDft{\evpctx{\tLetVar{x}{v}{t}}}{T_0}$ for some $T_0$,
  $\typ{\G, y :_! T_0}{u}{T}$,
  and $\ninterfp{\G}{\cv{\evpctx{\tLetVar{x}{v}{t}}}}{(\cv{u}/y)}$.
  By IH we show that
  $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\evpctx{t}}{T_0}$.
  By weakening, $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}, y :_! T_0}{u}{T}$.
  To invoke (\textsc{let}) and conclude we have to show that
  $\ninterfp{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\cv{\evpctx{t}}}{(\cv{u}/y)}$.
  By weakening, we can show that
  $\ninterfp{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\cv{\evpctx{\tLetVar{x}{v}{t}}}}{(\cv{u}/y)}$.
  By induction on the structure of $e$,
  we can show that
  $\sub{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\cv{\evpctx{t}}}{\cv{\evpctx{\tLetVar{x}{v}{t}}} \cup \set{x, x^?}}$.
  To invoke Lemma \ref{lemma:subcapt-pres-ninter} and conclude,
  the remaining to be shown is
  $\ninterfp{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\set{x, x^?}}{(\cv{u}/y)}$.
  % We assume this does not hold and derive a contradiction.
  We have $\fFootprint{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\set{x, x^?}} = \set{x, x^?}$,
  and $\fQ{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\fFootprint{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\set{x, x^?}}} = \set{x, *}$.
  We conclude by the freshness of $x$, Lemma \ref{lemma:star-notin-good-env}
  and Lemma \ref{lemma:value-typing-star-notin-cv}.

  \emph{When $e = \tLetMode{!}{y}{u}{e^\prime}$}.
  In this case, we have $\typDft{\tLetMode{!}{y}{u}{\evpctx{\tLetVar{x}{v}{t}}}}{T}$.
  By inverting the typing derivation we can show that
  we show that
  $\typ{\G}{u}{T_0}$ for some $T_0$,
  $\typ{\G, x :_! T_0}{\evpctx{\tLetVar{x}{v}{t}}}{T}$,
  and $\ninterfp{\G}{\cv{u}}{(\cv{\evpctx{\tLetVar{x}{v}{t}}}/y)}$.
  Notice that the condition that $\forall y :_\epsilon \tCap{C_y}{S} \in \G, x :_! T_0. * \notin C_y$
  still holds and thus we can invoke IH.
  We prove this case as in the previous case.
\end{proof}

\subsubsection{Substitution}

\begin{lemma}[Term substitution preserves non-interference ($\epsilon$)]
	If (i) $\ninterfp{\G_1, x :_\epsilon P, \G_2}{C_1}{C_2}$,
  (ii) $\typ{\G_1}{y}{P}$,
  then $\ninterfp{\G_1, [y^*/x^*] \G_2}{([y^*/x^*]C_1)}{([y^*/x^*]C_2)}$.
\end{lemma}

\begin{proof}
  By induction by $| \G_2 |$.
  Let $\theta = [y^*/x^*]$,
  $\Xi = \G_1, x :_\epsilon P, \G_2$,
  and $\Xi^\prime = \G_1, \theta \G_2$.

  \emph{When $| \G_2 | = 0$}.
  Now we split the cases based on whether $x^*$ is a member of $C_1, C_2$.
  \begin{enumerate}[(i)]
  \item \emph{When $x^* \notin C_1$ and $x^* \notin C_2$}.
    In this case, $\theta C_1 = C_1/x^*$
    and $\theta C_2 = C_2/x^*$.
    Therefore, we have $\max_{\tau \in \theta C_1 \cup \theta C_2} \fDepth{\Xi}{\tau} < | \G |$.
    We conclude by Corollary \ref{coro:ninter-strengthening}.

  \item \emph{When $x^* \in C_i$ but $x^* \notin C_j$, here $i, j$ is $1$ or $2$}.
    WLOG, we assume that $x^* \in C_1$ but $x^* \notin C_2$.
    Similarly to the previous case, we can show that
    $\ninterfp{\G}{C_1/x^*}{C_2/x^*}$.
    The remaining to be shown is $\ninterfp{\G}{y}{C_2}$ if $x \in C_1$
    and $\ninterfp{\G}{y^?}{C_2}$ if $x^? \in C_1$.
    If $x \in C_1$,
    we have $\ninterfp{\Xi}{C_x}{C_2}$.
    Note that $\fFootprint{\Xi}{x} = \fFootprint{\Xi}{C_x}$
    where $C_x$ denotes $\cv{P}$.
    Assume that $y :_m \tCap{C_y}{S_y} \in \G_1$.
    By inverting the typing judgment $\typ{\G_1}{y}{P}$,
    we can show that $\sub{\G_1}{\set{y}}{C_x}$,
    and by weakening we show that $\sub{\Xi}{\set{y}}{C_x}$.
    Now we invoke Lemma \ref{lemma:subcapt-pres-ninter} and show that
    $\ninterfp{\Xi}{\set{y}}{C_2}$.
    Now we invoke Corollary \ref{coro:ninter-strengthening} and conclude.
    We similarly prove the case when $x^? \in C_1$.

  \item \emph{When $x^* \in C_1$ and $x^* \in C_2$}.
    We can similarly prove that $\ninterfp{\G}{C_1/x^*}{C_2/x^*}$ as in the previous case.
    Similarly to the previous case, we prove that
    $\ninterfp{\G}{y^*}{C_i/x^*}$ for $i = 1, 2$.
    Also, we can show that $\ninterfp{\G}{y^*}{y^*}$ and conclude this case.
  \end{enumerate}

  \emph{When $\G_2 = \G_2^\prime, z :_\epsilon \tCap{C_z}{S_z}$}.
  Define $\Xi_0 = \G_1, x :_\epsilon P, \G_2^\prime$
  and similarly for $\Xi_0^\prime$.
  Note that $\fFootprint{\Xi}{z} = \fFootprint{\Xi}{C_z}$.
  We could invoke Lemma \ref{lemma:footprint-strengthening} to show that
  $\fFootprint{\Xi_0}{C_z}$.
  Moreover, we have the similar fact for $z^?$.
  Now we do a case analysis on whether $z^*$ is a member of $C_1, C_2$
  and in each case we conclude by IH and the noted fact.

  \emph{When $\G_2 = \G_2^\prime, z :_! \tCap{C_z}{S_z}$}.
  If $z^* \notin C_1, C_2$, then we invoke IH and Corollary \ref{coro:ninter-strengthening} and conclude.
  Otherwise, we check if $\intf{\Xi}{z}$ holds.
  If so, then $z^*$ at most be a member of one of $C_1, C_2$.
\end{proof}

\begin{lemma}[Term substitution preserves typing ($\epsilon$)]  \label{lemma:term-subst-pres-typing-eps}
  If $\typ{\G_1, x :_\epsilon T, \G_2}{t}{U}$ and $\typ{\G_1}{y}{T}$,
  then $\typ{\G_1, [y^*/x^*] \G_2}{[y^*/x^*]t}{[y^*/x^*]U}$.
\end{lemma}
\TODO{assumed}

\begin{lemma}[Term substitution preserves typing ($!$)]  \label{lemma:term-subst-pres-typing-bang}
  If $\typ{\G_1, x :_! T, \G_2}{t}{U}$, $\typ{\G_1}{y}{T}$ and $\ninterfp{\G_1}{(\cv{t} \cap \dom{\G_1})}{y}$,
  then $\typ{\G_1, [y^*/x^*] \G_2}{[y^*/x^*]t}{[y^*/x^*]U}$.
\end{lemma}
\TODO{assumed}

\subsubsection{Main Theorems}

\begin{lemma}[Lookup inversion: lambda]  \label{lemma:lookup-inv-lambda}
	If (i) $\match{}{\sta; e}{\G; \Delta}$,
  (ii) $\typ{\G, \Delta}{x}{C\, \forall(z :_m U) T}$,
  and (iii) $\sta(\tVal{x}) = \lambda(z :_m U^\prime) t$,
  then (i) $\sub{\G, \Delta}{U}{U^\prime}$,
  (ii) $\typ{\G, \Delta, z :_m U^\prime}{t}{T}$,
  and (iii) $\sub{\G, \Delta}{\cv{t}/z}{C}$.
\end{lemma}
\TODO{assumed}

\begin{lemma}[Erasing $!$-notation preserves non-interference]  \label{lemma:erase-bang-ninter}
  If
  (i) $\ninterfp{\G, x :_! \tCap{C_v}{S_x}, \Delta}{C_1}{C_2}$,
  (ii) $\ninter{\G}{\fFootprint{\G}{C_v}}{(\fFootprint{\G}{C_2}) \cap \dom{\G}}$ for $i = 1, 2$,
  then $\ninterfp{\G, x :_{[!]} \tCap{C_v}{S_x}}{C_1}{C_2}$.
\end{lemma}

\begin{proof}
  First, let $\Xi = \G, x :_! \tCap{C_v}{S_x}, \Delta$,
  and $\Xi^\prime = \G, x :_{[!]} \tCap{C_v}{S_x}, \Delta$.
  Proceed by splitting into the following four cases.

  \begin{enumerate}
  \item \emph{When $x^* \notin \fFootprint{\Xi}{C_1}$ and $x^* \notin \fFootprint{\Xi}{C_2}$}.
    In this case, $\fFootprint{\Xi^\prime}{C_i} = \fFootprint{\Xi}{C_i}$ for $i = 1, 2$.
    We therefore conclude this case immediately.

  \item \emph{When $x^* \notin \fFootprint{\Xi}{C_1}$ and $x^* \in \fFootprint{\Xi}{C_2}$}.
    In this case, $\fFootprint{\Xi^\prime}{C_1} = \fFootprint{\Xi}{C_1}$ as in the previous case.
    We first assume that $x \in \fFootprint{\Xi}{C_2}$ but not $x^?$.
    We can show that $\fFootprint{\Xi^\prime}{C_2} = (\fFootprint{\Xi}{C_2})/{x} \cup \fFootprint{\G}{C_v}$.
    From the precondition it follows directly that $\ninter{\Xi^\prime}{\fFootprint{\Xi^\prime}{C_1}}{\left( \fFootprint{\Xi}{C_2} \right)/{x}}$.
    Therefore, the remaining to be shown is that
    $\ninter{\Xi^\prime}{\fFootprint{\Xi}{C_1}}{\fFootprint{\G}{C_v}}$.
    We proceed by induction on $\max_{\tau \in C_1} \fDepth{\Xi}{\tau}$.
    \begin{itemize}
    \item When $\max_{\tau \in C_1} \fDepth{\Xi}{\tau} < | \tau |$.
      Then $C_1 \cap \dom{\G} = C_1$ and we conclude by the premise.

    \item Given $y^* \in C_1$ such that $\fDepth{\Xi}{y^*}$ is the largest.
      First, we assume that $y \in C_1$ but not $y^?$.
      We have $\fFootprint{\Xi}{C_1} = \fFootprint{\Xi}{C_1/y} \cup \fFootprint{\Xi}{y}$.
      It follows from IH that $\ninter{\Xi^\prime}{\fFootprint{\Xi}{C_1/y}}{\fFootprint{\G}{C_v}}$.
      If $y :_! \tCap{C_y}{S_y} \in \Delta$,
      then $\fFootprint{\Xi}{C_1} = \fFootprint{\Xi}{C_1/y} \cup \set{y}$.
      By the well-formedness of $\G$, $y \notin \fFootprint{\G}{C_v}$.
      We therefore conclude.
      Otherwise, if $y :_\epsilon \tCap{C_y}{S_y} \in \Delta$,
      we have $\fFootprint{\Xi}{C_1} = \fFootprint{\Xi}{C_1/y} \cup \fFootprint{\Xi}{C_y}$.
      Again by the well-formedness of $\Xi$ we have $\max{\tau \in C_y} \fFootprint{\Xi}{\tau} < \fDepth{\Xi}{y}$.
      We can therefore invoke IH and conclude.
      We can prove the case when $y^? \in C_1$ similarly.
    \end{itemize}

  \item \emph{When $x^* \in \fFootprint{\Xi}{C_1}$ and $x^* \notin \fFootprint{\Xi}{C_2}$}.
    This case can be proven the same way as the previous one since these two are symmetric.

  \item \emph{When $x^* \in \fFootprint{\Xi}{C_1}$ and $x^* \in \fFootprint{\Xi}{C_2}$}.
    If $\intf{\Xi}{x}$,
    we can show that $x^? \in \fFootprint{\Xi}{C_1}$ and $x^? \in \fFootprint{\Xi}{C_2}$ but not $x$.
    % We conclude by the fact that $\ninterfp{\G}{C_v^{??}}{C_v^{??}}$.
    Similarly to the above case we do induction to show that
    $\ninter{\Xi^\prime}{\fFootprint{\G}{C_v^{??}}}{(\fFootprint{\Xi}{C_i})/x^*}$ for $i = 1, 2$
    and conclude.
    Otherwise, if $\intf{\Xi}{x}$ does not hold,
    we show that $\ninterfp{\Xi^\prime}{C_v^{??}}{C_v^{??}}$ by Lemma \ref{lemma:non-intf-implies-ninter}.
    We similarly do induction to show that
    $\ninter{\Xi^\prime}{\fFootprint{\G}{C_v}}{(\fFootprint{\Xi}{C_i})/x^*}$ for $i = 1, 2$
    and conclude this case.
  \end{enumerate}
\end{proof}

\begin{lemma}[Erasing $!$-notation preserves subtyping and subcapturing]
  The following propositions hold:

	(1) $\sub{\G, x :_! T, \Delta}{C_1}{C_2}$ implies $\sub{\G, x :_{[!]} T, \Delta}{C_1}{C_2}$;

	(2) $\sub{\G, x :_! T, \Delta}{T_1}{T_2}$ implies $\sub{\G, x :_{[!]} T, \Delta}{T_1}{T_2}$.
\end{lemma}

\begin{proof}
  By straightforward induction on the derivations.
  No rule in this two judgments makes use of the kind of the bindings.
\end{proof}

\begin{lemma}
  Given
  $\Xi = \G, x :_! \tCap{C_v}{S_v}, \Delta$
  and $\Xi^\prime = \G, x :_\epsilon \tCap{C_v}{S_v}, \Delta$,
	if
  (i) $\typ{\Xi}{t}{T}$,
  (ii) $\ninter{\G}{\fFootprint{\G}{C_v}}{\fFootprint{\Xi}{\fv{t}} \cap \dom{\G}}$,
  (iii) given $\Delta = \Delta_1, y :_\epsilon \tCap{C_y}{S_y}, \Delta_2$,
  we have $\ninter{\G}{\fFootprint{\G}{C_v}}{\fFootprint{\G, x :_! \tCap{C_v}{S_x}, \Delta_0}{C_y}}$,
  then
  $\typ{\Xi^\prime}{t^\prime}{T}$.
\end{lemma}

\begin{proof}
	By induction on the typing derivation.

  \emph{Case \textsc{let}}.
  In this case, $t = \tLetMode{m}{y}{s}{u}$,
  $\typ{\Xi}{s}{\tCap{C_y}{S_y}}$ for some $C_y, S_y$,
  $\typ{\Xi, y :_m \tCap{C_y}{S_y}}{u}{T}$,
  and $\ninter{\Xi}{C_y \cup \fv{s}}{\fv{u}/y}$ if $m =\ !$.
  Note that $\fv{t} = \fv{s} \cup \fv{u}/y$,
  therefore from premise (ii) we have
  $\ninter{\G}{\fFootprint{\G}{C_v}}{\fFootprint{\Xi}{\fv{s}} \cap \dom{\G}}$.
  We now invoke IH and show that $\typ{\Xi^\prime}{s}{\tCap{C_y}{S_y}}$.
\end{proof}

\begin{lemma}[Erasing non-interference annotation]  \label{lemma:erase-ninter}
  Given a value $v$ and a program $t$ such that $\ninter{\G}{\cv{v}}{\cv{t}/x}$,
  the following propositions hold:

  (i) $\typ{\G, x :_! \tCap{\cv{v}}{S}, \Delta}{u}{T}$ and $\cv{u} \subseteq \cv{t}$
  implies
  $\typ{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{u}{T}$;

  (ii) $\sub{\G, x :_! \tCap{\cv{v}}{S}, \Delta}{T}{U}$ and $\fv{T} \subseteq \cv{t}$
  implies
  $\sub{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{T}{U}$;

  (iii) $\sub{\G, x :_! \tCap{\cv{v}}{S}, \Delta}{C}{D}$ and $C \subseteq \cv{t}$
  implies
  $\sub{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{C}{D}$;

  (iv) $\ninterfp{\G, x :_! \tCap{\cv{v}}{S}, \Delta}{C_1}{C_2}$ and $C_1, C_2 \subseteq \cv{t}$
  implies
  $\ninterfp{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{C_1}{C_2}$.
\end{lemma}

\begin{proof}
  By straightforward induction on the derivations of (i), (ii), (iii).
  Most cases does not care about the kind of the bindings.
  The only interesting cases are the non-interference check in typing
  which relies on proposition (iv).
  Now we prove proposition (iv).

  Let $\Xi = \G, x :_! \tCap{\cv{v}}{S}, \Delta$ and $\Xi^\prime = \G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta$.
  By induction on $\fFootprint{\Xi^\prime}{C_1}$ and $\fFootprint{\Xi^\prime}{C_2}$,
  we could show that $\fFootprint{\Xi^\prime}{C_1} = [x^* \mapsto (\fFootprint{\Xi^\prime}{\cv{v}})^*] \fFootprint{\Xi}{C_2}$
  and $\fFootprint{\Xi^\prime}{C_2} = [x^* \mapsto (\fFootprint{\Xi^\prime}{\cv{v}})^*] \fFootprint{\Xi}{C_2}$.
  And since $\Xi$ and $\Xi^\prime$ are well-formed, we have $\fFootprint{\Xi^\prime}{\cv{v}^*} = \fFootprint{\Xi}{\cv{v}^*}$.
  Also, we prove that $\forall C. \fQ{\Xi^\prime}{C} = \fQ{\Xi}{C}/x$ by straightforward induction on $\fQ{\Xi}{C}$.
  Now we split into the following cases.
  \begin{itemize}
  \item \emph{When $x^* \notin \fFootprint{\Xi}{C_1}$ and $x^* \notin \fFootprint{\Xi}{C_2}$}.\\
    Then $\fFootprint{\Xi^\prime}{C_1} = \fFootprint{\Xi}{C_1}$ and $\fFootprint{\Xi^\prime}{C_2} = \fFootprint{\Xi}{C_2}$.
    Note that $\fQ{\Xi^\prime}{C_1} = \fQ{\Xi}{C_1}/x$ and similarly for $C_2$, we can conclude this case.

  \item \emph{When $x^* \notin \fFootprint{\Xi}{C_1}$ and $x^* \in \fFootprint{\Xi}{C_2}$}.\\
    We first assume that $x \in \fFootprint{\Xi}{C_2}$ but not $x^?$.
    Then $\fFootprint{\Xi^\prime}{C_1} = \fFootprint{\Xi}{C_1}$ and $\fFootprint{\Xi^\prime}{C_2} = \fFootprint{\Xi}{C_2}/x \cup \fFootprint{\Xi}{\cv{v}}$.
    We could show that $\ninterfp{\Xi^\prime}{C_1}{C_2/x}$ as in the previous case.
    So the remaining to be shown is $\ninterfp{\Xi^\prime}{C_1}{\cv{v}}$.
    By the preconditions we can show that $\ninterfp{\Xi}{C_1/x}{\cv{v}}$.
    Then since we have $C_1/x = C_1$ and $\forall C. \fQ{\Xi^\prime}{C} \subseteq \fQ{\Xi}{C}$,
    we could conclude this case.
    When $x^{?} \in \fFootprint{\Xi}{C_2}$ we conclude similarly.

  \item \emph{When $x^* \in \fFootprint{\Xi}{C_1}$ and $x^* \notin \fFootprint{\Xi}{C_2}$}.\\
    As in the previous case. The two cases are symmetric.

  \item \emph{When $x^* \in \fFootprint{\Xi}{C_1}$ and $x^* \in \fFootprint{\Xi}{C_2}$}.\\
    If $\intf{\Xi}{\cv{v}}$, then by Lemma \ref{lemma:intf-implies-non-ninter}
    we know that $x \notin \fFootprint{\Xi}{C_1}, \fFootprint{\Xi}{C_2}$.
    Therefore $x^? \in \fFootprint{\Xi}{C_1}, \fFootprint{\Xi}{C_2}$.
    Therefore, $\fFootprint{\Xi^\prime}{C_1} = \fFootprint{\Xi}{C_1}/x^? \cup \fFootprint{\Xi}{\cv{v}^{??}}$,
    and $\fFootprint{\Xi^\prime}{C_2} = \fFootprint{\Xi}{C_2}/x^? \cup \fFootprint{\Xi}{\cv{v}^{??}}$.
    We already have $\ninter{\Xi}{\fFootprint{\Xi}{C_1}/x^?}{\fFootprint{\Xi}{C_2}/x^?}$
    and from $\forall C. \fQ{\Xi^\prime}{C} \subseteq \fQ{\Xi}{C}$
    we show that $\ninter{\Xi^\prime}{\fFootprint{\Xi}{C_1}/x^?}{\fFootprint{\Xi}{C_2}/x^?}$.
    Also, by the definition of $\fFootprint{\Xi^\prime}{\cdot}$
    it holds trivially that $\ninterfp{\Xi^\prime}{\cv{v}^{??}}{\cv{v}^{??}}$.
    The remaining to be shown is that $\ninter{\Xi^\prime}{\fFootprint{\Xi}{C_1}/x^?}{\fFootprint{\Xi}{\cv{v}^{??}}}$,
    which follows straightforwardly from $\forall C. \fQ{\Xi^\prime}{C} \subseteq \fQ{\Xi^\prime}{C}$,
    Lemma \ref{lemma:ninter-implies-qq},
    and the preconditions.
    Otherwise, if $\intf{\Xi}{\cv{v}}$ does not hold.
    we apply the similar reasoning,
    and to conclude it suffices to show that $\ninterfp{\Xi^\prime}{\cv{v}}{\cv{v}}$.
    By Lemma \ref{lemma:non-intf-implies-ninter}
    we show that $\ninterfp{\Xi}{\cv{v}}{\cv{v}}$,
    and conclude by the fact that $\forall C. \fQ{\Xi^\prime}{C} \subseteq \fQ{\Xi}{C}$.
  \end{itemize}
\end{proof}

\begin{theorem}[Preservation]
  If (i) $\match{}{\sta}{\G}$,
  (ii) $\typDft{t}{T}$,
  and (iii) $\reduction{\stDft{t}}{\st{\sta^\prime}{t^\prime}}$,
  then there exists $\G^\prime$ such that $\match{}{\sta}{\G^\prime}$
  and $\typ{\G^\prime}{t^\prime}{T}$.
\end{theorem}

\begin{proof}
	By splitting the cases of the reduction derivation.

  \emph{Case \textsc{apply}}.
  In this case, $t = \evctx{x\,y}$, $\sta(\tVal{x}) = \lambda(z: U) s$ and $t^\prime = \evctx{[y/z] s}$.
  We invoke Lemma \ref{lemma:evctx-typing-inv} and show that there exists $\Delta, Q$ such that
  $\match{\G}{e}{\Delta}$ and $\typ{\G, \Delta}{x\,y}{Q}$.
  We inspect the derivation of $\typ{\G, \Delta}{x\,y}{Q}$, based on which we can show that
  $\typ{\G, \Delta}{x}{C\,\forall(z :_m U^\prime)\ Q^\prime}$,
  $\typ{\G, \Delta}{y}{U^\prime}$,
  and $Q = [y/z]Q^\prime$.
  We invoke Lemma \ref{lemma:lookup-inv-lambda} and use narrowing to show that
  $\typ{\G, \Delta, z :_m U^\prime}{s}{Q^\prime}$ and $\typ{\G, \Delta}{\cv{s}/z}{C}$.
  Now we invoke Lemma \ref{lemma:term-subst-pres-typing-eps} or Lemma \ref{lemma:term-subst-pres-typing-bang}
  based the value of $m$,
  and show that $\typ{\G, \Delta}{[y/z] s}{Q}$.
  Now, to invoke Lemma \ref{lemma:plug-back-evctx} and conclude the case,
  the remaining to be shown is that $\sub{\G, \Delta}{\cv{[y/z] s}}{\cv{x\, y}}$.
  If $z \notin \cv{s}$, we have $\cv{[y/z] s} = \cv{s}/z$, and we therefore conclude.
  Otherwise, we have $\cv{[y/z] s} = \cv{s}/z \cup \cv{y}$ and conclude by Lemma \ref{lemma:subcapt-join}.

  \emph{Case \textsc{tapply} and \textsc{open}}. As above.

  \emph{Case \textsc{let-value}}.
  In this case, $t = \evctx{\tLetMode{m}{x}{v}{s}}$,
  $t^\prime = s$,
  $\sta^\prime = \sta, \tVal{x} \mapsto v$,
  and $\dom{e} \cap \fv{v} = \varemptyset$.
  We invoke Lemma \ref{lemma:evctx-typing-inv} and show that there exists $\Delta, Q$ such that
  $\match{\G}{e}{\Delta}$ and $\typ{\G, \Delta}{\tLetMode{m}{x}{v}{s}}{Q}$.
  By inverting the typing judgment we can show that
  $\typ{\G, \Delta}{v}{\tCap{\cv{v}}{S}}$
  and $\typ{\G, \Delta, x :_m \tCap{\cv{v}}{S}}{s}{Q}$.
  Also, if $m =\ !$, we also have $\ninterfp{\G, \Delta}{\cv{v}}{\cv{s}/x}$.
  If $m =\ !$, then we invoke Lemma \ref{lemma:erase-ninter} and show that
  $\typ{\G, \Delta, x :_\epsilon \tCap{\cv{v}}{S}}{s}{Q}$.
  Therefore, in both cases we show that
  $\typ{\G, \Delta, x :_\epsilon \tCap{\cv{v}}{S}}{s}{Q}$.
  Since we have $\typ{\G, \Delta}{\tLetMode{m}{x}{v}{s}}{T}$,
  by weakening we have $\typ{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{\tLetMode{m}{y}{v}{[y/x] s}}{Q}$.
  Also, $\typ{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{s}{Q}$ by permutation of the typing context.
  Now to invoke Lemma \ref{lemma:evctx-reification-subcapt}
  we have to show that $\sub{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{\cv{s}}{\cv{\tLetMode{m}{y}{v}{[y/x] s}}}$.
  Also, note that $\cv{\tLetMode{m}{x}{v}{s}} = \cv{\tLetMode{m}{y}{v}{[y/x] s}}$.
  Now split into two cases.
  If $x \notin \cv{s}$, we have $\cv{s} = \tLetMode{m}{x}{v}{s} = \cv{s}/x$ and we conclude.
  Otherwise, if $x \in \cv{s}$, we have $\cv{s} = \cv{s}/x \cup \set{x}$,
  and $\cv{\tLetMode{m}{x}{v}{s}} = \cv{s}/x \cup \cv{v}$.
  We have $\sub{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{\set{x}}{\cv{v}}$.
  We conclude that $\sub{\G, x :_\epsilon \tCap{\cv{v}}{S}, \Delta}{\cv{s}}{\cv{\tLetMode{m}{y}{v}{[y/x] s}}}$
  by Lemma \ref{lemma:subcapt-join}.
  Therefore we have $\typ{\G, x :_\epsilon \tCap{\cv{v}}{S}}{\evctx{s}}{T}$ and conclude.

  \emph{Case \textsc{rename}}. As above.

  \emph{Case \textsc{var-value}}.
  In this case, $t = \evctx{\tLetVar{x}{v}{u}}$, $t^\prime = \evctx{u}$,
  $\sta^\prime = \sta, \tVar{x} = v$
  and $\dom{e} \cap \fv{v} = \varemptyset$.
  Now we invoke Lemma \ref{lemma:evctx-typing-inv}
  and show that there exists $\Delta, Q$ such that
  $\match{\G}{e}{\Delta}$
  and $\typ{\G, \Delta}{\tLetVar{x}{v}{u}}{Q}$.
  By inverting this typing judgment,
  we show that $\typ{\G, \Delta}{v}{S}$ for some $S$.
  Now invoke Lemma \ref{lemma:star-notin-eps-binding}
  to show that $\forall y :_\epsilon \tCap{C}{S} \in \G$ we have $* \notin C$.
  Having shown this, we can invoke Lemma \ref{lemma:lift-var-to-store}
  and show that $\typ{\G, x :_! \tCap{\set{*}}{\tRef{S}}}{\evctx{u}}{T}$.
  Finally, we show that $\match{}{\sta, \tVar{x} = v}{\G, x :_! \tCap{\set{*}}{\tRef{S}}}$
  and conclude this case.

  \emph{Case \textsc{lookup}}.
  As above.

  \emph{Case \textsc{lift-set}}.
  In this case, $t = \evctx{\tWrite{x}{y}}$,
  $\sta(\tVal{y}) = v$,
  $x \in \bvar{\sta}$,
  $t^\prime = v$,
  and $\sta^\prime = \sta, \tSet{x} = v$.
  Notice that $\match{}{\sta^\prime}{\G}$ holds.
  To proceed we invoke Lemma \ref{lemma:evctx-typing-inv}
  to show that there exists $\Delta, Q$,
  such that $\match{\G}{e}{\Delta}$,
  and $\typ{\G, \Delta}{\tWrite{x}{y}}{Q}$.
  By inverting the typing judgment,
  we can show that $\typ{\G, \Delta}{x}{\tCap{C_x}{\tRef{S}}}$,
  $\typ{\G, \Delta}{y}{S}$ and $\sub{\G, \Delta}{S}{Q}$.
  Now we invoke Lemma \ref{lemma:val-lookup-inv}
  to show that $\typ{\G, \Delta}{v}{S}$.
  Therefore, we have $\typ{\G, \Delta}{v}{S}$.
  Now to invoke Lemma \ref{lemma:plug-back-evctx} and conclude this case
  the remaining to be shown is that
  $\sub{\G, \Delta}{\cv{v}}{\set{x, y}}$.
  We invert the typing of $\typ{\G, \Delta}{v}{S}$
  to show that $\sub{\G, \Delta}{\cv{v}}{\varemptyset}$,
  and thus conclude this case.

  \emph{Case \textsc{read}}.
  Similar to the previous case.
\end{proof}
